Multidimensional Eigenwave Multiplexing Modulation for Non-Stationary Channels

While interference in time domain (caused by path difference) is mitigated by OFDM modulation, interference in frequency domain (due to velocity difference), can be mitigated by OTFS modulation. However, in non-stationary channels, the relative difference in acceleration will cause Inter-Doppler Interference (IDI) and a modulation method for mitigating IDI does not exist in the literature. Both methods in the literature use carriers in a specific domain which achieve orthogonality in the target domain to mitigate interference. Moreover, those modulation cannot directly incorporate space domain, which requires additional precoding technique to mitigate inter-user interference (IUI) for MU-MIMO channels. This work presents a generalized modulation for any multidimensional channel. Recently, Higher Order Mercer's Theorem (HOGMT) [1] has been proposed to decompose multi-user non-stationary channels into independent fading subchannels (Eigenwaves). Based on HOGMT decomposition, we develop Multidimensional Eigenwaves Multiplexing (MEM) modulation which uses jointly orthogonal eigenwaves, decomposed from the multidimensional channel as subcarriers. Data symbols modulated by these eigenwaves can achieve orthogonality across each degree of freedom(\eg space (users/antennas), time-frequency and delay-Doppler). Consequently, the transmitted remain independent over the high dimensional channel, thereby avoiding interference from other symbols.

==> AE.tex <==
\section{HOGMT Decomposition}
\label{sec:intro}
\begin{table*}[h]
\caption{Comparison of HOGMT with other channel decomposition methods}
\renewcommand*{\arraystretch}{1.2}
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Decomposition methods} & \textbf{Time-varying} & \textbf{Asymetric} & \textbf{DoF decorrelation} & \textbf{High-order} \\ \hline
SVD: $H = U \Sigma V^*$             &   & \checkmark & \checkmark &          \\ \hline
Karhunen–Loève Transform (KLT): $X(t) = \Sigma_n \sigma_n \phi_n(t)$             &  \checkmark & \checkmark &  &                        \\ \hline
Mercer's Theorem: $K(t,t') = \Sigma_n \lambda_n \phi_n(t) \phi_n(t')$            &  \checkmark & & \checkmark &                    \\ \hline
Generalized Mercer's Theorem (GMT): $K(t,t') = \Sigma_n \sigma_n \psi_n(t) \phi_n(t')$&  \checkmark & \checkmark & \checkmark &  \\ \hline
\rowcolor[HTML]{FFFFBF}HOGMT: $K(\zeta_1{,}{...}{,}\zeta_P{;} \gamma_1{,}{...}{,} \gamma_Q) {=} {\sum_{n}} \sigma_n \psi_n(\zeta_1{,}{...}{,}\zeta_P) \phi_n(\gamma_1{,}{...}{,}\gamma_Q)$ 
    &  \checkmark & \checkmark & \checkmark & \checkmark
\\ \hline
\end{tabular}
\label{tab:decomp}
\end{table*}

 We express the spatio-temporal channel response %\cite{2011Hlawatsch} 
% is expressed 
by extending the time-varying response $h(t,\tau)$ to incorporate multiple users, i.e., $h_{u,u'}(t,\tau)$ \cite{almers2007survey}, which denotes the time-varying impulse response between the $u'$\textsuperscript{th} transmit antenna and the $u$\textsuperscript{th} user. Without loss of generality, for convenience of exposition let us consider the case where each user has a single antenna. 
Thus the received signal in \eqref{eq:h_relation} is extended to
% by extending the time-varying response $h(t,\tau)$ to incorporate multiple users, i.e., $h_{u,u'}(t,\tau)$ \cite{2017GhazalNSmodel}, where $u$ is the antenna index of combined all receivers and $u'$ is the antenna index of the transmit. The 4-D spatio-temporal channel estimation is widely investigated \cite{2020CESrivastava,2005CEXiaoli,2008CEMilojevic} . In this paper we assume perfect CSI at transmit. Thus the received signal in \eqref{eq:h_relation} is extended as}
% \ingreen{The kernel $\mathcal{H}(t, f ; \tau, \nu)$ in \eqref{eq:compute_H} is used to extract the statistics for non-stationary channel $H$ which across time-frequency delay-Doppler domain. While the input-output relation can still denote as \eqref{eq:h_relation}. The spatio-temporal channel response \cite{MATZ20111} %\cite{2011Hlawatsch} 
% is expressed by extending \eqref{eq:h_relation} to incorporate multiple users as in \eqref{eq:MU}},
the multi-user case of $h(t,\tau)$ and is given by \eqref{eq:H_t_tau},
\begin{align}
\label{eq:H_t_tau}
\mathbf{H}(t,\tau) = \begin{bmatrix}
 h_{1,1}(t,\tau) &\cdots & h_{1,u'}(t,\tau)  \\
 \vdots& \ddots &  \\
h_{u,1}(t,\tau) &  & h_{u,u'}(t,\tau)
\end{bmatrix}
\end{align}
% 
% where $h_{u,u'}(t,\tau)$ \cite{almers2007survey} denotes the time-varying impulse response between the $u'$\textsuperscript{th} transmit antenna and the $u$\textsuperscript{th} user, where each user has a single antenna. 
Therefore, the received signal in \eqref{eq:h_relation} is extended as in \eqref{eq:r_mu_discrete}.
\begin{table*}[h]
\begin{align}
    r_u (t) &{=} \int \sum_{u'} h_{u,u'}(t,\tau) s_{u'}(t-\tau) d\tau + v_{u}(t) \label{eq:r_mu_discrete} \\
    &{=} \underbrace{h_{u,u}(t,0)s_{u}(t)}_\text{Signal with the attenuation coefficient} + \underbrace{\sum_{u'\neq u} h_{u,u'}(t,0)s_{u'}(t)}_\text{Spatial interference} + \underbrace{\int h_{u,u}(t,\tau) s_{u}(t-\tau) d\tau}_\text{Temporal interference} + \underbrace{\int \sum_{u' \neq u} h_{u,u'}(t,\tau) s_{u'}(t-\tau)d\tau}_\text{Joint spatio-temporal interference} + \underbrace{v_{u}(t)}_\text{Noise} \label{eq:r_mu}
    % r_u (t) &= \sum_{u'} h_{u,u'}(t,\tau) s_{u'}(t-\tau) + v_{u}(t) \nonumber \\
    % & = \sum_{u'} k_{u,u'}(t,t') s_{u'}(t') + v_{u}(t)
\end{align}
\end{table*}
The first term in \eqref{eq:r_mu} is desired signal with fading effects. 
Spatial and temporal interference correspond to the second and third terms in \eqref{eq:r_mu}.
Additionally, the space-time kernel induces joint spatio-temporal due to the interference from delayed symbols from other users as shown in the last term of \eqref{eq:r_mu}. 

==> KLT_precoding.tex <==
\section{KLT based precoding}
\label{sec:klt_precoding}
\subsection{Optimization}
Equation~\ref{eq:argmin} aims to minimize the space-time-frequency interference, denoted as $\epsilon(x)$
\begin{equation}
\epsilon(x) = \sum_{u} \sum_{k} \sum_{p}||s(u,k,p) - \sum_{n=1}^N x_n \sigma_n(u,k,p)||^2
\end{equation}

Sum $\sigma_n(u,k,p)$ along eigen dimension. Then by KLT decompostion, we can get the eigen basis (eigenfunctions) of $\{ \sigma_n\}$
\begin{align}
    A(u,k,p) & {=} \sum_{n=1}^N \sigma_n(u,k,p) \nonumber\\
    &{=} \sum_{j}^J e_j \phi_j(u,k,p) \nonumber 
\end{align}

Then $\sigma_n$ can be represented as
\begin{align}
   &\sigma_n(u,k,p) {=} \sum_{j}^J e_{n,j} \phi_j(u,k,p) \quad \text{where,} \quad \nonumber\\
    &e_{n,j} = \sum_u \sum_k \sum_p \sigma_n(u,k,p) \phi_j(u,k,p)
\end{align}

$\epsilon(x)$ can be rewritten as

\begin{align}
    & \epsilon(x) {=} \sum_u \sum_k \sum_p ||s(u,k,p) - \sum_{n}^N x_n \sum_j^J e_{n,j} \phi_j(u,k,p)||^2 \nonumber\\
    & {=} \sum_u \sum_k \sum_p ||s(u,k,p) - \sum_j^J \sum_{n}^N x_n e_{n,j} \phi_j(u,k,p)||^2 \nonumber\\
    & {=} \sum_u \sum_k \sum_p \{ ||s(u,k,p)||^2 - 2\sum_j^J \sum_{n}^N x_n e_{n,j} \phi_j(u,k,p) \nonumber\\
    & {\cdot} s(u,k,p) + \sum_j^J \sum_{n}^N \sum_{j'}^J \sum_{n'}^N x_n x_{n'} e_{n,j} e_{n',j'} \phi_j(u,k,p) \nonumber\\
    & {\cdot} \phi_{j'}(u,k,p) \} \nonumber \\
    & {=} e_{s,s} - 2\sum_j^J \sum_{n}^N x_n e_{n,j} e_{s,j} + \sum_j^J \sum_{n}^N x_n^2 e_{n,j}^2 \nonumber \\
    & {+} \sum_j^J \sum_{n}^N \sum_{n'\neq n}^N x_n x_{n'} e_{n,j} e_{n',j}  \nonumber \\ 
\end{align}
where $e_{s,s} = \sum_u \sum_k \sum_p ||s(u,k,p)||^2$ is the energy of $S$, and $e_{s,j} = \sum_u \sum_k \sum_p s(u,k,p) \phi_j(u,k,p)$ is the projection of $S$ onto $\phi_j$.

To find the minimum $\epsilon(x)$, let the partial derivative of $\epsilon(x)$ with respect to $x_n$ be zero
\begin{align}
    \pdv{\epsilon(x)}{x_n} & {=} - 2\sum_j^J e_{n,j} e_{s,j} + 2 \sum_j^J x_n e_{n,j}^2 \nonumber \\
    & {+} 2 \sum_j^J \sum_{n'\neq n}^N x_{n'} e_{n,j} e_{n',j} = 0 \nonumber \\ 
\end{align}

Then $x_n$ is
\begin{align}
    x_n & {=} \frac{\sum_j^J e_{n,j} e_{s,j} + \sum_j^J \sum_{n'\neq n}^N x_{n'} e_{n,j} e_{n',j} }{\sum_j^J e_{n,j}^2} \nonumber \\
    & {=} \frac{\sum_j^J e_{s,n} e_{j,j} + \sum_j^J \sum_{n'\neq n}^N x_{n'} e_{n,n'} e_{j,j} }{\sum_j^J e_{n,n} e_{j,j}} \nonumber \\
    & {=}  \frac{e_{s,n} + \sum_{n'\neq n}^N x_{n'} e_{n,n'} }{e_{n,n}} \nonumber 
\end{align}
where $e_{n,n} = \sum_u \sum_k \sum_p ||\sigma_n(u,k,p)||^2$ is the energy of $\sigma_n$. $e_{s,n}$ and $e_{n,n'}$ are the projection of $S$ and $\sigma_n'$ onto $\sigma_n$, respectively. It's an iterative optimization. 

Specifically, if $\{ \sigma_n \}_n^N$ are orthogonal basis, i.e. $e_{n,n'} = \sum_u \sum_k \sum_p \sigma_n(u,k,p) \sigma_{n'}(u,k,p) = 0 \quad \text{for} \quad n' \neq n$, we have 
\begin{align}
    x_n & {=} \frac{ e_{s,n}}{e_{n,n}} \nonumber \\
\end{align}

\noindent
\textbf{KLT precoding}: 
Decompose the mixed space-time-frequency response $z(m,l,p)$ to get eigenfunction $\{ \phi_n \}$. We can not ensure the projection $\{\sigma_n\}$ are orthogonal to fully cancel interference (here, interference means $\epsilon(x)$).  

Interference: minimize $\epsilon(x)$ but can not ensure $\epsilon(x) = 0$. (in some cases, the combination of non-orthogonal $\{\sigma_n\}$ can achieve $\epsilon(x) = 0$.)

Diversity: fully use.

Complexiy: low.

If KLT precoding can design eigenfunctions $\{ \phi_n \}$ that can directly get orthogonal $\{\sigma_n\}$, it would be optimal with respect to interference, diversity and complexity.

\note{
\noindent
\textbf{BD-KLT precoding}:
Find $N=U*K*P$ eigenfunctions, each eigenfuntion is the zero space of the response of all users over all time and all carriers except for the response at desired $(u,k,p)$, i.e.,
\begin{align}
    & \sum_m \sum_l \sum_q h(u,k,p;m,l,q) * \phi_n^* (m,l,q) \nonumber\\
    &{=} \left\{\begin{array}{ll}
    \sigma_n(u,k,p) & \text { if } n = u*P*K+p*K+k \\
    0 & \text { otherwise}
    \end{array}\right.
\end{align}

Then we can get $N=U*K*P$ orthogonal basis $\{\sigma_n\}$, where $N$ is greater or equal to the rank of $S$. So we must achieve $\epsilon(x) = 0$.  

Interference: $\epsilon(x) = 0$

Diversity: not use other channels gain

Complexiy: low

\noindent
\textbf{THP-KLT precoding}:
Using GS method to get the eigenfunctions of each $h(u,k,p;m,l,q)$. For example, by GS we get
\begin{align}
    &h(1,1,1;m,l,q) = \sigma_1(1,1,1) \phi_1(m,l,q) \nonumber\\
    &h(1,1,2;m,l,q) = \sigma_1(1,1,2) \phi_1(m,l,q) + \sigma_2(1,1,2) \phi_2(m,l,q)
\end{align}

Then we can get $x_n$ by
\begin{align}
    &x_1 = \frac{s(1,1,1)}{\sigma_1(1,1,1)} \nonumber\\
    &x_2 = \frac{s(1,1,2) - x_1 \sigma_1(1,1,2)}{\sigma_2(1,1,2)}
\end{align}

Interference: $\epsilon(x) = 0$

Diversity: fully use

Complexiy: high
}

\subsection{Error analysis}
\note{
\noindent
Waiting for extension.
}
% \begin{equation}
% \mathbf{H}=\sum_{n} \sum_{k} \sum_{m} \sum_{l} \eta_{n, k}^{m, l} \mathbf{\phi}_{n T_{0}, k F_{0}}^{m \tau_{0}, l \nu_{0}}
% \end{equation}

% The ambiguity function of the $x$, $A_{x}(t, f; \tau, \nu)$ is defined by 


% \begin{equation}
% \begin{aligned}
% A_{x}(t, f; \tau, \nu) &=\left\langle x(t), x(t-\tau) e^{j 2 \pi (f-\nu) t}\right\rangle \\
% &=\int x(t) x^{*}(t-\tau) e^{-j 2 \pi (f - \nu t)} d t
% \end{aligned}
% \end{equation}
In this section, we investigate the performance and limitations of the precoding algorithm using eigenfunctions obtained from section \ref{sec:AE}.

\noindent
\inred{Zhibin: Reformulate Lemmas 1-3 to be consistent with Section III.}

\begin{lemma}
\label{lemma:1}
Let $\{\hat{\phi}_n\}_{n=1}^N$ be the \note{eigenfunctions corresponding to the obsolete CSI/ prediction}, then the precoded signal {X} can be decomposed by
\begin{equation}
\begin{aligned}
X &=\sum_{n}^{N} x_{n} \hat{\phi}_{n} \\
&=\sum_{n}^{N} \langle\phi_{n}, \hat{\phi}_{n} \rangle \phi_{n} x_{n}+\langle \Delta \phi_{n}, \hat{\phi}_{n} \rangle \Delta \phi_{n} x_{n}
\end{aligned}
\end{equation}\
where, $\phi_n$ is $n^{th}$ eigenfuntion of real channel.  $\Delta \phi_n $ is the prediction error and orthogonal to $\phi_n$ , and 
\begin{equation}
    \langle \phi_n ,\phi_m \rangle = \int \phi_n \phi_m d t
\end{equation}
denotes the inner product. Where we have $\langle \phi_n ,\phi_n \rangle = 1, \langle \Delta \phi_n ,\phi_n \rangle = 0, \langle \phi_n ,\phi_m \rangle = 0 ~ \text{for} ~ n \neq m$, and

\begin{equation}
    \langle \hat{\phi}_n ,\hat{\phi}_n \rangle ^2 = \langle \phi_n ,\hat{\phi}_n \rangle ^2 + \langle \Delta \phi_n ,\hat{\phi}_n \rangle ^2
\end{equation}
\end{lemma}
The proof is provided in Appendix~\ref{app:lemma_1}.

\begin{lemma}
\label{lemma:2}
The eigenfunctions prediction error $\Delta\Phi = \{\Delta \phi_n\}_{n=1}^N$ can be equivalent to CSI error $\Delta H = \sum_{n=1}^{N} \Delta \sigma_n \phi_n$ where
\begin{equation}
\Delta \sigma_{n}=\frac{\sigma_{n} \sum_{m} x_{m} \langle \phi_{n}, \Delta \phi_{m}\rangle}{x_{n}}
\end{equation}
\end{lemma}

The proof is provided in Appendix~\ref{app:lemma_2}.

\begin{lemma}
\label{lemma:3}
Given CSI error $\Delta H$, the expected transmit error is bounded by 
\begin{equation}
\sigma_{N} \min \left(x_{1}\cdots x_{N}\right) E_{\Delta} \leqslant E[ \Delta H \tilde{X} ]\leqslant \sigma_{1} \max \left(x_{1}\cdots x_{N}\right) E_{\Delta},
\end{equation}
where, $E_{\Delta}=\int \Delta \Phi \cdot \Phi$. $\tilde{X}$ is the transmitted signal precoded by perfect eigenfunctions.
\end{lemma}
The proof is provided in Appendix~\ref{app:lemma_3}.


\note{The objective function can choose minimizing MSE $E\{|\Delta H \tilde{X}|^{2}\}$ or maximizing the SINR}

\begin{equation}
\argmax_{\{x_{n}\} \{\hat{\phi}_{n}\}} \mathrm{SINR}=\frac{E\{|H \tilde{X}|^2\}}{\sigma_W^{2}+E\{|\Delta H \tilde{X}|^2\}}
\end{equation}








\begin{comment}


The received signal can be written as
\begin{equation}
Y = HX + W.    
\end{equation}

Let $E\{W^2\} = \sigma^2_W$. We have
\begin{equation}
\begin{aligned}
& E\{H X\} \\
=& \int \sum_{n}^{N} \sigma_{n} \phi_{n} \cdot \sum_{m}^{N} X_{m}(\langle \hat{\phi}_{m}, \phi_{m} \rangle \phi_{m}+\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle \Delta \phi_{m}) d t\\
=& \sum_{n}^{N} \int \sigma_{n} \phi_{n} \cdot x_{n}(\langle\phi_{n}, \hat{\phi}_{n}\rangle \phi_{n}+\langle\phi_{n}, \hat{\phi}_{n} \rangle \Delta \phi_{n})\\
+&\sum_{m \neq n}^{N} \sigma_{n} \phi_{n} \cdot x_{m}(\langle\phi_{m}, \hat{\phi}_{n}\rangle \phi_{m}+\langle\Delta \phi_{n}, \hat{\phi}_{m}\rangle \Delta \phi_{n}) d t\\
=& \sum_{n}^{N}\{\sigma_{n} x_{n}\langle \phi_{n} \hat{\phi}_{n}\rangle \cdot \int \phi_{n} \phi_{n} d t +\sigma_{n} x_{n}\langle\Delta \phi_{n}, \hat{\phi}_{n}\rangle \cdot\int \phi_{n} \Delta \phi_{n} d t \\
+&\sum_{m \neq n}^{N}[\sigma_{n} x_{m}\langle\phi_{m}, \hat{\phi}_{m}\rangle \cdot \int \phi_{n} \phi_{m} d t+\sigma_{n} x_{m}\langle \Delta \phi_{m} \hat{\phi}_{m} \rangle \int \Delta \phi_{m} \phi_{n} d t]\} \\
=& \sum_{n}^{N}[\sigma_{n} x_{n}\langle\phi_{n}, \hat{\phi}_{n}\rangle+\sum_{m}^{N} \sigma_{n} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle \int \phi_{n} \Delta \phi_{m} d t]\\
=& \sum_{n}^{N}[\sigma_{n} x_{n}\langle\phi_{n}, \hat{\phi}_{n}\rangle+\sum_{m}^{N} \sigma_{n} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle \langle \phi_{n}, \Delta \phi_{m} \rangle]\\
\end{aligned}
\end{equation}

We also have 

\begin{equation}
\begin{aligned}
E\{H \tilde{X}\} &=\int \sum_{n}^{N} \sigma_{n} \phi_{n}  \cdot \sum_{m}^{N} x_{m} \phi_{m} d t \\
&=\sum_{n} \sigma_{n} x_{n} .
\end{aligned}
\end{equation}

Thus the MSE caused by imperfect CSI is given by
\begin{equation}
\begin{aligned}
& E\{|\Delta H \tilde{X}|^{2}\}= E\{|H \Delta X|^{2}\} = E\{|H X-H \tilde{X}|^{2}\}\\
=&E\{| \sum _ { n } [ \sigma_{n} x_{n} ( \langle\phi_{n}, \hat{\phi}_{n}\rangle -1) +\sum_{m}^{N} \sigma_{n} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle \langle\Delta \phi_{m}, \phi_{n}\rangle ]|^{2} \} \\
=&E\{|\sum_{n}^{N} \sigma_{n}[x_{n}(\langle\phi_{n}, \hat{\phi}_{n}\rangle-1) +\sum_{m}^{N} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle \Delta \phi_{m}, \phi_{n}\rangle]|^{2}\}\\
=& \sum_{n}^{N} E\{\sigma_{n}^{2}|x_{n}(\langle\phi_{n}, \hat{\phi}_{n}\rangle-1)+\sum_{m}^{N} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle\Delta \phi_{m}, \phi_{n}\rangle|^{2}\} \\
&+\sum_{n^{'} \neq n}^{N} E\{\sigma_{n^{'}} \sigma_{n} \cdot |\cdots|^{2}\},
\end{aligned}
\end{equation}

where $|\cdots|^2$ is the residual part, which is uncorrelated with $\sigma_n$. 
Meanwhile $E \{ \sigma_n \sigma_{n^{'}} \} = 0$ for $n \neq n^{'}$ , so the last item is $0$. Then We have

\begin{equation}
\begin{aligned}
&E\{|\Delta H \tilde{X}|^{2}\}\\
=& \sum_{n}^{N} \sigma_{n}^{2} E\{|x_{n}(\langle\phi_{n}, \hat{\phi}_{n}\rangle-1)+\sum_{m}^{N} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle\Delta \phi_{m}, \phi_n \rangle|^{2}\} \\
=& \sum_{n}^{N} \sigma_{n}^{2} E\{| x_{n}[(\langle\phi_{n}, \hat{\phi}_{n}\rangle-1) + \langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle\Delta \phi_{m}, \phi_{n}\rangle]\\
&+\sum_{m \neq n} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle \Delta \phi_{m}, \phi_{n}\rangle|^{2}\}\\
=&\sum_{n}^{N} \sigma_{n}^{2} E\{ x_{n}^{2}[(\langle\phi_{n}, \hat{\phi}_{n}\rangle-1)+ \langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle\Delta \phi_{m}, \phi_{n} \rangle]^{2}\\
&+\sum_{m \neq n}^{N} x_{m}^{2}(\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle\Delta \phi_{m}, \phi_{n} \rangle)^{2}\} + \sum_{n^{'} \neq n}E \{x_{n^{'}} x_{n} \cdot |\cdots|^{2}\}.
\end{aligned}
\end{equation}

Also, $|\cdots|$ is uncorrelated with $x_n$ and $E \{ x_n x_{n^{'}} \} = 0$ for $n \neq n^{'}$. So, we have
\begin{equation}
\begin{aligned}
&E\{|\Delta H \tilde{X}|^{2}\}\\
=&\sum_{n}^{N} \sigma_{n}^{2} \{ x_{n}^{2}[(\langle\phi_{n}, \hat{\phi}_{n}\rangle-1) + \langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle \langle\Delta \phi_{m}, \phi_{n} \rangle]^{2}\\
&+\sum_{m \neq n}^{N} x_{m}^{2}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle ^2 \langle\Delta \phi_{m}, \phi_{n} \rangle^{2}\}.
\end{aligned}
\end{equation}

\note{The objective function can choose minimizing MSE $E\{|\Delta H \tilde{X}|^{2}\}$ or maximizing the SINR}

\begin{equation}
\argmax_{\{x_{n}\} \{\hat{\phi}_{n}\}} \mathrm{SINR}=\frac{E\{|H \tilde{X}|^2\}}{\sigma_W^{2}+E\{|\Delta H \tilde{X}|^2\}}
\end{equation}

% \begin{equation}
% E\{||H X||^2\} = \iiiint \mathcal{C}_{\mathbf{H}}(t, f ; \tau, \nu) \cdot \sigma^2 |\phi|^2 \mathrm{d} t \mathrm{d} f \mathrm{d} \tau \mathrm{d} \nu
% \end{equation}
\end{comment}


\note{
Objectives:\\
1. Model and solve the optimization problem for one criteria (MSE, SINR, EE, BER, etc.) under imperfect CSI/predicted eigenfunctions.\\
2. Predict eigenfunctions (Take the time-memory advantages of KLT over SVD).\\
3. Design autoencoder.}

\begin{theorem}
\note{Generalized precoding theorem: The proposed method is an optimal precoding approach for any channel / better than other methods.}

\end{theorem}


\begin{corollary}
\label{corollary_1}
For SU-MIMO, given perfect time series CSI $H(t) =\sum_{n=1}^{N} \sigma_n \phi_n (t)$, the expected capacity can be achieved by KLT precoding $X(t) = \sum_{n=1}^{N} x_n \phi_n(t)$, where $\{x_n\}_{n=1}^N$ is designed by water filling algorithm.
\end{corollary}

The proof is provided in Appendix [].







==> background_icc.tex <==
\section{Background}
\label{sec:pre}
% \note{Zhibin: I removed some mentions of the LTV channel here and changed it to non-WSSUS check if this is correct.}

The wireless channel is typically expressed by a linear operator $H$, and the received signal $r(t)$ is given by $r(t){=}Hs(t)$, where $s(t)$ is the transmitted signal. The physics of the impact of $H$ on $s(t)$ is described using the delays and Doppler shifts in the multipath propagation~\cite{MATZ20111} given by \eqref{eq:H_delay_Doppler},
%
\begin{equation}
    r(t) = \sum\nolimits_{p=1}^P h_p s(t-\tau_p) e^{j2\pi \nu_p t}
    \label{eq:H_delay_Doppler}
\end{equation}
where $h_p$, $\tau_p$ and $\nu_p$ are the path attenuation factor, time delay and Doppler shift for path $p$, respectively. 
% The generalized form with respect to $\tau$ and $\nu$ is 
\eqref{eq:H_delay_Doppler} is expressed in terms of the overall delay $\tau$ and Doppler shift $\nu$ \cite{MATZ20111} in \eqref{eq:S_H}, 
% \eqref{eq:H_delay_Doppler} is rewritten in a general form %of $H$ 
% with respect to the overall delay $\tau$ and Doppler shift $\nu$ \cite{MATZ20111} in \eqref{eq:S_H}, 
%
\begin{align}
    % &r(t) = \iint S_H(\tau, \nu) s(t{-} \tau) e^{j2\pi \nu t} ~d\tau ~d\nu \label{eq:S_H} \\
    % & {=} \int L_H(t, f) S(f) e^{j2\pi tf} df; \enskip  L_H(t,f) {=} \iint S_H(\tau, \nu) e^{j2\pi (t\nu{-} f \tau)} d\tau d\nu \\
    % & {=} \int h(t, \tau) s(t{-} \tau) d\tau; \enskip h(t,\tau) {=} \int S_H(\tau, \nu) e^{j2\pi t \nu} d\nu \label{eq:h_relation}
    r(t) &= \iint S_H(\tau, \nu) s(t{-} \tau) e^{j2\pi \nu t} ~d\tau ~d\nu \label{eq:S_H} \\
    & = \int L_H(t, f) S(f) e^{j2\pi tf} ~df \\
    & = \int h(t, \tau) s(t{-} \tau) ~d\tau \label{eq:h_relation}
\end{align}
% where $S_H(\tau, \nu)$ is the \textit{(delay-Doppler) spreading function} of channel $H$, which describes the combined attenuation factor for all paths in the delay-Doppler domain. The time-frequency (TF) domain representation of $H$ is characterized by its \textit{TF transfer function}, $L_H(t,f)$, which is obtained by the 2-D Fourier transform of $S_H(\tau, \nu)$ as in \eqref{}. The time-varying response is $h(t,\tau) = \int S_H(\tau, \nu) e^{j2\pi t \nu} ~d\nu$.
where $S_H(\tau, \nu)$ is the \textit{(delay-Doppler) spreading function} of channel $H$, which describes the combined attenuation factor for all paths in the delay-Doppler domain. $S(f)$ is the Fourier transform of $s(t)$ and the time-frequency (TF) domain representation of $H$ is characterized by its \textit{TF transfer function}, $L_H(t,f)$, which is obtained by the 2-D Fourier transform of $S_H(\tau, \nu)$ as in \eqref{eq:TF_SH}. 
The time-varying impulse response $h(t,\tau)$ is obtained as the Inverse Fourier transform of $S_H(\tau, \nu)$ from the Doppler domain to the time domain as in  \eqref{eq:h_SH}.
\begin{align}
    L_H(t,f) &{=} \iint S_H(\tau, \nu) e^{j2\pi (t\nu{-} f \tau)} ~d\tau ~d\nu \label{eq:TF_SH}\\
    h(t,\tau) &{=} \int S_H(\tau, \nu) e^{j2\pi t \nu} ~d\nu \label{eq:h_SH}
\end{align}
% where $S_H(\tau, \nu)$ is the \textit{(delay-Doppler) spreading function} of channel $H$, which describes the combined attenuation factor for all paths in the delay-Doppler domain. $S(f)$ is the Fourier transform of $s(t)$ and the time-frequency (TF) domain representation of $H$ is characterized by its \textit{TF transfer function}, $L_H(t,f)$, which is obtained by the 2-D Fourier transform of $S_H(\tau, \nu)$ as $L_H(t,f) {=} \iint S_H(\tau, \nu) e^{j2\pi (t\nu{-} f \tau)} ~d\tau ~d\nu$. The time-varying response is $h(t,\tau) {=} \int S_H(\tau, \nu) e^{j2\pi t \nu} ~d\nu$.
% where $S_H(\tau, \nu)$ is the \textit{(delay-Doppler) spreading function} of channel $H$, which is the overall (all paths) attenuation factor at delay-Doppler domain. 
% \note{Do we need this: In this paper, we follow the LTV model in~\cite{MATZ20111}.}
% \ingreen{
% The time-varying response $h(t,\tau)$ of the channels is given by \eqref{eq:h_tau},
% \begin{equation}
% \label{eq:h_tau}
%     h(t,\tau) = \int S_H(\tau, \nu) e^{j2\pi t \nu} ~d\nu
% \end{equation}
% Maqsood: the $h(t,\tau$ in (21) is defined here.}
% The time-frequency (TF) domain representation of $H$ is characterized by its \textit{TF transfer function}, $L_H(t,f)$, which is obtained by the 2-D Fourier transform of $S_H(\tau, \nu)$ as in \eqref{eq:TH_L_H},
% \begin{align}
%     L_H(t,f) = \iint S_H(\tau, \nu) e^{j2\pi (t\nu{-} f \tau)} ~d\tau ~d\nu
%     \label{eq:TH_L_H}
% \end{align}
%
%
% For LTI channel TF transfer function is reduced to frequency response $L_H(t,f) {=} H(f)$. 
Figures \ref{fig:SH} and \ref{fig:LH} show the time-varying response and TF transfer function for an example of a time-varying channel. 
% \ingreen{Maqsood: I will show the $h(t,\tau)$ and $L_H(t,f)$ figures and they can both show NS. It's better to explain (6) and (7) by $h(t,\tau)$ instead of $S_H$.}
% \noindent
% \note{Is it needed:}
For stationary channels, the TF transfer function is a stationary process with $\mathbb{E}\{L_H(t, f) L_H^*(t',f')\} {=} R_H(t{-}t',f{-}f')$, and the spreading function is a white process (uncorrelated scattering), i.e., $\mathbb{E}\{S_H(\tau, \nu) S_H^*(\tau',\nu')\} {=} C_H(\tau,\nu) \delta (\tau{-} \tau') \delta(\nu{-} \nu')$, where $\delta(\cdot)$ is the Dirac delta function.
$C_H(\tau,\nu)$ and $R_H(t-t',f-f')$ are the \textit{scattering function} and \textit{TF correlation function}, respectively, which are related via 2-D Fourier transform, 
% as,
% \textbf{WSSUS channel:} 1) TF transfer function is a stationary process with $\mathbb{E}\{L_H(t, f) L_H^*(t',f')\} {=} R_H(t-t',f-f')$. 2) Spreading function is a white process (uncorrelated scattering), i.e., $\mathbb{E}\{S_H(\tau, \nu) S_H^*(\tau',\nu')\} {=} C_H(\tau,\nu) \delta (\tau{-} \tau') \delta(\nu{-} \nu')$ .
% $C_H(\tau,\nu)$ and $R_H(t-t',f-f')$ are \textit{scattering function} and \textit{TF correlation function}, respectively, which are related via 2-D Fourier transform
% \useshortskip
\begin{equation}
    C_H(\tau,\nu) = \iint R_H(\Delta t, \Delta f) e^{-j2\pi(\nu \Delta t -  \tau \Delta f)} ~d\Delta t ~d\Delta f
\end{equation}
% \noindent
% \textbf{Non-WSSUS channel:}
In contrast, for non-stationary channels, the TF transfer function is non-stationary process and the spreading function is a non-white process. %Since $C_H(\tau,\nu)$ is not defined for non-WSSUS channel, 
Therefore, a \textit{local scattering function} (LSF) $\mathcal{C}_H(t,f;\tau,\nu)$ \cite{MATZ20111} is defined to extend $C_H(\tau,\nu)$ to the non-stationary channels in \eqref{eq:LSF}. 
Similarly, the \textit{channel correlation function} (CCF) $\mathcal{R}(\Delta t, \Delta f;\Delta \tau, \Delta \nu)$ generalizes $R_H(\Delta t, \Delta f)$ to the non-stationary case in \eqref{eq:CCF}.
\begin{align}
\begin{split}
    &\mathcal{C}_H(t,f ; \tau,\nu)  \label{eq:LSF}\\
    & {=} {\iint} R_L(t, f; \Delta t, \Delta f) e^{-j2\pi(\nu \Delta t -  \tau \Delta f)} ~d\Delta t ~d\Delta f  \\
    & {=} \iint R_S(\tau, \nu; \Delta \tau, \Delta \nu) e^{-j2\pi(t \Delta \nu -  f \Delta \tau)} ~d\Delta \tau ~d\Delta \nu \\
\end{split}\\
\begin{split}
    &\mathcal{R}(\Delta t, \Delta f;\Delta \tau, \Delta \nu) \label{eq:CCF}\\
    & {=} \iint R_L(t, f; \Delta t, \Delta f) e^{-j2\pi(\Delta \nu  t -  \Delta \tau  f)} ~d t ~d f \\
    & {=} \iint R_S(\tau, \nu; \Delta \tau, \Delta \nu) e^{-j2\pi(\Delta t \nu -  \Delta f  \tau)} ~d \tau ~d \nu
\end{split}
\end{align}
where $R_L(t, f; \Delta t, \Delta f){=}\mathbb{E}\{L_H(t, f {+} \Delta f) L_H^*(t {-} \Delta t, f)\}$ and $R_S(\tau, \nu; \Delta \tau, \Delta \nu){=}\mathbb{E}\{S_H(\tau, \nu {+} \Delta \nu) S_H^*(\tau{-} \Delta \tau, \nu)\}$. 
For stationary channels, CCF reduces to TF correlation function $\mathcal{R}(\Delta t, \Delta f;\Delta \tau, \Delta \nu){=}R_H(\Delta t, \Delta f) \delta(\Delta t) \delta(\Delta f)$.
\textit{Due to space constraint, the complete proofs of Theorems and Lemmas are provided in an external document \cite{appendix_link}. 
% \ingreen{ they are defined by Matz' paper, not proved by us.}
}
% 
\vspace{-10pt}
\begin{figure}[h]
\begin{subfigure}{.24\textwidth}
  \centering
%   \includegraphics[trim={0 0 0 3cm},clip,width=1\linewidth]{figures/ht_tau_cropped.pdf}
\includegraphics[width=1\linewidth]{figures/ht_tau_cropped.pdf}
  \vspace{-20pt}
  \caption{Time-varying response $h(t,\tau)$}
  \label{fig:SH}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/L_H_cropped.pdf}
  \vspace{-20pt}
  \caption{TF transfer function $L_H(t,f)$}
  \label{fig:LH}
\end{subfigure}
\caption{Illustration of a non-stationary channel}
% \note{Is this time-varying or non-WSSUS? Change rotation of a) to match b)} 
  \vspace{-10pt}
\label{fig:toychannel}
\end{figure}
% \rood{Zhibin: Check whether eq.s (1)--(6) are directly used in the rest of the paper. If not, we need to cite and remove unless necessary somehow.} 

% \ingreen{Maqsood: In LTV channel, input relation of both WSSUS and non-WSSUS channel are the same ($h(t,\tau)$, $S_H$, $L_H$). We can only distinguish them by the statistics. That's why we need (6),(7) and other statistics to describes the non-WSSUS channel. They are not directly used but give us motivation to do unified characterization. Define unified characterization: all statistics/properties of any channel can be characterized by the same components (eigenvalues and eigenfunctions) decomposed by most general kernel $\mathcal{H}$}








\begin{comment}
Meanwhile, there is an inverse Fourier transformation from $\nu$ to $t$ in equation~\ref{eq:S_H}. Let $h(t,\tau) {=} \int S_H(\tau, \nu) e^{j2\pi \nu t} ~d\nu$, we have 

\begin{equation}
    r(t) = \int h(t,\tau) s(t{-} \tau) ~d\tau
\end{equation}
where $h(t,\tau)$ denotes time-varying impulse response. For NS channel, the correlation of time-varying response can be expressed as 

\begin{equation}
     R_h(t,\tau; \Delta t, \Delta \tau) \triangleq \mathbb{E}\{h(t,\tau+ \Delta \tau) h^*(t-\Delta t,\tau)\}
\end{equation}

In WSSUS channel case, $R_h(t,\tau; \Delta t, \Delta \tau) {=} R_h(\Delta t;\Delta \tau)$.  
\end{comment}


==> comment.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/data_flow.pdf}
    \caption{Data flow}
    \label{fig:Data_flow}
    \vspace{-10pt}
\end{figure*}

Figure~\ref{fig:Data_flow} shows the data flow of the space-time OFDM system. The kernel $k_H(u,t;u',t')$ has two explanations: 
\begin{enumerate}
    \item View from delay domain, the kernel can be seen as the time-varying delay response for MU case. The delay taps are non-stationary over time. The precoding aim to cancel ISI, IUI and ISI-IUI. 
    \item View from space domain, the kernel can be seen as time-varying space response with space delay. The space response are non-stationary over time. The precoding aim to cancel IUI and delayed IUI. 
\end{enumerate}

For the first explanation, it can also extend to space-time-frequency domain, where the kernel would be 6-D and the precoding can cancel ISI, IUI, ICI and ISI-ICI-IUI. For the second explanation, it can be seen as a MU precoding and can be combined with OFDM or OTFS.

\noindent
\textbf{Comparison with OTFS:} The OTFS delay-Doppler input-output relation can be expressed as continuous form
\begin{equation}
\label{eq:otfs_1}
    r(t,f) = \iint h_w(\tau, \nu) s(t - \tau, f - \nu) ~d\tau ~d\nu + v(t,f)
\end{equation}
where $v(\tau,\nu)$ is noise, and $h_w (\tau, \nu)$ is the convolution of delay-Doppler response $h_c(\tau, \nu)$ with window function $w(\tau,\nu)$ (Heisenberg transform):
\begin{equation}
\label{eq:otfs_2}
h_{w}(\tau, \nu)=\iint e^{-j 2 \pi \nu^{\prime} \tau^{\prime}} h_c\left(\tau^{\prime}, \nu^{\prime}\right) w\left(\nu-\nu^{\prime}, \tau-\tau^{\prime}\right) \mathrm{d} \tau^{\prime} \mathrm{d} \nu^{\prime}
\end{equation}

Notice $h_w(\tau, \nu)$ is the phase-shift correlation function of delay-Doppler response and window function for stationary case. \eqref{eq:otfs_1} is a composition of two Heisenberg transforms (Twisted convolution property), one corresponding to the modulation (window), and the other corresponding to the channel.

For kernel $K(u,t;u',t')$, the HOGMT precoding has different objective with OTFS and is not comparable but can combine with OTFS as the second explanation mentioned above. The HOGMT precoding is a general precoding method and can be applied to other kernels. To compare HOGMT precoding with OTFS but specify non-stationary channel, we define \textit{local spreading function} $h(t, f; \tau, \nu)$:

\begin{align}
\label{eq:deflsf}
    & h(t,f; \tau, \nu) \triangleq \mathbb{F}^2 \{ S_H(\tau, \nu + \Delta \nu) g^*(\tau - \Delta \tau, \nu) \} \nonumber \\
    & = \iint S_H(\tau, \nu + \Delta \nu) g^*(\tau - \Delta \tau, \nu) \nonumber \\
    & \times e^{j2\pi (t \Delta \nu - f \Delta \tau)} ~d\Delta \tau ~d\Delta \nu
\end{align}
which denotes delay-Doppler complex attenuation at TF location $(t,f)$. $g(\tau, \nu)$ is the window function with $\iint ||g(\tau,\nu)||^2 ~d\tau ~d\nu {=} 1$. 

The multi-carrier input-output relation for non-stationary channel can be written as 
\begin{equation}
\label{eq:h}
    r(t,f) = \iint h(t,f; \tau, \nu) s(t - \tau, f - \nu) ~d\tau ~d\nu + v(t,f)
\end{equation}

Notice~\eqref{eq:deflsf} and~\eqref{eq:h} has the similar form with~\eqref{eq:otfs_1} and~\eqref{eq:otfs_2}, respectively, but for non-stationary case. OTFS reduce the interference by designing symbols which experience minimal cross. It transmit symbols through delay-Doppler domain where existing less interference than time-frequency domain. However, equalizer is still required to cancel the OTFS intersymbol interference. While HOGMT precoding decompose the channel kernel to jointly orthogonal eigenfunctions (dual-flat fading sub-channels) and design waveform to cancel total interference of the channel. 

\setlength{\textfloatsep}{0.1cm}
\setlength{\tabcolsep}{0.2em}
\begin{table}[h]
\caption{Comparison between OTFS and HOGMT-Precoding}
\renewcommand*{\arraystretch}{1.2}
\centering
\begin{tabular}{|l|l|l|}
\hline
Techniques & OTFS & HOGMT-Precoding \\ \hline
Types     &  Modulation & Precoding\\ \hline
CSI & Perfect CSI at Rx & Perfect CSI at TX             \\ \hline
Channel   &  Staionary & Non-Stationary    \\ \hline
Interference-free & No & Yes \\ \hline
Extension to MU-MIMO &  Additional Equalizer  &  Yes  \\ \hline
\end{tabular}
\label{tab:cha}
\vspace{-10pt}
\end{table}

Overall, OTFS can make general channels "generate" less interference. HOGMT-Precoding is specific to each channel and can cancel existing interference of that channel. 

==> conclusion_icc22.tex <==
\section{Conclusion}
\label{sec:conclusion}

% \note{Rewrite:
% \ingreen{This paper answer Marts' open problem: How can non-WSSUS be decomposed into flat fading channels. By GMT, the channel is decomposed into \textbf{dual eigen flat fading subchannels}. When we transmit one eigenfunctions set with coefficients, because of eigen properties, we actually transfer another eigenfunctions set with the coefficients, which atomic reconstruct data signal.}
In this work, we derived a high-order generalized version of Mercer's Theorem to decompose the general non-stationary channel kernel into 2-dimensional jointly orthogonal flat fading sub-channels (eigenfunctions).
Through theoretical analysis and simulations, we draw three firm conclusions for non-stationary channels: 1) The 2-dimensional eigenfunctions are sufficient to completely derive the second-order statistics of the non-stationary channel and consequently leads to an %accurate and 
unified characterization of any wireless channel, 2) precoding by combining these eigenfunctions with optimally derived coefficients %leads to 
mitigates the spatio-temporal interference, %in non-stationary channels
% mitigates the independent and joint spatio-temporal interference achieving \ingreen{near AWGN BER}
and 3) the precoded symbols when propagated over the non-stationary channel directly reconstruct the data symbols at the receiver when combined with calculated coefficients, consequently alleviating the need for complex complementary decoding at the receiver.
Therefore, the encouraging results from this work will form the core of robust and unifed characterization and highly reliable communication over nonstationary channels, supporting emerging application.
% We propose the generalized Mercer's theorem to decompose the channel kernel into different eigenfunctions. Non-WSSUS channel properties are unifiedly characterized by the decomposed eigenvalues and eigenfunctions. 
% 

% We also studied the precoding technique with eigenfunctions and shows that because of the orthonormal property of eigenfunctions, we can propagate eigenfunctions of channel kernel 
% % \ingreen{not eigenfunctions of channel kernel. eigenfunctions of channel kernel also can have the same dimension by KLT. should be eigenfunctions decomposed by GMT} 
% to achieve the orthornomal projections, which can automatic construct data signals with certain coefficients. 
% }

\section{ACKNOWLEDGEMENT}
This work is funded by the Air Force Research Laboratory Visiting Faculty Research Program (SA10032021050367), Rome, New York, USA.

\begin{comment}
In this paper, the local spreading function is proposed to specify the non-WSSUS channel, which can be decomposed into the time-frequency eigenfunction and delay-Doppler eigenfunction by the proposed novel decomposition method. The statistics is well characterized by the decomposed eigenfunctions and eigenvalues.  

We also studied the precoding technique for non-WSSUS channel and shows that because of the orthonormal property of eigenfunctions, we can propagate eigenfunctions of non-WSSUS channel kernel in delay-Doppler domain to achieve the orthornomal projections in time-frequency domain. With the novel decomposition method, the non-WSSUS channel precoding can achieve interference-free performance.

In the future work, we will investigate more precoding strategies based on non-WSSUS channel decomposition and study the implementation for MU-MIMO non-WSUSS case. 
\end{comment}


\begin{comment}
In this paper, we studied the interpretation of neural network based receivers for single and multiple antenna systems. 
Through rigorous theoretical and empirical analysis we show that a feed-forward deep NN-based receiver with the MSE loss function is equivalent to the optimal classical MAP receiver, under sufficiently rich training. 
We show that under finite training, the expected error is distributed as a Gaussian, and derive tight upper bounds on the BER of the NN-based receivers. %, under finite training samples. 
Extensive practical simulations have corroborated that the BER of such NN-based receivers are within the derived theoretical bounds, and cannot outperform optimal classical receivers when a rigorous mathematical channel model is available. 
% These results show that a single neural network can replace the classical receiver, and learns a computationally tractable algorithm to decode the received signal regardless of the channel condition. 
Moreover, we empirically derive the model of the NN-based receiver for which the error rate is minimum for a given data-set.
The guarantees on the achievable error rate of NN-based receivers is a necessary step towards ensuring wide-spread adoption of NN-based transceivers in xG systems. 
% Furthermore, under incomplete training the BER can be minimized by optimizing the hyper parameters such as the depth and width of the NN-based receiver, which is currently being investigated. 

% However, the DL estimator is sensitive to the quality of training data and its performance would significantly degrade if the data in real environments distributes broader than the training data. 
% The benefits of the DL estimator have to weigh against its costs when applied to the channel estimation in real wireless communication systems. We should strike a balance between DL based channel estimation and traditional channel estimation.


%\note{add more to the conclusion}
% In this paper, we studied the opportunities and limitations of NN-based transceivers over classical approaches for wireless communications.
% Through theoretical proofs, simulation and analysis we draw the following conclusions: 
% 1) the equivalence of NN-based and classical transceivers under known and stationary channels, 
% 2) NN-based transceivers outperform classical transceivers under unknown channel distributions and non-stationary statistics.
% 3) the inverse design of NN-based transceivers achieve guaranteed BER performance,
% Therefore, NN-based transceiver design is only useful in wireless communications, if properly designed and under certain channel conditions. 
\end{comment}














































==> intro_ICC22.tex <==
\section{Introduction}
\label{sec:intro}


Precoding at the transmitter is investigated in the literature and is relatively tractable when the wireless channel is stationary, by employing the gamut of linear algebraic and statistical tools to ensure interference-free communication \cite{Cho2010MIMObook,fatema2017massive,CostaDPC1983}. However, there are many instances, in modern and next Generation %(xG) 
propagation environments such as mmWave, V2X, and massive-MIMO networks, where %the distribution of 
the channel is %either partially observed, undefined, non-linear, higher dimensional or 
statistically non-stationary \cite{wang2018survey,huang2020general,mecklenbrauker2011vehicular} (the distribution is a function of time). 
% The lack of accurate models/ characterization especially for non-stationary channels \cite{}, leads to sub-optimal and sometimes catastrophic performance even with state-of-the-art precoding \cite{AliNS0219}. 
This leads to sub-optimal and sometimes catastrophic performance even with state-of-the-art precoding \cite{AliNS0219} due to two factors: 
a) the time-dependence of the channel statistics,
and b) the existence of interference both jointly and independently across multiple dimensions (space (users/ antennas), frequency or time) in communication systems that leverage multiple degrees of freedom (\eg MU-MIMO, OFDM, OTFS \cite{OTFS_2018_Paper}).
This necessitates a unified characterization of the statistics of wireless channels that can also incorporate time-varying statistics, and novel precoding algorithms 
% that leverage such characterizations 
% that ensure orthogonality across dimensions to 
warrant flat-fading over the higher-dimensional interference profiles in non-stationary channels. 
% 
% \note{
Our solution to the above addresses a challenging open problem in the literature \cite{2006MatzOP} : ``how to decompose non-stationary channels into independently fading sub-channels (along each degree of freedom) and how to precode using them", which is central to both characterizing channels and minimizing interference. 
%warranting interference-free communication. 
% By GMT, the channel is decomposed into \textbf{dual eigen flat fading subchannels}. When we transmit one eigenfunctions set with coefficients, because of eigen properties, we actually transfer another eigenfunctions set with the coefficients, which atomic reconstruct data signal.
% }

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Structure.pdf}
    % \vspace{-5pt}
    \caption{Unified characterization \& precoding
    % \rood{Some modifications}
    % \note{Show the dataflow and maybe integrate parts of fig. 8.}
    } %\note{Remove LTV, and start with CSI.}
    \vspace{-20pt}
    \label{fig:Df}
\end{figure}
Unlike stationary channels,
% the time-frequency dependence of the statistics are constant.}, 
the second order statistics of non-stationary channels are 4-dimensional, as they are functions of both time-frequency and delay-Doppler dimensions\footnote{Second order statistics of stationary channels %employed in the literature %are 2-D and 
depend only on the delay-Doppler (2-D) and hence can be extracted as a degenerate case of the non-stationary channel model, when its time-frequency dependence is constant.} \cite{MATZ20111}.
% \textbf{Unified Characterization:}
% Therefore, the spatio-temporal CSI obtained from each receiver (user) is used to construct a spatio-temporal channel kernel \cite{Matz2005NS}.\ingreen{spatio-temporal CSI and channel kernel is not mentioned is Non-WSSUS channel paper. They just mention $\mathcal{H}(t,f;\tau,\nu)$. And before "Therefore", the last sentense is talk about time-frequency delay-doppler 4-D dimension but here the sentense is about spatio-time domain. They are unrelated. Our precoding 4-D kernel $K_H(u,t;u',t')$ is just straight extension from $h_u(t,\tau)$.} %, corresponding to the time index, frequency and extracted delay and Doppler values.
% \ingreen{Maqsood:In figure 1, 4-D kernel $\mathcal{H} (t , f ; \tau,\nu)$ is defined by Matz's paper~\cite{Matz2005NS}, better directly cite it. Unified characterization is a model part, we don't want to mention CSI and how to get it. Also, this paper doesn't talk about space-time-frequency jointly precoding.}
% The spatio-temporal CSI for MU-MIMO OFDM is given by $\mathcal{H}_{N \times N_{FFT} \times N_{t} \times N_{r} \times N_{u}}$, where $N$, $N_{FFT}$, $N_{t}, N_{r}, N_{u}$ are the number of time samples and OFDM subcarriers respectively. 
% \note{This paper addresses an open problem in the literature (Add relevant citations:\cite{2006MatzOP}): ``how to decompose non-stationary channels into individual flat fading subchannels along each degree of freedom, which is central to minimizing interference. %warranting interference-free communication. 
% By GMT, the channel is decomposed into \textbf{dual eigen flat fading subchannels}. When we transmit one eigenfunctions set with coefficients, because of eigen properties, we actually transfer another eigenfunctions set with the coefficients, which atomic reconstruct data signal.
% Therefore, we consider the most general channel
The core of our wireless channel characterization method, is the decomposition of this 4-dimensional channel kernel into 2-dimensional %spatio-temporal 
eigenfunctions that are jointly orthogonal across these dimensions, using a generalization of Mercer's Theorem to high-dimensional and asymmetric kernels. %of the channel kernel, which results 
% into 2-dimensional %spatio-temporal 
% eigenfunctions that are jointly orthogonal in across these dimensions. %(i.e., they are dual flat-fading subchannels), 
Unlike recent literature that only partially characterize the non-stationary channel using a select few local statistics~\cite{2018PMNS, bian2021general}, these eigenfunctions %decomposed from the most general channel kernel 
are used to extract any second-order statistics of the non-stationary channels that completely characterizes its distribution.  %leading to an accurate and unified characterization of any wireless channel.
% Since these eigenfunctions are obtained by decomposing the most general non-stationary channel kernel, this 
Since any wireless channel model (\eg deterministic, stationary, frequency flat or selective) can be extracted from the general non-stationary channel kernel, the extracted eigenfunctions lead to a unified method to characterize the statistics of any wireless channel. %we show that 
% the proposed characterization and precoding generalizes to any wireless channel (non-stationary/ stationary). 
% These eigenfunctions are used to extract the second-order statistics of the non-stationary channel which completely characterizes its distribution. 
% central to canceling the joint interference across space-time dimensions. 
% The core of our precoding method is the decomposition of this 4-dimensional channel kernel using a generalization of Mercer's Theorem %of the channel kernel, which results 
% into 2-dimensional %spatio-temporal 
% eigenfunctions that are jointly orthogonal in across these dimensions. %(i.e., they are dual flat-fading subchannels), 
% which are central to canceling the joint interference across space-time dimensions. 
% The core of our precoding method is the unified characterization of the channel statistics by a novel high dimensional decomposition (generalization of Mercer's Theorem) of its kernel, which results in 2-dimensional space-time eigenfunctions that are jointly orthogonal in the space-time dimensions, and are central to canceling the interference across space-time dimensions. 
% \rood{Other literature use high-D decomp, but they do not preserve orthogonality in the 2-D time-frequency domains.}
% By definition, eigenfunctions are constituent subchannels %time series 
% of the channel kernel that only undergo a scaling when transmitted over channel. 
% Hence, precoding using those yields interference-free and flat fading at the receiver.
% Unlike recent literature that only partially characterize the non-stationary channel using a select few local statistics (Add 2 citations here:\cite{}), these spatio-temporal eigenfunctions %decomposed from the most general channel kernel 
% can completely define any second order statistics of non-stationary channels leading to an accurate and unified characterization of any wireless channel.
% \rood{Although many literature attempt to characterize the channel they are often impractical as they rely on several statistics, by we do something different...}
% However, while extracting accurate eigenfunctions may lead to optimal precoding, a significant drawback of this method is its extremely high computational complexity to extract large number of eigenfunctions at each time step that makes it impractical \cite{}. We address this with Autoencoder for computational efficiency, generality and adaptability.
% While extracting accurate eigenfunctions may lead to optimal precoding, it is often impractical due to the high computational complexity and the availability of limited CSI at the transmitter \cite{}. 
% Therefore, we rely on a

Figure \ref{fig:Df} shows the data flow for joint spatio-temporal precoding at the transmitter.
% \textbf{Unified Characterization:}
The spatio-temporal CSI obtained from the receivers are used to construct a 4-dimensional channel kernel. 
% Figure \ref{fig:Df} shows the joint spatio precoding system diagram at the transmitter.
% \textbf{Joint space-time precoding:}
In addition to spatial (inter-user or inter-antenna) or temporal (inter-symbol) interference, the time-varying kernel of non-stationary channels, induces joint
space-time interference.
We design a joint space-time precoding at the transmitter that %of symbols to be transmitted 
involves combining the spatio-temporal eigenfunctions obtained by decomposing the space-time channel kernel, with optimal coefficients that %are obtained as the closed-form solution to an 
%are calculated by solving an optimization problem that 
minimize the least square error in the transmitted and received symbols.
Since the eigenfunctions are independently and jointly orthonomal sub-channels over space and time, %(i.e., jointly flat-fading over space and time), 
precoding using them warrants flat-fading (interference-free communication) even in the presence of joint space-time interference. 
Further, these transmitted (precoded) symbols directly reconstruct the data symbols at the receiver when combined with calculated coefficients. 
Therefore, unlike existing precoding methods that require complementary decoding at the receiver\cite{Cho2010MIMObook}, we alleviate any need for complex receiver processing thereby significantly reducing its computational burden. 
% 
% \ingreen{This paper addresses an open problem in the literature: How can non-WSSUS be decomposed into flat fading channels. By GMT, the channel is decomposed into \textbf{dual eigen flat fading subchannels}. When we transmit one eigenfunctions set with coefficients, because of eigen properties, we actually transfer another eigenfunctions set with the coefficients, which atomic reconstruct data signal.}
% 
% By definition, eigenfunctions are constituent subchannels %time series 
% of the channel kernel that only undergo a scaling when transmitted over channel. 
% Hence, precoding using those yields interference-free and flat fading at the receiver.
% Unlike recent literature that only partially characterize the non-stationary channel using a select few local statistics (Add 2 citations here:\cite{}), these spatio-temporal eigenfunctions %decomposed from the most general channel kernel 
% can completely define any second order statistics of non-stationary channels leading to an accurate and unified characterization of any wireless channel.
% \note{We further show that this precoding method also generalizes to any wireless channel (non-stationary/ stationary) and aleviates the need for any complex %complementary 
% decoding, consequently reducing the computational burden at the receiver.}
% 
% Consequently, this precoding ensures minimum interference across dimensions for non-stationary channels, but also generalizes to any other wireless channel. 
% 
% We derive closed-form solution to these coefficients
% These coefficients are extracted as those that minimize the L2-norm between the projection of the CSI onto its extracted eigenfunctions (which results in eigenvalues) and the symbols to  be transmitted. 
% These coefficients are extracted as those that minimize the L2-norm between the projection of the CSI onto its extracted eigenfunctions (which results in eigenvalues) and the symbols to be transmitted. 
Finally, the precoded symbols are scheduled to each user and are processed through the conventional transmitter signal processing blocks (\eg CP/ guard insertion) before transmission.
To the best of our knowledge, precoding for non-stationary channels is unprecedented in the literature. However, we include a comprehensive comparison with related precoding techniques in Appendix A-A %\ref{App:related_NLP} 
in \cite{appendix_link}.
% \vspace{3in}
% 
% Therefore, we make the following contributions:
% \begin{enumerate}
%     % \item We propose a high-order generalization of Mercer's Theorem to decompose the non-stationary channel into spatio-temporal eigenfunctions that are jointly orthogonal in the space-time dimensions.
%     \item We propose a high-order generalization of Mercer's Theorem to decompose the non-stationary channel into spatio-temporal eigenfunctions and derive a unified characterization of any wireless channel by explaining its statistics (Section \ref{sec:NSdec}).
%     % \item We derive a unified characterization of any wireless channel by extracting its second order statistics from the decomposed 2-dimensional eigenfunctions
%     % \item We propose a generalized Mercer's theorem showing the singular value decomposition for the NS channel kernel and gives the eigenfunctions explanation for the NS channel statistics (Section \ref{sec:NSdec}).
%     % \item We design a novel joint spatio-temporal precoding for non-stationary channels, that transmits the eigenfunction combined with optimal coefficients to achieve flat-fading subchannels over each dimension.  %mitigates the interference across space, time and joint space-time domain to approach minimum BER performance at the receiver (Section \ref{sec:Precoding}).
%     \item We design a novel joint spatio-temporal precoding method for non-stationary channels, that mitigates the interference across space, time and joint space-time domain to approach minimum BER performance at the receiver (Section \ref{sec:Precoding}).
%     % \footnote{This is easily extended to space-time-frequency precoding for OFDM communications by considering the frequency dimension.}.
%     % \item We design a generalized joint space-time interferece precoding method for NS channel, which approaches optimal performance across space-time-frequency at a low computational complexity. To our best knowledge, this is the first precoding technique for NS channel (Section \ref{sec:Precoding}).
%     % \item We design an Autoencoder (AE) to extract accurate space-time-frequency eigenfunctions of the channel with low computational complexity (Section \ref{sec:AE}).
%     % \item Through extensive theoretical analysis, we show that our precoding approach outperforms the SoTA for NS channels, while approaching the performance of SoTA for stationary channels.
%     \item Through extensive theoretical analysis and practical simulations, we show the accuracy of the proposed unified channel characterization and joint space-time precoding compared to existing methods.
% \end{enumerate}
% \ingreen{This paper answer Marts' open problem: How can non-WSSUS be decomposed into flat fading channels. By GMT, the channel is decomposed into \textbf{dual eigen flat fading subchannels}. When we transmit one eigenfunctions set with coefficients, because of eigen properties, we actually transfer another eigenfunctions set with the coefficients, which atomic reconstruct data signal.}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PRECODING STORYLINE%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
Precoding at the transmitter is investigated in the literature and is relatively tractable when the wireless channel is stationary, by employing the gamut of linear algebraic and statistical tools to ensure interference-free communication \cite{Cho2010MIMObook,fatema2017massive,CostaDPC1983}. However, there are many instances, in modern and next Generation %(xG) 
propagation environments such as mmWave, V2X, and massive-MIMO networks, where %the distribution of 
the channel is %either partially observed, undefined, non-linear, higher dimensional or 
statistically non-stationary \cite{wang2018survey,huang2020general,mecklenbrauker2011vehicular} (the distribution is a function of time). 
% The lack of accurate models/ characterization especially for non-stationary channels \cite{}, leads to sub-optimal and sometimes catastrophic performance even with state-of-the-art precoding \cite{AliNS0219}. 
This leads to sub-optimal and sometimes catastrophic performance even with state-of-the-art precoding \cite{AliNS0219} due to two factors: a) the lack of accurate models/ characterization for non-stationary channels \cite{}, and b) the existence of interference both jointly and independently across multiple dimensions (space (users/ antennas), frequency or time) in communication systems that leverage multiple degrees of freedom (\eg MU-MIMO, OFDM, OTFS \cite{OTFS_2018_Paper}).
This necessitates a unified characterization of wireless channels that can also incorporate time-varying statistics, and novel precoding algorithms that leverage such characterizations to ensure orthogonality across dimensions to warrant interference-free communication. 
% 

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/Structure.pdf}
    % \vspace{-10pt}
    \caption{Connection of unified characterization \& precoding.} %\note{Remove LTV, and start with CSI.}
    \vspace{-10pt}
    \label{fig:Df}
\end{figure}
Figure \ref{fig:Df} shows the wireless channel characterization and precoding system diagram at the transmitter.
Unlike stationary channels\footnote{Second order statistics of stationary channels employed in the literature %are 2-D and 
depend only on the delay-Doppler (2-D) and hence can be extracted as special cases of non-stationary channels when the time and frequency dependence of the statistics are constant}, the second order statistics of non-stationary channels are 4-dimensional, as they are functions of both time-frequency and delay-Doppler dimensions \cite{MATZ20111}.
% \textbf{Unified Characterization:}
Therefore, the spatio-temporal CSI obtained from each receiver (user) is used to construct a spatio-temporal channel kernel \cite{Matz2005NS}.\ingreen{spatio-temporal CSI and channel kernel is not mentioned is Non-WSSUS channel paper. They just mention $\mathcal{H}(t,f;\tau,\nu)$. And before "Therefore", the last sentense is talk about time-frequency delay-doppler 4-D dimension but here the sentense is about spatio-time domain. They are unrelated. Our precoding 4-D kernel $K_H(u,t;u',t')$ is just straight extension from $h_u(t,\tau)$.} %, corresponding to the time index, frequency and extracted delay and Doppler values.
% \ingreen{Maqsood:In figure 1, 4-D kernel $\mathcal{H} (t , f ; \tau,\nu)$ is defined by Matz's paper~\cite{Matz2005NS}, better directly cite it. Unified characterization is a model part, we don't want to mention CSI and how to get it. Also, this paper doesn't talk about space-time-frequency jointly precoding.}
% The spatio-temporal CSI for MU-MIMO OFDM is given by $\mathcal{H}_{N \times N_{FFT} \times N_{t} \times N_{r} \times N_{u}}$, where $N$, $N_{FFT}$, $N_{t}, N_{r}, N_{u}$ are the number of time samples and OFDM subcarriers respectively. 
\note{This paper addresses an open problem in the literature (Add relevant citations:\cite{2006MatzOP}): ``how to decompose non-stationary channels into individual flat fading subchannels along each degree of freedom, which is central to minimizing interference. %warranting interference-free communication. 
% By GMT, the channel is decomposed into \textbf{dual eigen flat fading subchannels}. When we transmit one eigenfunctions set with coefficients, because of eigen properties, we actually transfer another eigenfunctions set with the coefficients, which atomic reconstruct data signal.
The core of our precoding method is the high dimensional decomposition (by a novel generalization of Mercer's Theorem) of the channel kernel, which results in 2-dimensional spatio-temporal eigenfunctions that are jointly orthogonal in the space-time dimensions (i.e., they are dual flat-fading subchannels), and are central to canceling the joint interference across space-time dimensions. 
% The core of our precoding method is the unified characterization of the channel statistics by a novel high dimensional decomposition (generalization of Mercer's Theorem) of its kernel, which results in 2-dimensional space-time eigenfunctions that are jointly orthogonal in the space-time dimensions, and are central to canceling the interference across space-time dimensions. 
% \rood{Other literature use high-D decomp, but they do not preserve orthogonality in the 2-D time-frequency domains.}
By definition, eigenfunctions are constituent subchannels %time series 
of the channel kernel that only undergo a scaling when transmitted over channel. 
Hence, precoding using those yields interference-free and flat fading at the receiver.
Unlike recent literature that only partially characterize the non-stationary channel using a select few local statistics (Add 2 citations here:\cite{}), these spatio-temporal eigenfunctions %decomposed from the most general channel kernel 
can completely define any second order statistics of non-stationary channels leading to an accurate and unified characterization of any wireless channel.}
% \rood{Although many literature attempt to characterize the channel they are often impractical as they rely on several statistics, by we do something different...}
% However, while extracting accurate eigenfunctions may lead to optimal precoding, a significant drawback of this method is its extremely high computational complexity to extract large number of eigenfunctions at each time step that makes it impractical \cite{}. We address this with Autoencoder for computational efficiency, generality and adaptability.
% While extracting accurate eigenfunctions may lead to optimal precoding, it is often impractical due to the high computational complexity and the availability of limited CSI at the transmitter \cite{}. 
% Therefore, we rely on a
\note{We further show that this precoding method also generalizes to any wireless channel (non-stationary/ stationary) and aleviates the need for any complex %complementary 
decoding, consequently reducing the computational burden at the receiver.}

% \textbf{Joint space-time precoding:}
Joint space-time precoding at the transmitter %of symbols to be transmitted 
involves combining the space-time eigenfunctions with specific coefficients that are obtained as a closed-form solution to an optimization problem that minimizes the least square error in the transmitted and received symbols. 
% \ingreen{This paper addresses an open problem in the literature: How can non-WSSUS be decomposed into flat fading channels. By GMT, the channel is decomposed into \textbf{dual eigen flat fading subchannels}. When we transmit one eigenfunctions set with coefficients, because of eigen properties, we actually transfer another eigenfunctions set with the coefficients, which atomic reconstruct data signal.}
Consequently, this precoding ensures minimum interference across dimensions for non-stationary channels, but also generalizes to any other wireless channel. 
% 
% We derive closed-form solution to these coefficients
% These coefficients are extracted as those that minimize the L2-norm between the projection of the CSI onto its extracted eigenfunctions (which results in eigenvalues) and the symbols to  be transmitted. 
% These coefficients are extracted as those that minimize the L2-norm between the projection of the CSI onto its extracted eigenfunctions (which results in eigenvalues) and the symbols to be transmitted. 
Finally, the precoded symbols are scheduled to each user and are processed through the conventional transmitter signal processing blocks (S/P, IFFT, P/S, CP insertion etc.) before transmission.
To the best of our knowledge a precoding for non-stationary channels is unprecedented in the literature. However, we include a comprehensive comparison with related precoding techniques in Appendix \ref{App:related_NLP} in \cite{appendix_link}.
% \vspace{3in}
% 
Therefore, we make the following contributions: 
% \ingreen{This paper answer Marts' open problem: How can non-WSSUS be decomposed into flat fading channels. By GMT, the channel is decomposed into \textbf{dual eigen flat fading subchannels}. When we transmit one eigenfunctions set with coefficients, because of eigen properties, we actually transfer another eigenfunctions set with the coefficients, which atomic reconstruct data signal.}
\begin{enumerate}
    % \item We propose a high-order generalization of Mercer's Theorem to decompose the non-stationary channel into spatio-temporal eigenfunctions that are jointly orthogonal in the space-time dimensions.
    \item We propose a high-order generalization of Mercer's Theorem to decompose the non-stationary channel into spatio-temporal eigenfunctions and derive a unified characterization of any wireless channel by explaining its statistics (Section \ref{sec:NSdec}).
    % \item We derive a unified characterization of any wireless channel by extracting its second order statistics from the decomposed 2-dimensional eigenfunctions
    % \item We propose a generalized Mercer's theorem showing the singular value decomposition for the NS channel kernel and gives the eigenfunctions explanation for the NS channel statistics (Section \ref{sec:NSdec}).
    % \item We design a novel joint spatio-temporal precoding for non-stationary channels, that transmits the eigenfunction combined with optimal coefficients to achieve flat-fading subchannels over each dimension.  %mitigates the interference across space, time and joint space-time domain to approach minimum BER performance at the receiver (Section \ref{sec:Precoding}).
    \item We design a novel joint spatio-temporal precoding method for non-stationary channels, that mitigates the interference across space, time and joint space-time domain to approach minimum BER performance at the receiver (Section \ref{sec:Precoding}).
    % \footnote{This is easily extended to space-time-frequency precoding for OFDM communications by considering the frequency dimension.}.
    % \item We design a generalized joint space-time interferece precoding method for NS channel, which approaches optimal performance across space-time-frequency at a low computational complexity. To our best knowledge, this is the first precoding technique for NS channel (Section \ref{sec:Precoding}).
    % \item We design an Autoencoder (AE) to extract accurate space-time-frequency eigenfunctions of the channel with low computational complexity (Section \ref{sec:AE}).
    % \item Through extensive theoretical analysis, we show that our precoding approach outperforms the SoTA for NS channels, while approaching the performance of SoTA for stationary channels.
    \item Through extensive theoretical analysis and practical simulations, we show the accuracy of the proposed unified channel characterization and joint space-time precoding compared to existing methods.
\end{enumerate}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD INTRO %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\newpage
Precoding at the transmitter is investigated in the literature and is relatively tractable when the wireless channel is stationary, by employing the gamut of linear algebraic and statistical tools to ensure interference-free communication \cite{}. However, there are many instances, in modern and next Generation (xG) propagation environments such as mmWave, V2X, and massive-MIMO networks, where %the distribution of 
the channel is %either partially observed, undefined, non-linear, higher dimensional or 
statistically non-stationary \cite{} (the distribution is a function of time). 
The lack of accurate models/ characterization especially for non-stationary channels \cite{}, leads to sub-optimal and sometimes catastrophic performance even with state-of-the-art precoding \cite{AliNS0219}. 
The time-varying channel distribution and statistics, necessitates a decomposition (for precoding) that is a function of time (\eg eigenfunctions), but also preserves orthogonality across domains to ensure interference-free communication. 
% However, extracting such eigenfunctions is computationally prohibitive, especially when the channel statistics change rapidly, and for higher dimensional channels (i.e, when there are additional degrees of freedom, like multiple frequency subcarriers in OFDM, large number of antennas in massive/ XL MIMO, or large number of users in MU-MIMO). Therefore, we need computationally tractable methods to extract such eigenfunctions and effectively jointly precode across space-time-frequency to approach interference-free communication at the receiver.
% 
Furthermore, in communication systems that leverage multiple degrees of freedom (space (users/ antennas), frequency or time, \eg MU-MIMO or OFDM), the existence of interference in each or across multiple dimensions, necessitates novel precoding methods that ensure orthogonality of the transmitted signals across each dimension/ plane to ensure interference-free communication. 
% achieving these gains require interference-free communication in all degrees of freedom (i.e., orthogonality of transmissions across space-time-frequency).
% The lack of accurate models/ characterization especially for such non-stationary channels \cite{} and the inability to cancel interference that occurs simultaneously across multiple degrees of freedom leads to sub-optimal and sometimes catastrophic performance even with state-of-the-art precoding \cite{}.
% This leads to sub-optimal and sometimes catastrophic performance even with state-of-the-art precoding \cite{}, due to the lack of accurate models especially for non-stationary channels \cite{} and teh 
% These gains are realized through the ability of MIMO-OFDM communications to achieve higher diversity across multiple degrees of freedom; space (users/ antennas), frequency and time.
% As one of the most promising wireless communication solutions, multiple-input multiple-output (MIMO) technology has been widely used in IEEE 802.11ac/n (WiFi), IEEE 802.16e (WiMAX), LTE/LTE-A (4G), and other protocols and systems [1].
% Therefore, precoding for non-stationary channels  interference-free communication in all degrees of freedom (i.e., orthogonality of transmissions across space-time-frequency).
% Therefore, the central challenge in MIMO transceiver design is to achieve IUI (Inter-User Interference), IAI (Inter-Antenna Interference), ICI (Inter-Carrier Interference) and ISI (Inter-Symbol Interference) free communication at the receiver.
% 


\note{Optimal mitigation of such interference, necessitates pre-processing at the transmitter using Dirty Paper Coding (DPC) \cite{CostaDPC1983} across space-time-frequency dimensions, however it is often impractical as it requires both perfect and complete (up-to-date) Channel State Information (CSI) at the transmitter and incurs a high computational complexity that increases with the number of users and receive antennas.}
This is especially challenging in practical propagation environments where the channel is high dimensional (\eg MU-MIMO, Massive/ XL MIMO) and both time varying and frequency selective (doubly dispersive \cite{}), where only occasional or statistical CSI is available at transmitter. 
Therefore, existing precoding %in the literature 
typically treat these as separate problems, where spatial precoding at the transmitter attempts to mitigate inter-user and inter-antenna interference, while equalization at the receiver attempts to mitigate inter-carrier and inter-symbol interference.
% 
% Optimal spatial precoding techniques exploit DPC across users, and are typically infeasible for practical adoption due to the high complexity (especially in MU/ Massive MIMO). %especially as the number of users or antennas increase (in MU/ Massive MIMO), 
% while linear precoding techniques are sub-optimal \cite{}.
% On the other hand, adaptive time-frequency equalization at the receiver add computational burden to receivers and are sub optimal compared to transmit pre-processing \cite{}. 
% 
Therefore, we believe that space-time-frequency precoding is essential to jointly mitigate the interference across each dimension and minimize space-time-frequency interference
% optimal performance (\inred{Zhbin: Include what criteria} \note{SINR}) 
at a low computational complexity. 
% While optimal spatial precoding can be achieved at the transmitter by Dirty Paper Coding \cite{CostaDPC1983}, it incurs high computational complexity as the number of antennas and users increases and relies on the availability of 
% 
\note{``Joint space-time-freqency precoding does not exist", and existing techniques treat them as separate problems typically at Tx for space and Rx for time-frequency.  An example solution here is to exploit a higher dimensional decomposition technique (maybe some form of higher-order KLT or SSA) and attempt to achieve space-time-frequency interference-free communication, by enforcing some form of orthogonality or diagonal matrices in the preceded signals. In OFDM we are mostly interested in correcting the ICI that arises from doppler spreads in time-varying channels, and in MIMO we need spacial interference removal. If we employ proper Cyclic Prefix according to the multipath fading environment we may be able to combat most ISI, but it becomes trickier in NS channels. 
}


Figure \ref{fig:Df} shows the data flow from transmitter to receiver.
% \textbf{Unified Characterization:}
The space-time-frequency CSI is obtained from the receivers and accumulated into a 4-dimensional channel kernel. 
% The spatio-temporal CSI for MU-MIMO OFDM is given by $\mathcal{H}_{N \times N_{FFT} \times N_{t} \times N_{r} \times N_{u}}$, where $N$, $N_{FFT}$, $N_{t}, N_{r}, N_{u}$ are the number of time samples and OFDM subcarriers respectively. 
The core of our method is the unified characterization of the channel by a novel higher dimensional decomposition of this kernel, which for non-stationary channels, results in space-time-frequency eigenfunctions that are jointly orthogonal independently and jointly across each dimension, and are central to the precoding method to cancel the interference across space-time-frequency domains. 
By definition, eigenfunctions are constituent time series of the CSI that only undergo a scaling when transmitted over channel. Hence, precoding (across subcarriers \cite{}) using those yields interference-free and flat fading at the receiver. 
% However, while extracting accurate eigenfunctions may lead to optimal precoding, a significant drawback of this method is its extremely high computational complexity to extract large number of eigenfunctions at each time step that makes it impractical \cite{}. We address this with Autoencoder for computational efficiency, generality and adaptability.
% While extracting accurate eigenfunctions may lead to optimal precoding, it is often impractical due to the high computational complexity and the availability of limited CSI at the transmitter \cite{}. 
% Therefore, we rely on a

% \textbf{Joint space-time precoding:}
Joint space-time-frequency precoding at the transmitter %of symbols to be transmitted 
involves combining the extracted eigenfunctions with optimal coefficients (that ensure minimum interference). These coefficients are extracted as those that minimize the L2-norm between the projection of the CSI onto its extracted eigenfunctions (which results in eigenvalues) and the symbols to 
be transmitted. Finally, the precoded symbols are divided/ scheduled to each user and are processed through the conventional OFDM blocks (S/P, IFFT, P/S, CP insertion etc.) before transmission.
% \vspace{3in}
% 
Therefore, we make the following contributions:
\begin{enumerate}
    \item We propose a novel generalized method to decompose the NS channel kernel into its eigenfunctions and we derive a unified characterization of any wireless channel by \note{explaining or extracting} its statistics.
    % \item We propose a generalized Mercer's theorem showing the singular value decomposition for the NS channel kernel and gives the eigenfunctions explanation for the NS channel statistics (Section \ref{sec:NSdec}).
    \item We design a novel joint space-time precoding method for NS channels, which mitigates the interference across space, time and joint space-time domain to approach minimum BER performance at the receiver (Section \ref{sec:Precoding})\footnote{This can be extended to space-time-frequency by considering the frequency dimension.}.
    % \item We design a generalized joint space-time interferece precoding method for NS channel, which approaches optimal performance across space-time-frequency at a low computational complexity. To our best knowledge, this is the first precoding technique for NS channel (Section \ref{sec:Precoding}).
    % \item We design an Autoencoder (AE) to extract accurate space-time-frequency eigenfunctions of the channel with low computational complexity (Section \ref{sec:AE}).
    % \item Through extensive theoretical analysis, we show that our precoding approach outperforms the SoTA for NS channels, while approaching the performance of SoTA for stationary channels.
    \item Through extensive theoretical analysis and practical simulations, we show the accuracy of the proposed unified channel characterization and joint space-time precoding compared to existing methods.
\end{enumerate}
% 1. 
% 2. We use the eigenfunctions to propose a novel joint/combined IUI+ICI+ISI precoding that achieves the performance of multiple SoTA techniques combined, but at a lower complexity.

% \note{NS channel precoding is unprecedented in the literature \cite{AliNS0219} and is quite challenging as the CSI/ channel distribution and its statistics are functions of time, which necessitate latent representations that are also functions of time and capture the NS change in the statistics (\eg eigenfunctions). However, extracting such eigenfunctions is computationally prohibitive, especially when the channel statistics change rapidly, and for higher dimensional channels (i.e, when there are additional degrees of freedom, like multiple frequency subcarriers in OFDM, large number of antennas in massive/ XL MIMO, or large number of users in MU-MIMO). Therefore, we need computationally tractable methods to extract such eigenfunctions and effectively jointly precode across space-time-frequency to approach interference-free communication at the receiver.}
\end{comment}

\begin{comment}
Multiple-Input Multiple-Output (MIMO) communications and its variants (MU-MIMO, Massive/ XL MIMO) have emerged as promising technologies to achieve the network capacity, efficiency, and reliability required to accommodate the exponential growth in connected devices and network traffic.
These gains are realized through the ability of MIMO-OFDM communications to achieve higher diversity across multiple degrees of freedom; space (users/ antennas), frequency and time.
% As one of the most promising wireless communication solutions, multiple-input multiple-output (MIMO) technology has been widely used in IEEE 802.11ac/n (WiFi), IEEE 802.16e (WiMAX), LTE/LTE-A (4G), and other protocols and systems [1].
However, achieving these gains require interference-free communication in all degrees of freedom (i.e., orthogonality of transmissions across space-time-frequency).
Therefore, the central challenge in MIMO transceiver design is to achieve IUI (Inter-User Interference), IAI (Inter-Antenna Interference), ICI (Inter-Carrier Interference) and ISI (Inter-Symbol Interference) free communication at the receiver.
\end{comment}

\begin{comment}
\inred{
\note{\textbf{Contributions:}\\
1. Decomposition of NS channels.\\
2. Design an autoencoders for computationally efficient and generalized decomposition of the channel (non-stationary) into KLT eigenfunctions.\\
3. Precoding for NS channels.
}

\noindent
What is the contribution and \textbf{why exactly are we seeing a gain}.\\
For time-varying channel, using KLT decomposition to achieve space-time-frequency jointly orthogonal eigenfunctions, by which we design precoding method to cancel IUI, ISI and ICI.

Why is it better than SoTA (for NS channels)\\

The special of eigenfunctions: If we have a flat fading channel H, we can transmit data through the orthogonal space of the channel to cancel ISI. We know any channel can be represented by orthogonal sine waves. So we can transmit data trough frequency space, which is OFDM. but when it comes to delay-Doppler time-varying channels. There will be interferences at frequency space. So we can find eigenfunctions jointly orthogonal at time-frequency space to cancel both ISI can ICI. Expand it to space, eigenfunctions can jointly orthogonal at space-time-frequency domain.

The paper~\ref{} showed eigenfunctions are optimal to cancel interference but impractical. \ref{} gives a OTFS modulation aim to cancel ISI and ICI. 

Not sure benefits for NS channels.
}
\end{comment}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD INTRO %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\newpage
Precoding at the transmitter is investigated in the literature and is relatively tractable when the wireless channel is stationary, by employing the gamut of linear algebraic and statistical tools to ensure interference-free communication \cite{}. However, there are many instances, in modern and next Generation (xG) propagation environments such as mmWave, V2X, and massive-MIMO networks, where %the distribution of 
the channel is %either partially observed, undefined, non-linear, higher dimensional or 
statistically non-stationary \cite{} (the distribution is a function of time). 
The lack of accurate models/ characterization especially for non-stationary channels \cite{}, leads to sub-optimal and sometimes catastrophic performance even with state-of-the-art precoding \cite{AliNS0219}. 
The time-varying channel distribution and statistics, necessitates a decomposition (for precoding) that is a function of time (\eg eigenfunctions), but also preserves orthogonality across domains to ensure interference-free communication. 
% However, extracting such eigenfunctions is computationally prohibitive, especially when the channel statistics change rapidly, and for higher dimensional channels (i.e, when there are additional degrees of freedom, like multiple frequency subcarriers in OFDM, large number of antennas in massive/ XL MIMO, or large number of users in MU-MIMO). Therefore, we need computationally tractable methods to extract such eigenfunctions and effectively jointly precode across space-time-frequency to approach interference-free communication at the receiver.
% 
Furthermore, in communication systems that leverage multiple degrees of freedom (space (users/ antennas), frequency or time, \eg MU-MIMO or OFDM), the existence of interference in each or across multiple dimensions, necessitates novel precoding methods that ensure orthogonality of the transmitted signals across each dimension/ plane to ensure interference-free communication. 
% achieving these gains require interference-free communication in all degrees of freedom (i.e., orthogonality of transmissions across space-time-frequency).
% The lack of accurate models/ characterization especially for such non-stationary channels \cite{} and the inability to cancel interference that occurs simultaneously across multiple degrees of freedom leads to sub-optimal and sometimes catastrophic performance even with state-of-the-art precoding \cite{}.
% This leads to sub-optimal and sometimes catastrophic performance even with state-of-the-art precoding \cite{}, due to the lack of accurate models especially for non-stationary channels \cite{} and teh 
% These gains are realized through the ability of MIMO-OFDM communications to achieve higher diversity across multiple degrees of freedom; space (users/ antennas), frequency and time.
% As one of the most promising wireless communication solutions, multiple-input multiple-output (MIMO) technology has been widely used in IEEE 802.11ac/n (WiFi), IEEE 802.16e (WiMAX), LTE/LTE-A (4G), and other protocols and systems [1].
% Therefore, precoding for non-stationary channels  interference-free communication in all degrees of freedom (i.e., orthogonality of transmissions across space-time-frequency).
% Therefore, the central challenge in MIMO transceiver design is to achieve IUI (Inter-User Interference), IAI (Inter-Antenna Interference), ICI (Inter-Carrier Interference) and ISI (Inter-Symbol Interference) free communication at the receiver.
% 


\note{Optimal mitigation of such interference, necessitates pre-processing at the transmitter using Dirty Paper Coding (DPC) \cite{CostaDPC1983} across space-time-frequency dimensions, however it is often impractical as it requires both perfect and complete (up-to-date) Channel State Information (CSI) at the transmitter and incurs a high computational complexity that increases with the number of users and receive antennas.}
This is especially challenging in practical propagation environments where the channel is high dimensional (\eg MU-MIMO, Massive/ XL MIMO) and both time varying and frequency selective (doubly dispersive \cite{}), where only occasional or statistical CSI is available at transmitter. 
Therefore, existing precoding %in the literature 
typically treat these as separate problems, where spatial precoding at the transmitter attempts to mitigate inter-user and inter-antenna interference, while equalization at the receiver attempts to mitigate inter-carrier and inter-symbol interference.
% 
% Optimal spatial precoding techniques exploit DPC across users, and are typically infeasible for practical adoption due to the high complexity (especially in MU/ Massive MIMO). %especially as the number of users or antennas increase (in MU/ Massive MIMO), 
% while linear precoding techniques are sub-optimal \cite{}.
% On the other hand, adaptive time-frequency equalization at the receiver add computational burden to receivers and are sub optimal compared to transmit pre-processing \cite{}. 
% 
Therefore, we believe that space-time-frequency precoding is essential to jointly mitigate the interference across each dimension and minimize space-time-frequency interference
% optimal performance (\inred{Zhbin: Include what criteria} \note{SINR}) 
at a low computational complexity. 
% While optimal spatial precoding can be achieved at the transmitter by Dirty Paper Coding \cite{CostaDPC1983}, it incurs high computational complexity as the number of antennas and users increases and relies on the availability of 
% 
\note{``Joint space-time-freqency precoding does not exist", and existing techniques treat them as separate problems typically at Tx for space and Rx for time-frequency.  An example solution here is to exploit a higher dimensional decomposition technique (maybe some form of higher-order KLT or SSA) and attempt to achieve space-time-frequency interference-free communication, by enforcing some form of orthogonality or diagonal matrices in the preceded signals. In OFDM we are mostly interested in correcting the ICI that arises from doppler spreads in time-varying channels, and in MIMO we need spacial interference removal. If we employ proper Cyclic Prefix according to the multipath fading environment we may be able to combat most ISI, but it becomes trickier in NS channels. 
}

\end{comment}

\begin{comment}
Figure \ref{fig:Df} shows the data flow from transmitter to receiver.
% \textbf{Unified Characterization:}
The space-time-frequency CSI is obtained from the receivers and accumulated into a 4-dimensional channel kernel. 
% The spatio-temporal CSI for MU-MIMO OFDM is given by $\mathcal{H}_{N \times N_{FFT} \times N_{t} \times N_{r} \times N_{u}}$, where $N$, $N_{FFT}$, $N_{t}, N_{r}, N_{u}$ are the number of time samples and OFDM subcarriers respectively. 
The core of our method is the unified characterization of the channel by a novel higher dimensional decomposition of this kernel, which for non-stationary channels, results in space-time-frequency eigenfunctions that are jointly orthogonal independently and jointly across each dimension, and are central to the precoding method to cancel the interference across space-time-frequency domains. 
By definition, eigenfunctions are constituent time series of the CSI that only undergo a scaling when transmitted over channel. Hence, precoding (across subcarriers \cite{}) using those yields interference-free and flat fading at the receiver. 
% However, while extracting accurate eigenfunctions may lead to optimal precoding, a significant drawback of this method is its extremely high computational complexity to extract large number of eigenfunctions at each time step that makes it impractical \cite{}. We address this with Autoencoder for computational efficiency, generality and adaptability.
% While extracting accurate eigenfunctions may lead to optimal precoding, it is often impractical due to the high computational complexity and the availability of limited CSI at the transmitter \cite{}. 
% Therefore, we rely on a

% \textbf{Joint space-time precoding:}
Joint space-time-frequency precoding at the transmitter %of symbols to be transmitted 
involves combining the extracted eigenfunctions with optimal coefficients (that ensure minimum interference). These coefficients are extracted as those that minimize the L2-norm between the projection of the CSI onto its extracted eigenfunctions (which results in eigenvalues) and the symbols to 
be transmitted. Finally, the precoded symbols are divided/ scheduled to each user and are processed through the conventional OFDM blocks (S/P, IFFT, P/S, CP insertion etc.) before transmission.
% \vspace{3in}
% 
Therefore, we make the following contributions:
\begin{enumerate}
    \item We propose a novel generalized method to decompose the NS channel kernel into its eigenfunctions and we derive a unified characterization of any wireless channel by \note{explaining or extracting} its statistics.
    % \item We propose a generalized Mercer's theorem showing the singular value decomposition for the NS channel kernel and gives the eigenfunctions explanation for the NS channel statistics (Section \ref{sec:NSdec}).
    \item We design a novel joint space-time precoding method for NS channels, which mitigates the interference across space, time and joint space-time domain to approach minimum BER performance at the receiver (Section \ref{sec:Precoding})\footnote{This can be extended to space-time-frequency by considering the frequency dimension.}.
    % \item We design a generalized joint space-time interferece precoding method for NS channel, which approaches optimal performance across space-time-frequency at a low computational complexity. To our best knowledge, this is the first precoding technique for NS channel (Section \ref{sec:Precoding}).
    % \item We design an Autoencoder (AE) to extract accurate space-time-frequency eigenfunctions of the channel with low computational complexity (Section \ref{sec:AE}).
    % \item Through extensive theoretical analysis, we show that our precoding approach outperforms the SoTA for NS channels, while approaching the performance of SoTA for stationary channels.
    \item Through extensive theoretical analysis and practical simulations, we show the accuracy of the proposed unified channel characterization and joint space-time precoding compared to existing methods.
\end{enumerate}
% 1. 
% 2. We use the eigenfunctions to propose a novel joint/combined IUI+ICI+ISI precoding that achieves the performance of multiple SoTA techniques combined, but at a lower complexity.

% \note{NS channel precoding is unprecedented in the literature \cite{AliNS0219} and is quite challenging as the CSI/ channel distribution and its statistics are functions of time, which necessitate latent representations that are also functions of time and capture the NS change in the statistics (\eg eigenfunctions). However, extracting such eigenfunctions is computationally prohibitive, especially when the channel statistics change rapidly, and for higher dimensional channels (i.e, when there are additional degrees of freedom, like multiple frequency subcarriers in OFDM, large number of antennas in massive/ XL MIMO, or large number of users in MU-MIMO). Therefore, we need computationally tractable methods to extract such eigenfunctions and effectively jointly precode across space-time-frequency to approach interference-free communication at the receiver.}

Multiple-Input Multiple-Output (MIMO) communications and its variants (MU-MIMO, Massive/ XL MIMO) have emerged as promising technologies to achieve the network capacity, efficiency, and reliability required to accommodate the exponential growth in connected devices and network traffic.
These gains are realized through the ability of MIMO-OFDM communications to achieve higher diversity across multiple degrees of freedom; space (users/ antennas), frequency and time.
% As one of the most promising wireless communication solutions, multiple-input multiple-output (MIMO) technology has been widely used in IEEE 802.11ac/n (WiFi), IEEE 802.16e (WiMAX), LTE/LTE-A (4G), and other protocols and systems [1].
However, achieving these gains require interference-free communication in all degrees of freedom (i.e., orthogonality of transmissions across space-time-frequency).
Therefore, the central challenge in MIMO transceiver design is to achieve IUI (Inter-User Interference), IAI (Inter-Antenna Interference), ICI (Inter-Carrier Interference) and ISI (Inter-Symbol Interference) free communication at the receiver.
\end{comment}

\begin{comment}
\inred{
\note{\textbf{Contributions:}\\
1. Decomposition of NS channels.\\
2. Design an autoencoders for computationally efficient and generalized decomposition of the channel (non-stationary) into KLT eigenfunctions.\\
3. Precoding for NS channels.
}

\noindent
What is the contribution and \textbf{why exactly are we seeing a gain}.\\
For time-varying channel, using KLT decomposition to achieve space-time-frequency jointly orthogonal eigenfunctions, by which we design precoding method to cancel IUI, ISI and ICI.

Why is it better than SoTA (for NS channels)\\

The special of eigenfunctions: If we have a flat fading channel H, we can transmit data through the orthogonal space of the channel to cancel ISI. We know any channel can be represented by orthogonal sine waves. So we can transmit data trough frequency space, which is OFDM. but when it comes to delay-Doppler time-varying channels. There will be interferences at frequency space. So we can find eigenfunctions jointly orthogonal at time-frequency space to cancel both ISI can ICI. Expand it to space, eigenfunctions can jointly orthogonal at space-time-frequency domain.

The paper~\ref{} showed eigenfunctions are optimal to cancel interference but impractical. \ref{} gives a OTFS modulation aim to cancel ISI and ICI. 

Not sure benefits for NS channels.
}
\end{comment}

==> intro_old.tex <==
\section{Introduction}
\label{sec:intro}
\vspace{-5pt}
%Although there has been tremendous interest in the design of Neural Network based transceivers in the literature, their practical adoption has been limited due to a lack of explainability and performance guarantees on the error rate or the complexity (training or hardware complexity). 
Deep Learning (DL) has been shown to be a versatile tool for physical layer communication due to its proficiency in systems with model and algorithm deficit \cite{simeone2018very}, and has been used to replace individual blocks in communication systems for optimized performance for a given dataset. 
% Deep Learning (DL) has been shown to be a versatile tool for physical layer communication due to its proficiency in systems with model and algorithm deficit \cite{simeone2018very}, and has been used to replace individual blocks in communication systems for optimized performance for a given dataset. 
% Recent developments in this area leverage the underlying physics, causal structures, recurrent behaviors, transfer learning and human interpretability (explainable AI or XAI~\cite{xai,xai_1,beaudouin2020flexible,chen2020adaptive}), to move away from a \textit{black box} approach to employing DL. 
However, much of the effort have focused on training neural networks as black-box systems that lack guarantees on their performance and model complexity, and have at best approaching the error rate of classical (non-DL) methods \cite{kim2018communication,gruber2017deep}.
These often require %lead NN-based receivers that incur 
prohibitive amount of training and computational resources \cite{wang2017deep,HeModelDrivenComms} that limit their practical adoption. 
% to achieve a target classification error (symbol detection is a multidimensional classification problem) for a specific dataset, 
% and lack guarantees on their error rate, model complexity and training time, which has limited their practical adoption.  
% However, these benefits come at the cost of increased training time and model complexity and have at best approached the error rate of classical (non-DL) methods \cite{kim2018communication,gruber2017deep}. 
The stringent requirements on reliability and throughput in Next Generation (xG) propagation environments demand wireless transceivers to achieve provable performance guarantees over a variety of channels. 
% Fueled by the promising results shown in other domains, wireless researchers have adopted a learning based approach in order to tame the stochasticity of the wireless channel. 
% So far, much of the effort has been focused on training neural networks as black-box systems to achieve a target classification error (symbol detection is a multidimensional classification problem) for a specific dataset, and lack guarantees on their error rate, model complexity and training time, which has limited their practical adoption.  
% In order to achieve provable guarantees for NN-based receivers
Therefore, \textit{explaining} how an NN-based receiver detects symbols (generally a multidimensional classification problem) is paramount to achieve such guarantees \cite{guo2020explainable6G} while providing insights on amount of required training and robustness to different signal configurations and channels.
% Therefore, \textit{explaining} the internal mechanisms of NN-based receivers is paramount to achieve %provable performance 
% such guarantees \cite{guo2020explainable6G}
% % and understand the limitations of such systems \cite{guo2020explainable6G} 
% while providing insights into amount of training required and its robustness to different signal configurations and propagation environments. %beyond the training data.
% Therefore, \textit{explaining} how a NN-based receivers classifies symbols () is paramount to achieve %provable performance 
% such guarantees \cite{guo2020explainable6G}
% and understand the limitations of such systems \cite{guo2020explainable6G} 
% while providing insights into amount of training required and its robustness to different signal configurations and propagation environments. %beyond the training data.
% generating representative datasets and end-to-end training of neural networks to achieve a target classification error (symbol detection is a general multidimensional classification problem). 
% Therefore, 
%
In order to achieve this goal, %explain the internal mechanisms of NN-based receivers, these 
two things should be mathematically and semantically understood: 1) A measure of the knowledge acquired by the NN-based receiver and 2) Bounds on learnability (or error) of the neural network model used for signal processing. 
Due to the difficulty of explaining the behaviour of neural networks in high-dimensional stochastic systems like wireless channels~\cite{simeone2018very,tjoa2020survey}, we have to define an equivalent NN-based receiver that eventually performs the same optimization as a classical symbol detector, which is optimal for stationary channel distributions with a known mathematical model \cite{Proakis2007Book}.  %when there exists a ma stationary and know channels.
% Due to the difficulty of explaining the behaviour of neural networks in high-dimensional stochastic systems like wireless channels~\cite{tjoa2020survey}, we have to define an equivalent NN-based receiver that eventually performs the same optimization as a classical symbol detector, which is known to be optimal for AWGN channels.
% Due to the difficulty of explaining the behaviour of neural networks in high-dimensional stochastic systems like wireless channels~\cite{tjoa2020survey}, %in order to make NN-based receiver (denoted by {\tnn}) explainable, 
% we have to define an %first set a \note{baseline understanding} 
% equivalent %of what happens inside the 
% NN-based receiver that eventually performs the same optimization as a classical symbol detector, which is known to be optimal for AWGN channels.
% Therefore, in order to make NN-based receiver (denoted by {\tnn}) explainable, we have to set a baseline understanding of what happens inside the neural network that eventually performs the exact same optimization as in a classical receiver (denoted by {\tmap}).
% These fixed function ``black-box" implementations that fit a particular dataset cannot be generalized to other scenarios, unless these two things are mathematically and semantically understood: 1) A \textit{measure} of the knowledge acquired by the neural network receiver and 2) Bounds on \textit{learnability} (or error) of the neural network model used for processing the signal. In order to make NN-based receiver explainable, we have to set a baseline understanding of what happens inside the neural network that eventually performs the exact same optimization as in a classical receiver. 
The key to establishing this \textit{equivalence}, shown in figure~\ref{fig:whole}, is deriving the risk function and other structural criteria of the NN-based receiver {\tnn} that eventually leads to the error performance of classical symbol detector {\tmap}.
% , \note{under the availability of training data that is representative of the entire channel distribution.}
% The key to establish equivalence is the derivation of the risk function of the NN-based receiver, \note{under the availability of training data that is representative of the entire channel distribution.}
% This equivalent receiver is referred to as {\tnn}.
% 
% The stringent requirements on reliability and achievable throughput in xG propagation environments demand wireless communication systems that achieve provable performance guarantees over a variety of channels. 
% Although there has been tremendous interest in the design of NN-based transceivers in the literature, their pracical adaptation have been limited due to their lack of explainability and performance guarantees on the error rate or the complexity (training or hardware complexity). 
% Therefore, a single feedforward neural network ach
This serves as the much-needed theoretical evidence on the similarity in the performance of NN-based and classical receivers %when a channel model exists, 
that can be the stepping stone towards corroborating the efficacy and limitations of NN-based transceivers in different channel conditions. % applications.
% Moreover, this provides the cri
% Moreover, this allows 
% Moreover, 
% Moreover, we show that the equivalent 
% We further show that the equivalent {\tnn} receiver is robust to data that is not seen during training, and allows us to derive bounds even 
% We show that 
Such an equivalent {\tnn} receiver is not only robust to data that is not seen during training but also reduces the amount of training and leads to performance guarantees even when trained on channels with unknown distribution. 
% This allows for the implementation of classical receivers using equivalent deep feed forward neural networks that are computationally tractable. 
% Moreover, explaining the internal mechanisms of NN-based receivers provides insights into the amount of training required, the robustness to different signal configurations and propagation environments beyond the training data.  

\begin{figure}%[t]
        \centering
		\includegraphics[width=0.48\textwidth]{figures/whole_systemFF.pdf}  %{FullSystemFFF.pdf}
% 		\vspace{-30pt}
        \caption{Equivalence between {\tnn} and {\tmap} receivers
        }   %IMAGE MUST BE MODIFIED
        \label{fig:whole}
    \vspace{-20pt}   
\end{figure}
% \begin{figure}
%         \centering
%         \begin{subfigure}{0.39\textwidth}
% 		\includegraphics[width=\textwidth]{figures/System_Diagram.pdf}
%                 \caption{Block structure of {\tmap} and the wireless channel}%Constellation before pre-compensation
%                 \label{fig:T_MAP}
%         \end{subfigure}\\% 
%         % \quad
%         \begin{subfigure}{0.4\textwidth}
%                 \includegraphics[width=\textwidth]{figures/NNReceiver.pdf}
%                 \caption{Structure of {\tnn} to achieve equivalence with {\tmap}}%Constellation after pre-compensation
%                 \label{fig:T_NN}
%         \end{subfigure}
% 	\caption{Equivalent receivers of {\tnn} and {\tmap} (Change).}
% 	\label{fig:whole}
% % 	\vspace{-10pt}
% \end{figure}


% Establishing %\note{baseline} a 
% equivalence will allow us to 
% quantify the disparity between NN-based and classical receivers even when the training data is not representative of the entire channel distribution.
% % \note{Quantifying}
% this disparity is central to deriving mathematically tight data-dependent bounds on their error rate. % of NN-based receivers.
% Establishing %\note{baseline} a 
The risk function of the {\tnn} derived for equivalence also serves as a measure of the disparity between NN-based and classical receivers, %, when training  %when the tr 
% even when the training data is not representative of the entire channel distribution.
% \note{Quantifying}
that is central to deriving mathematically tight data-dependent bounds on its error rate. % of NN-based receivers.
Unlike previous literature, this provides a means to evaluate the best and worst case performance of such receivers before field testing or practical implementation.
% Moreover, these 
Moreover, this information allows us to empirically determine the structure of {\tnn} that approach the error rate of {\tmap}, even under incomplete training.
% These bounds can lead to strict guarantees on the fidelity of communication and complexity, that are critical towards meeting the reliability and throughput requirements in existing and xG networks. % including mission critical application.
This allows for the implementation of practical receivers using data-driven, low-complexity NN structures that is both computationally efficient and robust to the underlying channel. %that adapt to the propagation environment.  %that are computationally tractable 
Therefore, this work enables implementation of tractable NN-based receivers with guaranteed error rate and model complexity, which is critical to meet the reliability and throughput requirements in existing and xG networks. % including mission critical application.
%various channel and signal configurations.
% Therefore, we take the first step towards explaining the behaviour of NN-based receivers, that is capable of achieving provable performance guarantees under various channel and signal configurations.








\begin{comment}
%Although there has been tremendous interest in the design of Neural Network based transceivers in the literature, their practical adoption has been limited due to a lack of explainability and performance guarantees on the error rate or the complexity (training or hardware complexity). 
Deep Learning (DL) has been shown to be a versatile tool for physical layer communication due to its proficiency in systems with model and algorithm deficit \cite{simeone2018very}, and has been used to replace individual blocks in communication systems for optimized performance for a given dataset. 
% Recent developments in this area leverage the underlying physics, causal structures, recurrent behaviors, transfer learning and human interpretability (explainable AI or XAI~\cite{xai,xai_1,beaudouin2020flexible,chen2020adaptive}), to move away from a \textit{black box} approach to employing DL. 
However, these benefits come at the cost of increased training time and model complexity and have at best approached the error rate of classical (non-DL) methods \cite{kim2018communication,gruber2017deep}. 
The stringent requirements on reliability and achievable throughput in xG propagation environments demand wireless transceivers that achieve provable performance guarantees over a variety of channels. 
% Fueled by the promising results shown in other domains, wireless researchers have adopted a learning based approach in order to tame the stochasticity of the wireless channel. 
So far, much of the effort has been focused on generating representative datasets and end-to-end training of neural networks to achieve a target classification error (symbol detection is a general multidimensional classification problem). 
These fixed function ``black-box" implementations that fit a particular dataset cannot be generalized to other scenarios, unless these two things are mathematically and semantically understood: 1) A \textit{measure} of the knowledge acquired by the neural network receiver and 2) Bounds on \textit{learnability} (or error) of the neural network model used for processing the signal. In order to make %\note{wireless communications} 
NN-based receiver explainable, we have to set a baseline understanding of what happens inside the neural network that eventually performs the exact same optimization as in a classical receiver. 
The key to establish equivalence is the derivation of the risk function of the NN-based receiver, \note{under the availability of training data that is representative of the entire channel distribution.}
% This equivalent receiver is referred to as {\tnn}.
% 
% The stringent requirements on reliability and achievable throughput in xG propagation environments demand wireless communication systems that achieve provable performance guarantees over a variety of channels. 
% Although there has been tremendous interest in the design of NN-based transceivers in the literature, their pracical adaptation have been limited due to their lack of explainability and performance guarantees on the error rate or the complexity (training or hardware complexity). 
% Therefore, a single feedforward neural network ach
This serves as the much-needed theoretical evidence of the similarity in the performance of NN-based and classical receivers, that \note{is the or can be the} stepping stone towards corroborating the \note{use-cases or efficacy} and limitations of \note{learning-based or NN-based transceivers} in wireless communications. % applications.
% This allows for the implementation of classical receivers using equivalent deep feed forward neural networks that are computationally tractable. 
Moreover, explaining the internal mechanisms of NN-based receivers provides insights into the amount of training required, the robustness to different signal configurations and propagation environments beyond the training data.  

\begin{figure}%[t]
        \centering
		\includegraphics[width=0.48\textwidth]{figures/whole_systemFF.pdf}  %{FullSystemFFF.pdf}
% 		\vspace{-30pt}
        \caption{Equivalence between {\tnn} and {\tmap} receivers
        }   %IMAGE MUST BE MODIFIED
        \label{fig:whole}
    \vspace{-20pt}   
\end{figure}
% \begin{figure}
%         \centering
%         \begin{subfigure}{0.39\textwidth}
% 		\includegraphics[width=\textwidth]{figures/System_Diagram.pdf}
%                 \caption{Block structure of {\tmap} and the wireless channel}%Constellation before pre-compensation
%                 \label{fig:T_MAP}
%         \end{subfigure}\\% 
%         % \quad
%         \begin{subfigure}{0.4\textwidth}
%                 \includegraphics[width=\textwidth]{figures/NNReceiver.pdf}
%                 \caption{Structure of {\tnn} to achieve equivalence with {\tmap}}%Constellation after pre-compensation
%                 \label{fig:T_NN}
%         \end{subfigure}
% 	\caption{Equivalent receivers of {\tnn} and {\tmap} (Change).}
% 	\label{fig:whole}
% % 	\vspace{-10pt}
% \end{figure}


Establishing \note{baseline} a equivalence will also %allow us to 
quantify the disparity between NN-based and classical receivers even when the training data is not representative of the entire channel distribution.
\note{Quantifying} this disparity is central to deriving mathematically tight data-dependent bounds on their error rate. % of NN-based receivers.
Unlike previous literature, this provides a means to evaluate the best and worst case performance of such receivers before field testing or practical implementation.
These bounds lead to strict guarantees on the fidelity of communication and complexity, that are critical towards meeting the reliability and throughput requirements in existing and xG networks. % including mission critical application.
% Moreover, these 
Furthermore, this information is used to empirically determine the structure of the NN-based receiver that approach the error rate of classical receivers, even under incomplete training.
This allows for the implementation of practical receivers using data-driven, low-complexity NN structures that is robust to the underlying channel. %that adapt to the propagation environment.  %that are computationally tractable 
Therefore, this work serves as the foundation, towards designing tractable data-driven transceivers that can achieve target guarantees in %communication 
error rate and model complexity over various channel and signal configurations.
% Therefore, we take the first step towards explaining the behaviour of NN-based receivers, that is capable of achieving provable performance guarantees under various channel and signal configurations.
\end{comment}



% \note{This allows us to theoretically corroborate that NN-based receivers approach the error rate of optimal classical receivers when a mathematical channel model exists, and outperform classical receivers when a channel model does not exist. 
% Moreover, NN-based receivers are computationally tractable over a variety of channels.}
 
% \note{Why is equivalence important. How is it achieved. What does this lead to. What can be done using this knowledge.}

% \noindent
% 1. Emerging communication systems (xG) require transceivers that achieve strict guarantees.\\
% 2. Unfortunately all existing NN based transceivers lack such guarantees which has prevented their wide-spread adoption in practical systems.\\
% 3. The first step towards achieving guarantees is to explain the internal mechanisms of a NN-based transceiver, that eventually performs the exact same optimizations as the classical transceivers.\\
% 4. Establishing this baseline equivalence, allows us to determine the disparity between NN-based and classical approaches even when the training data is not representative of the entire channel distribution.\\
% 5. This information is used to derive tight data-dependent bounds on the error rate of practical NN-based receivers, which consequently leads to guarantees on the fidelity of communication (\eg reliability and achievable throughput) and complexity (hardware and training). \\
% 6. This work is the first step towards the design of optimal data-driven communication systems that can achieve target guarantees in communication and complexity. 


% \begin{itemize}
%     % \item Showing that {\tnn} and {\tmap} are equivalent.
%     % \item Derive the complexity penalty of NNs to minimize the generalization error of {\tnn}.
%     \item Theoretically proving that a feed forward deep NN-based receiver with the MSE loss function is probabilistically equivalent to the optimal MAP receiver, under complete training and a sufficiently rich data-set, without requiring any prior knowledge of channel statistics.
%     \item We show that for a finite training data-set, the average testing loss of the NN-based receiver is distributed as a Gaussian.
%     \item We derive tight upper and lower bounds on the Bit Error Rate (BER) of the NN-based receiver as a function of average testing loss and the number of training samples.
%     \item Practical evaluation using a simulation framework to corroborate the accuracy of the proposed interpretation and bounds and compare the performance of NN-based and classical receivers over a variety of channels.
%     % \item Derive the loss functions of NNs to achieve equivalence of {\tnn} and {\tmap}.
%     % \item Derive bounds on the performance of {\tnn} for BER and complexity.
%     % % \item Derive the structure of {\tnn} to achieve equivalence with {\tmap}.
%     % \item Practical evaluation using a simulation framework to show the equivalence of {\tnn} and {\tmap}.
%     % % \item Derive the complexity penalty of NNs to minimize the generalization error of {\tnn}.
% \end{itemize}














\begin{comment}


% \note{
% An optimal receiver using conventional communication theory strives to maximize the posterior probability to estimate the most likely transmitted symbol 
% %$\hat { m } = \underset { 1 \leq m \leq M } { \arg \max }_m\  \mathrm { P } \left[ \boldsymbol {s_m } | \boldsymbol {r} \right]$ 
% $\hat { m } = { \arg \max }_m\  \mathrm { P } \left[ \boldsymbol {s_m } | \boldsymbol {r} \right]$
% or the likelihood under the assumption of equal prior, 
% %$\hat { m } = \underset { 1 \leq m \leq M } { \arg \max }\  \mathrm { P } ( \boldsymbol { r } | \boldsymbol { s_m } )$, where, $\boldsymbol{r}$ 
% $\hat { m } = { \arg \max }_m\  \mathrm { P } ( \boldsymbol { r } | \boldsymbol { s_m } )$, where, $\boldsymbol{r}$ 
% is the received symbol for the transmitted symbol, $\boldsymbol{s_m}$. 
%These methods are designed to extract certain parameters of the channel PDF that assist in setting the noise boundaries during the maximum likelihood decoding. 
% While it is desirable to learn and predict the channel at the transmitter to achieve capacity using Dirty Paper Coding (DPC)~\cite{DPC_Costa}, it is a non-trivial problem in practice~\cite{thp_partial,dpc_lpc,precodingParticle,TomlinsonHarashima_Analysis,TomlinsonHarashima_Quantized}. Wireless channels are influenced by many external variables that are often correlated, time-dependant or unknown. Therefore, any acquired knowledge about these factors is inevitably ephemeral, requiring learning models that are fast, adaptive and evolve with time. 

The entire apparatus for error free decoding at the receiver in conventional communication theory relies on modeling the Probability Distribution Function (PDF) of the likelihood as Gaussian with zero mean and a constant variance, which leads to the optimal nearest neighbor decoding that is widely used in modern communication systems. This symbol detection problem is relatively tractable and has been studied in the literature for linear, stationary channels with normal distribution by employing the gamut of mathematical tools for Bayesian inference. 
However, there are many cases, such as observed in ne\underline{x}t \underline{G}eneration (xG) mmWave, V2X, and massive-MIMO networks 
where the PDF of the likelihood is either partially observed, undefined, non-linear, highly dimensional or non-stationary that leads to sub-optimal and sometimes catastrophic performance even with the state-of-the-art receiver signal processing. 

Deep Learning (DL) has emerged as a versatile tool for physical layer communication due to its proficiency in systems with model and algorithm deficit \cite{simeone2018very}, and has been used to replace individual blocks in communication systems for optimized performance for a given dataset. 
% Recent developments in this area leverage the underlying physics, causal structures, recurrent behaviors, transfer learning and human interpretability (explainable AI or XAI~\cite{xai,xai_1,beaudouin2020flexible,chen2020adaptive}), to move away from a \textit{black box} approach to employing DL. 
However, these benefits come at the cost of increased training time and model complexity and have at best approached the error rate of classical (non-DL) methods \cite{kim2018communication,gruber2017deep}. 
The stringent requirements on reliability and achievable throughput in xG propagation environments demand wireless communication systems that achieve provable performance guarantees over a variety of channels. 
Although there has been tremendous interest in the design of NN-based transceivers in the literature, their practical adaptation has been limited due to a lack of explainability and performance guarantees on the error rate or the complexity (training or hardware complexity). 
% Fueled by the promising results shown in other domains, wireless researchers have adopted a learning based approach in order to tame the stochasticity of the wireless channel. 
So far, much of the effort has been focused on generating representative datasets and end-to-end training of neural networks to achieve a target classification error (symbol decoding is a general multidimensional classification problem). These fixed function implementation that fits a particular dataset cannot be generalized to other scenarios, unless these two things are mathematically and semantically understood: 1) A measure of the acquired knowledge of the receiver neural network and 2) Bounds on learnability (or error) of a given neural network model for communication systems. In order to make wireless communications explainable, we have to set a baseline understanding of what happens inside a NN-based receiver that eventually performs the \textit{exact same} optimizations as performed in a conventional receiver. 
% This equivalent receiver is referred to as {\tnn}.
% 
% The stringent requirements on reliability and achievable throughput in xG propagation environments demand wireless communication systems that achieve provable performance guarantees over a variety of channels. 
% Although there has been tremendous interest in the design of NN-based transceivers in the literature, their pracical adaptation have been limited due to their lack of explainability and performance guarantees on the error rate or the complexity (training or hardware complexity). 
Therefore, we take the first step towards explaining the behaviour of NN-based receiver that is capable of achieving provable performance guarantees under various channel and signal configurations is crucial.
\note{This allows us to theoretically prove that NN-based receivers approach the error performance of optimal classical receivers when a mathematical channel model exists, and outperform classical receivers when a channel model does not exist. Moreover, NN-based receivers are computationally tractable over a variety of channels.}
Therefore we make the following contributions:

% Therefore, a NN-based communications system (or processing block) that does not require a rigorous mathematical model and that are computationally tractable and can achieve optimal performance guarantees under various channel and hardware imperfections is crucial. 
% 
% \textbf{Limitations of Existing NN-based Transceivers:}

% Therefore, a complete understanding of the theoretical foundation and limits of such approaches is imperative in order to identify opportunities where DL can outperform classical techniques. 
% We postulate that these opportunities are more substantial in the case of non-stationary, non-linear, non-Gaussian, multi-dimensional channels with unknown characteristics. Therefore the goal of this proposal is: \textit{To leverage the computational advantage of DL to iteratively reinforce the knowledge of hidden correlations in the channel in order to pre-compensate the waveform at the transmitter, such that a neural network based receiver operates with a deterministic error bound for any and all wireless environment}. 



% \note{
% The case for using neural networks for wireless communication has been getting stronger in recent years. 
% Fueled by the promising results shown in other domains, wireless researchers have adopted a learning based approach in order to tame the stochasticity of the wireless channel. 
% So far, much of the effort has been focused on generating representative datasets and end-to-end training of neural networks to achieve a target classification error (symbol decoding is a general multidimensional classification problem). We believe that fixed function implementation that fits a particular dataset cannot be generalized to other scenarios, unless these two things are mathematically and semantically understood: 1) A measure of the acquired knowledge of the receiver neural network and 2) Bounds on learnability (or error) of a given neural network model for communication systems. In order to make wireless communications explainable, we have to set a baseline understanding of what happens inside a NN-based receiver that eventually performs the \textit{exact same} optimizations as performed in a conventional receiver. This equivalent receiver is referred to as {\tnn}.
% }

% \noindent
% \textbf{Motivation:}\\
% \textbf{Limitations of Classical Transceivers:}
% Most existing signal processing algorithms in classical communications have strong foundations in statistics and information theory and are often provably optimal for tractable mathematically models of the channel, which are generally linear, stationary, and have Gaussian statistics. 
% However, practical and modern communication systems are highly dense and dynamic leading to channels that are non-linear (\eg non-linearity of power amplifiers, and quantization), highly dimensional (\eg MIMO and mm-wave), non-stationary (\eg V2X, UAV, massive MIMO) and poorly understood. Under such channels classical systems perform suboptimally and are often computationally intractable. Therefore, a NN-based communications system (or processing block) that does not require a rigorous mathematical model and that are computationally tractable and can achieve optimal performance guarantees under various channel and hardware imperfections is crucial. 
% % 
% % \textbf{Limitations of Existing NN-based Transceivers:}
% Although there has been tremendous interest in designing NN-based transceivers in the literature, they do not provide provable performance guarantees in terms of the BER/ capacity or the complexity (training or hardware complexity) and are limited to specific channel conditions. Therefore, a NN-based communications system that is capable of achieving provable performance guarantees under various channel and signal configurations is crucial. 

% \noindent\textit{\textbf{Goal:} To design equivalent NN structures to achieve performance guarantees in terms of BER and complexity. }

% \noindent
% \textbf{Contributions:} %Therefore our contributions are,
\begin{itemize}
    % \item Showing that {\tnn} and {\tmap} are equivalent.
    % \item Derive the complexity penalty of NNs to minimize the generalization error of {\tnn}.
    \item Theoretically proving that a feed forward deep NN-based receiver with the MSE loss function is probabilistically equivalent to the optimal MAP receiver, under complete training and a sufficiently rich data-set, without requiring any prior knowledge of channel statistics.
    \item We show that for a finite training data-set, the average testing loss of the NN-based receiver is distributed as a Gaussian.
    \item We derive tight upper and lower bounds on the Bit Error Rate (BER) of the NN-based receiver as a function of average testing loss and the number of training samples.
    \item Practical evaluation using a simulation framework to corroborate the accuracy of the proposed interpretation and bounds and compare the performance of NN-based and classical receivers over a variety of channels.
    % \item Derive the loss functions of NNs to achieve equivalence of {\tnn} and {\tmap}.
    % \item Derive bounds on the performance of {\tnn} for BER and complexity.
    % % \item Derive the structure of {\tnn} to achieve equivalence with {\tmap}.
    % \item Practical evaluation using a simulation framework to show the equivalence of {\tnn} and {\tmap}.
    % % \item Derive the complexity penalty of NNs to minimize the generalization error of {\tnn}.
\end{itemize}

\begin{figure*}
        \centering
        \begin{subfigure}{0.48\textwidth}
		\includegraphics[width=\textwidth]{figures/System_Diagram.pdf}
                \caption{Block structure of {\tmap} and the wireless channel: We design the structure of {\tnn} to achieve equivalence block-wise and as a whole with {\tmap}.}%Constellation before pre-compensation
                \label{fig:T_MAP}
        \end{subfigure}% 
        \quad
        \begin{subfigure}{0.48\textwidth}
                \includegraphics[width=\textwidth]{figures/NNReceiver.pdf}
                \caption{Structure of {\tnn} to achieve equivalence block-wise and as a whole with {\tmap}.}%Constellation after pre-compensation
                \label{fig:T_NN}
        \end{subfigure}
	\caption{Equivalent receivers of {\tnn} and {\tmap}.}
	\label{fig:whole}
% 	\vspace{-10pt}
\end{figure*}


% \note{
% An optimum decision yields the minimum error probability given as $P_{err}{=}P[\hat{m}{\neq} m]$, which is obtained by the maximum posteriori probability (MAP) rule. In neural network terms, $P_{err}$ is referred to as the \textit{Bayesian risk} \cite{ML_Probability_book_Murphy} that is analogous to a measure of the Bit Error Rate (BER). We define and design the {\tnn} that is equivalent to the optimal classical receiver, {\tmap} that achieves provable performance guarantees in terms of BER and model complexity. This is achieved by deriving the loss function of {\tnn} that guarantees the equivalence individually and collectively with each block of {\tmap} and implementing the corresponding equivalent optimum structure of {\tnn}. 
% Now, {\tnn} is defined as the NN model (with parameters $\delta_n$, where $n$ is the number of training samples) that minimizes a regularized risk $\tilde{\mathcal{R}}(\mathcal{D}, \delta_n)$ for given training data $\mathcal{D}$ as in \eqref{eq:NN_risk},
% }
%\useshortskip
% \small
% \begin{align}
% \label{eq:NN_risk}
% \hat{\delta}_{\lambda}&{=}\argmin_{\delta_n}\left[\tilde{\mathcal{R}}(\mathcal{D}, \delta_n)\right] \quad \text{ where,} \quad 
% \tilde{\mathcal{R}}(\mathcal{D}, \delta_n) {=} \mathcal{R}(\mathcal{D}, \delta_n)+\lambda C(\delta_n) \quad \text{and,} \quad 
% % \quad &&\text{where,}\\    
% \mathcal{R}(\mathcal{D}, \delta_n){=} \mathrm{E}[\mathcal{L}(\mathcal{D}, \delta_n)]  
% \end{align}
% \normalsize
% % where $\mathcal{R}(\mathcal{D}, \delta)$ is the risk function, $\mathcal{L}(\mathcal{D}, \delta)$ is the loss function . 

% %\vspace{-12pt}
% The risk function $\mathcal{R}(\mathcal{D}, \delta)$ is a measure of the average prediction or estimation error of the {\tnn} and is a measure of the Bayesian risk. $C(\delta_n)$ is a regularization term~\cite{ML_Probability_book_Murphy} and is essential to avoid over-fitting and $\lambda$ is used to trade-off accuracy and model complexity of {\tnn}.
% Let, $\fnn(\boldsymbol{r};\delta_n)$ be a function describing relationship between the input $\boldsymbol{r}$ and the output of the {\tnn} that has been trained as in \eqref{eq:NN_risk}. A {\tnn} with associated function $\fnn$ and {\tmap} with associated function $f_{MAP}$, are defined as equivalent if their outputs converge in probability as in 
% \eqref{eq:equivalence},
% %\vspace{-10pt}
% %\useshortskip
% \begin{align}
% \small
% %\vspace{-5pt}
% \lim_{n{\rightarrow}\infty}\mathrm{P}\left[|\fnn(\boldsymbol{r};\delta_n)-f_{MAP}(\boldsymbol{r})|\right]{\rightarrow}0.
% \label{eq:equivalence}
% \end{align}\normalsize

% %\vspace{-10pt}
% For known and stationary channel distributions, since {\tmap} is the receiver that achieves the minimum probability of error, we have that $\mathcal{R}(f_{MAP}){\leqslant} \mathcal{R}(\fnn)$. In other words, for known stationary distributions {\tnn} cannot achieve a lower error rate than {\tmap}, and the {\tnn} with minimum error rate is the one that achieves equivalence with {\tmap}. The tasks within this thrust aim to test this hypothesis, mathematically and experimentally, for wireless channels with known, unknown and non-stationary distributions. %We start with a general feedforward {\tnn} and determine the design criteria under which it achieves baseline equivalence with {\tmap}.



% \begin{figure*}
%   \centering
%     \subcaptionbox{Block structure of {\tmap} and the wireless channel: We design the structure of {\tnn} to achieve equivalence block-wise and as a whole with {\tmap}.
%     \label{fig:sys}}[.48\textwidth][c]{%
%     \includegraphics[width=0.48\textwidth]{figures/System_Diagram.pdf}}\quad
%     % \quad \quad \quad
%     \subcaptionbox{Structure of {\tnn} to achieve equivalence block-wise and as a whole with {\tmap}. \label{fig:T_NN}}[.48\textwidth][c]{%
%     \includegraphics[width=0.48\textwidth]{figures/NNReceiver.pdf}}
% %   \vspace{-15pt}
%   \caption{Equivalent receivers of {\tnn} and {\tmap}.}
%   \label{fig:adaptive_smoothing}
% %   \vspace{-10pt}
% \end{figure*}


% \begin{figure}[t]
%         \centering
% 		\includegraphics[width=0.5\textwidth]{figures/System_Diagram.pdf}  %{FullSystemFFF.pdf}
% % 		\vspace{-30pt}
%         \caption{Block structure of {\tmap} and the wireless channel: We design the structure of {\tnn} to achieve equivalence block-wise and as a whole with {\tmap}.
%         }   %IMAGE MUST BE MODIFIED
%         \label{fig:sys}
%     %  \vspace{-20pt}   
% \end{figure}
% \begin{figure}[h]
%         \centering
% 		\includegraphics[width=0.5\textwidth]{figures/NNReceiver.pdf}  %{FullSystemFFF.pdf}
% % 		\vspace{-30pt}
%         \caption{Structure of {\tnn} to achieve equivalence block-wise and as a whole with {\tmap}.
%         }   %IMAGE MUST BE MODIFIED
%         \label{fig:T_NN}
%     %  \vspace{-20pt}   
% \end{figure}

% Figure \ref{fig:sys} shows the modular block structure of {\tmap}: One of the guiding principles of communications systems design is to split the signal processing into a chain of multiple independent blocks; each executing a well defined and isolated function (e.g., source/channel coding, modulation, channel estimation, equalization).  This modular approach has led to the optimal, versatile and controllable classical communication systems we have today. Thus, we start by designing the equivalent structure of {\tnn} for each communication block as in figure \ref{fig:sys} and then focus on the end-to-end architecture of {\tnn} to jointly optimize the end-to-end system. 



% \begin{enumerate}
%     \item Model and preliminaries
%     \item Equivalence and Risk function determination
%     \item Generalization and loss function determination - Generalized BER bound
%     \item Inverse Design
% \end{enumerate}
\end{comment}











%-----------------OLD INTRO-----------------%
\begin{comment}
\section{Introduction}
\label{sec:intro}


The goal of this work is to identify the opportunities for learning in wireless communication and design a universal learning framework that is capable of adapting to any propagation environment. Design and analysis of optimal receivers using conventional communication theory, rely on mathematical and statistical channel models and, in some cases, instantaneous channel state information about the model, that describe how a signal is corrupted during transmission. 
%In particular, communication techniques such as modulation, coding and detection that mitigate performance degradation due to channel impairments are based on such channel models and, in some cases, instantaneous channel state information about the model. 
However, there are many propagation environments where this approach does not work well because the underlying physical channel is highly dimensional, non-linear, non-gaussian, poorly understood, or rapidly time-varying (non-stationary). 
These channels lead to sub-optimal and sometimes catastrophic performance using conventional receivers. 
This problem is relatively tractable and has been studied in the literature for linear, stationary channels with normal distribution by employing the gamut of mathematical tools for Bayesian inference. %that ranges from Autoregressive random walks, Kalman filters and Particle filters.

Deep Learning has emerged as a versatile tool for physical layer communication due to its proficiency in systems with model or algorithm deficit, and has been used to replace individual blocks in communication systems or optimize the entire transmitter-receiver (model agnostic) architecture. 
Recent developments in  the field seek to leverage the underlying physics (physics-driven, expert/domain based learning), underlying causal structures (causal learning), attention (transformer networks), memory (recurrent learning), learning to learn (meta-learning), adaptability to a wide variety of environments (transfer learning), distributed optimization (federated learning) and the interpretability of the underlying mechanism to provide learning guarantees (explainable AI). 
% The universal framework may lie at the intersection of these techniques, which needs further investigation. 
% Deep Learning techniques serve as universal function approximators driven by an objective, and have been attractive to systems with model-deficit or algorithm-deficit. 
%and have been used to replace individual blocks in classical communication systems or optimize and replace the the entire transmitter-receiver architecture 
However, they have come at the cost of increased hardware, memory and training complexity, poor-interpretability and have at best approached the performance of classical approaches (in terms of BER or throughput).
% Therefore to understand \textit{when and why it is beneficial to learn the channel},
Therefore we require a complete overhaul of the theoretical and analytical foundations and limitations of such approaches, to identify the true opportunities where learning the wireless channel is beneficial over classical techniques.
Modern wireless channels have been shown to exhibit adverse propagation conditions (unknown distributions, non-linearity, non-gasussian, non-stationary and multi-modal), which have rendered conventional communication techniques sub-optimal. 
We postulate and demonstrate that these opportunities are more substantial in the case of unknown channel distributions or when the channel is non-stationary, non-linear, non-gaussian, multi-dimensional channels with unknown characteristics.

Therefore, we make the following contributions:
%\note{check for correctness and add/modify if required}: 
\begin{enumerate}
    \item Theoretical proofs and experimental validation of the equivalency of NN-based and classical transceivers in SISO \& MIMO channels  (Section \ref{sec:equivalence}).
    \item Identifying the conditions under which NN-based transceivers outperform classical approaches. 
    \item The inverse design of NN-based transceivers for guaranteed performance (Section \ref{sec:design}).
    % \item Data augmentation to create a complete data-set (Section \ref{sec:data_augmentation}). 
    \item Practical evaluation using a simulations (Section \ref{sec:results}). 
\end{enumerate}

The key benefits of achieving equivalence:
\begin{enumerate}
    \item Theoretically optimal NN transceiver design under known channel models.
    \item Low complexity NN transceiver design for algorithm deficit problems.
    \item Design of near optimal NN transceivers for model deficit problems. 
    \item Reduction in the complexity of the NN: Algorithm/ Model Complexity, training complexity- From equivalence and the Universal approximation theorem we can now design each receiver block with one layer NN.
    % \item Data augmentation to create a complete data-set (Section \ref{sec:data_augmentation}). 
    \item This is the first step towards explainable and composable NN. 
\end{enumerate}
\end{comment}

==> models.tex <==
\section{MODELS}

==> models_icc22.tex <==
% \vspace{-10pt}
\section{Non-stationary channel decomposition and characterization}
\label{sec:NSdec}
The analysis of non-stationary channels is %particularly 
complicated as its statistics vary across both time-frequency and delay-Doppler domains resulting in 4-D second order statistics \cite{Matz2005NS}, which motivates the need for a unified characterization of wireless channels\footnote{Any channel can be generated as a special case of the non-stationary channel. Therefore a characterization of non-stationary channels would generalize to any other wireless channel \cite{MATZ20111}.}.
Wireless channels are completely characterized by their statistics, however they are difficult to extract for non-stationary channels, due to their time dependence.
% The analysis of non-stationary channels is %particularly 
% complicated as its statistics vary across both time-frequency and delay-Doppler domains resulting in 4-D second order statistics \cite{Matz2005NS}, which motivates the need for a unified characterization of wireless channels\footnote{Any channel can be generated as a special case of the non-stationary channel. Therefore a characterization of non-stationary channels would generalize to any other wireless channel \cite{MATZ20111}.}.
% Wireless channels are completely characterized by their statistics, however they are difficult to extract for non-stationary channels, due to their time dependence.
% % often difficult to extract in practice especially for non-stationary channels. 
% \note{Add how}.}. 
% which motivates us to find a method to unify the characterization of channels. 
% 
% The analysis of non-WSSUS channel is complicated as its statistics across time-frequency delay-Doppler 4-D domain, which motivates us to find a method to unify the characterization. 
% 
% Any LTV channel can be built by atomic channel $\mathbf{G}$~\cite{Matz2005NS}
Therefore, we start by expressing the channel $H$ using an atomic channel $G$ and the 4-D channel kernel $\mathcal{H}(t, f ; \tau, \nu)$~\cite{Matz2005NS} as in \eqref{eq:atomic}, 
% \ingreen{Both G and $\mathcal{H}$ are in Matz's paper} % as,
\begin{align}
\label{eq:atomic}
   H = \iiiint \mathcal{H}(t, f ; \tau, \nu) G_{t,f}^{\tau,\nu} ~dt ~df ~d\tau ~dv
\end{align}
% \note{Include definition/ meaning for $\mathcal{H}(t, f ; \tau, \nu)$.}
where $G$ is a normalized $(||G||{=}1)$ linear prototype system whose transfer function $L_G(t, f)$ is smooth and localized about the origin of the TF plane. $G_{t,f}^{\tau,\nu} {=} S_{t, f{+}\nu} G S_{t{-}\tau, f}^+$ means that the atomic channel $G$ shifts the signal components localized at $(t{-}\tau, f)$ to $(t, f{+}\nu)$ on the TF plane. $S_{\tau, \nu}$ is TF shift operator defined as $(S_{\tau, \nu}s)(t) {=} s(t{-}\tau) e^{j2 \pi \nu t}$. 
Then the channel kernel $\mathcal{H}(t, f ; \tau, \nu)$ is given by \eqref{eq:compute_H}.
\begin{align}
\label{eq:compute_H}
&\mathcal{H}(t, f ; \tau, \nu)=\left\langle H, G_{t, f}^{\tau, \nu}\right\rangle  \\
& {=}\mathrm{e}^{j 2 \pi f \tau} \iint L_{H}\left(t^{\prime}, f^{\prime}\right) L_{G}^{*}\left(t^{\prime}{\shortminus}t, f^{\prime}{\shortminus}f\right) %\nonumber \\
%  {\times} 
 \mathrm{e}^{{-}j 2 \pi\left(\nu t^{\prime}{-}\tau f^{\prime}\right)} \mathrm{d} t^{\prime} \mathrm{d} f^{\prime} \nonumber
 \end{align}

% Consider no matter how the domain transfer, the statistics can always be obtained by the 4-D kernel, if we can decompose it to a fundamental basis, it can give us chance to characterize the non-WSSUS channel in a unified form.
% Since the statistics of any wireless channel can always be obtained from the 4-D \note{kernel}, decomposing it into \note{fundamental basis}, provides a method
The statistics of any wireless channel %(regardless of the domain transfer) 
can always be obtained from the above 4-D channel kernel. Therefore, decomposing this kernel into fundamental basis allows us to derive a unified form to characterize any wireless channel.
% \rood{Define what is a unified characterization: Is it defined by the eigenfunctions or the statistics. Use citations.}

\begin{comment}
To characterize and precode non-WSSUS channel. The steps are
\begin{enumerate}
    \item Propose input-output relation specific to non-WSSUS channel with kernel, which should have following constraints/properties.
    \begin{itemize}
        \item Characterize non-WSSUS channel. The kernel is specific for non-WSSUS channel.
        \item Achievable. The kernel can be obtained by measurable items.
        \item Explainable. The kernel can be associated with non-WSSUS statistics, i.e., the non-WSSUS statistics can be expressed by the kernel.
    \end{itemize}
    \item Decompose the non-WSSUS channel kernel with properties that can  characterize statistics of non-WSSUS channel well.
    \item Design the precoding scheme based on the non-WSSUS channel kernel and the properties of decomposed components. 
\end{enumerate}
\subsection{non-WSSUS channel input-output relation}
\noindent
\end{comment}

\begin{comment}
To specify non-WSSUS channel, we define \textit{local spreading function} $h(t, f; \tau, \nu)$:
\begin{align}
\label{eq:deflsf}
    & h(t,f; \tau, \nu) \triangleq \mathbb{F}^2 \{ S_H(\tau, \nu + \Delta \nu) g^*(\tau - \Delta \tau, \nu) \} \nonumber \\
    & = \iint S_H(\tau, \nu + \Delta \nu) g^*(\tau - \Delta \tau, \nu) \nonumber \\
    & \times e^{j2\pi (t \Delta \nu - f \Delta \tau)} ~d\Delta \tau ~d\Delta \nu
\end{align}
which denotes delay-Doppler complex attenuation at TF location $(t,f)$. $g(\tau, \nu)$ is the window function with $\iint ||g(\tau,\nu)||^2 ~d\tau ~d\nu {=} 1$. 

The multi-carrier input-output relation for non-WSSUS channel can be written as 
\begin{equation}
\label{eq:h}
    r(t,f) = \iint h(t,f; \tau, \nu) s(t - \tau, f - \nu) ~d\tau ~d\nu + v(t,f)
\end{equation}

We have non-WSSUS channel statistics and local spreading relation proposition. 
\end{comment}
\begin{comment}
\begin{prop}

The time-frequency delay-Doppler input-output relation for non-WSSUS channel is 
\begin{equation}
\label{eq:h}
    r(t,f) = \iint h(t,f; \tau, \nu) s(t - \tau, f - \nu) ~d\tau ~d\nu + v(t,f)
\end{equation}
where $h(t,f; \tau, \nu)$ is local spreading function, and CCF can be expressed as


\begin{align}
    & \mathcal{A}(\Delta t, \Delta f;\Delta \tau, \Delta \nu) \nonumber \\
    &{=} \iiiint {E} \{h^*(t - \Delta t, f - \Delta f; \tau - \Delta \tau, v - \Delta \nu) \nonumber\\
    & \times h(t,f;\tau, \nu)\} ~dt ~df ~d\tau ~d\nu
\end{align}
\end{prop}
\begin{proof}
See Appendix~\ref{}
\end{proof}
\end{comment}

\begin{comment}
The \textit{short-time Fourier transform (STFT)} of \eqref{eq:S_H} can be expressed as 
\begin{align}
   r(t,f) = \iint S_H(\tau, \nu) s_{t,f}^{\tau,\nu} ~dt ~df ~d\tau ~dv
\end{align}
\end{comment}

\begin{comment}
\noindent
\textbf{Delay-Doppler domain:}
The OTFS delay-Doppler input-output relation theorem~\cite{hadani2018OTFS} can be expressed as continuous form
\begin{equation}
\label{eq:otfs_1}
    r(\tau,\nu) = \iint h_w(\tau', \nu') s(\tau - \tau', \nu - \nu') ~d\tau' ~d\nu' + v(\tau,\nu)
\end{equation}
where $v(\tau,\nu)$ is noise, and $h_w (\tau, \nu)$ is the convolution of delay-Doppler response $h_c(\tau, \nu)$ with window function $w(\tau,\nu)$:
\begin{equation}
\label{eq:otfs_2}
h_{w}(\tau, \nu)=\iint e^{-j 2 \pi \nu^{\prime} \tau^{\prime}} h_c\left(\tau^{\prime}, \nu^{\prime}\right) w\left(\nu-\nu^{\prime}, \tau-\tau^{\prime}\right) \mathrm{d} \tau^{\prime} \mathrm{d} \nu^{\prime}
\end{equation}

Notice $h_w(\tau, \nu)$ is the phase-shift correlation function of delay-Doppler response and window function for WSSUS case. 

For non-WSSUS case, define $h(\tau, \nu; \tau', \nu') \triangleq \mathbb{E}\{h_c(\tau'{-} \tau, \nu') w^*(\tau', \nu' {+} \nu)\}$. Then the delay-Doppler input-output relation can for non-WSSUS channel is 
\begin{equation}
\label{eq:otfs_1}
    r(\tau,\nu) = \iint h(\tau,\nu; \tau', \nu') s(\tau - \tau', \nu - \nu') ~d\tau' ~d\nu' + v(\tau,\nu)
\end{equation}
which has the similar form with \eqref{eq:h}.
\end{comment}
\begin{comment}
\begin{align}
\label{eq:deflsf}
    & h(t,f; \tau, \nu) = \mathbb{F}^2 \{ E[ S_H(\tau, \nu + \Delta \nu) g^*(\tau - \Delta \tau, \nu)] \} \nonumber \\
    & = \iint e^{-j2\pi \Delta \tau \Delta \nu} S_H(\Delta \tau, \Delta \nu)   \nonumber \\
    & \times g^*(\tau - \Delta \tau, \nu - \Delta \nu) e^{j2\pi (t \Delta \nu - f \Delta \tau)} ~d\Delta \tau ~d\Delta \nu
\end{align}
\end{comment}



\subsection{Channel decomposition}
% \rood{We need to re-format/write this section to be more direct. What is the problem, why and how we solve it. Need to mention specifics about why this decomposition is unique compared to any tensor decomposition. 4-D to 2-D is needed to ensure joint interference cancellation by precoding.}
% \note{Check: 
4-D channel kernel decomposition into orthonormal 2-D kernels is unprecedented the literature, but is essential to mitigate joint interference in the 2-D space and to completely characterize non-stationary channels.  
While Mercer's theorem \cite{1909Mercer} provides a method to decompose symmetric 2-D kernels into the same eigenfunctions along different dimensions, it cannot directly decompose 4-D channel kernels due to their high-dimensionality and since the kernel is not necessarily symmetric in the time-frequency delay-Doppler domains. 
% On the otherhand, 
Karhunen–Loève transform (KLT) \cite{wang2008karhunen}
provides a method to decompose kernels into component eigenfunctions of the same dimension, however is unable to decompose into orthonormal 2-D space-time eigenfunctions, and hence cannot be used to mitigate interference on the joint space-time dimensions. 
Therefore, we derive an %novel method for 
asymmetric 4-dimensional kernel decomposition method that %by deriving and combining 
combines the following two steps as shown in figure \ref{fig:thm}:
A) A generalization of Mercer's theorem that is applicable to both symmetric or asymmetric kernels, and B) An extension of KLT for high-dimensional kernels. 
% } 
% \ingreen{The reason we don't use KLT or highe order KLT is not because it is unstructured. The key is KLT can only decompose eignfunctions with same dimensions, i.e., 4-D kernel will only give us 4-D eigenfuntions. However, time-frequency and delay-doppler are two corresponding 2-D domains and many properties/statistics across 2-D domain not 4-D. So it should be further decomposed to more fundamental basis (2-D eigenfunctions) which give us more freedom to characterize properties.}
% Therefore, we propose a generalized version of Mercer's theorem that is applicable to both higher dimensional and asymmetric kernels. 
% \textit{Karhunen–Loève theorem} (KLT), which is deduced from Mercer's theorem, can decompose one dimensional process to eigenfunctions giving the opportunity to generalize Mercer's theorem for the non-symmetric case. 
% \begin{enumerate}
%     \item is not symmetric at time-frequency delay Doppler domain.
%     \item has higher dimension.
% \end{enumerate}


% \textit{Mercer's theorem} can decompose 2-D symmetric kernels into the same eigenfunctions along different direction/dimension. However, it can not be directly applied as the 4-D kernel  
% \begin{enumerate}
%     \item is not symmetric at time-frequency delay Doppler domain.
%     \item has higher dimension.
% \end{enumerate}

% \textit{Karhunen–Loève theorem} (KLT), which is deduced from Mercer's theorem, can decompose one dimensional process to eigenfunctions giving the opportunity to generalize Mercer's theorem for the non-symmetric case. 


\begin{lemma}
\label{lemma:GMT}
(Generalized Mercer's theorem (GMT))
% Given a 2-D process $K {\in} L^2(X {\times} Y)$, where $X$ and $Y$ both are square-integrable zero-mean random processes, the decomposition of $K$ is given by,
The decomposition of a 2-D process $K {\in} L^2(X {\times} Y)$, where $X$ and $Y$ are square-integrable zero-mean %random 
processes, %the decomposition of $K$ 
is given by,
\begin{align}
    K(t, t') = \sum\nolimits_{n=1}^{\infty} \sigma_n \psi_n(t) \phi_n(t')
    \label{eq:GMT}
\end{align}
where $\sigma_n$ is a random variable with $\mathbb{E}\{\sigma_n \sigma_{n'}\} {=} \lambda_n \delta_{nn'}$, and $\lambda_n$ is the $n$\textsuperscript{th} eigenvalue. $\psi_n(t)$ and $\phi_n(t')$ are eigenfunctions.
\end{lemma}
% 
\noindent
The proof combines %the 
Mercer's Theorem with KLT to generalize it to asymmetric kernels and is provided in Appendix B-A in the external document \cite{appendix_link}. %\ingreen{
% The proof is provided in Appendix \ref{App:gmt} in the external document in \cite{appendix_link}. 
% \note{Need more specifics:} 
% The proof combines the Mercer's Theorem with KLT to generalize it to asymmetric kernels.
% , and combines the Mercer's Theorem with KLT decompose one dimensional process to eigenfunctions giving the opportunity to generalize Mercer's theorem for the non-symmetric case
% \begin{proof}
% See Appendix~\ref{App:gmt}.
% \end{proof} 
% \noindent
% \textbf{High dimensional KLT}: 
% 
% By letting $\rho(t, t'){=}\psi_n(t) \phi_n(t')$, we have from Lemma~\ref{lemma:GMT} that, $K(t, t') {=} \sum_{n=1}^{\infty} \sigma_n \rho_n(t, t')$. 
From Lemma~\ref{lemma:GMT}, by letting $\rho(t, t'){=}\psi_n(t) \phi_n(t')$ in \eqref{eq:GMT} we have \eqref{eq:GMT_2D}, 
\begin{equation}
    K(t, t') {=} \sum_{n=1}^{\infty} \sigma_n \rho_n(t, t')
    \label{eq:GMT_2D}
\end{equation}
where the 2-D kernel is decomposed into random variable ${\sigma_n}$ with constituent %eigenvalues and 
2-D eigenfunctions, $\rho(t, t')$, this serves as an extension of KLT %(which is applicable to 1-D processes) 
to 2-D kernels.
% Letting $\rho(t, t'){=}\psi_n(t) \phi_n(t')$ in Lemma~\ref{lemma:GMT} we have that, $K(t, t') {=} \sum_{n=1}^{\infty} \sigma_n \rho_n(t, t')$. 
% Since the 2-D kernel is decomposed into constituent %eigenvalues and 
% 2-D eigenfunctions, $\rho(t, t')$, this serves as an extension of KLT %(which is applicable to 1-D processes) 
% to 2-D kernels.
A similar extension leads to the derivation of KLT for N-dimensional kernels which is %the 
key to deriving Theorem \ref{thm:hogmt}.
% Let $\rho(t, t'){=}\psi_n(t) \phi_n(t')$. Then from Lemma~\ref{lemma:GMT} we have that, $K(t, t') {=} \sum_{n=1}^{\infty} \sigma_n \rho_n(t, t')$, which is an extension from conventional 1-D KLT to 2-D KLT \note{Say why?}.

% Let $\rho(t, t'){=}\psi_n(t) \phi_n(t')$, from \textit{Lemma}~\ref{lemma:GMT}, we have $K(t, t') {=} \sum_{n=1}^{\infty} \sigma_n \rho_n(t, t')$ which is two-dimensional KLT. 

% Lemma~\ref{lemma:GMT} for high dimensional cases can also be deduced from high dimensional KLT. The deduce process is shown in Figure~\ref{fig:thm}.

\noindent
\fbox{\begin{minipage}{0.97\linewidth}
\begin{theorem}
\label{thm:hogmt}
(High Order GMT (HOGMT)) The decomposition of $M {=} Q{+}P$ dimensional kernel $K {\in} L^M(X {\times} Y)$, where $X(\gamma_1,\cdots,\gamma_Q)$ and $Y(\zeta_1,\cdots,\zeta_P)$ are $Q$ and $P$ dimensional kernels respectively, that are square-integrable zero-mean random processes, is given by \eqref{eq:col},
\begin{align}
\label{eq:col}
K(\zeta_1{,}{...}{,}\zeta_P{;} \gamma_1{,}{...}{,} \gamma_Q) {=} {\sum_{n{=}1}^ \infty} \sigma_n \psi_n(\zeta_1{,}{...}{,}\zeta_P) \phi_n(\gamma_1{,}{...}{,}\gamma_Q)
% K(\zeta_1{,}{...}{,}\zeta_P{;} \gamma_1{,}{...}{,} \gamma_Q) {=} {\sum_{n}^ \infty} \sigma_n \psi_n(\zeta_1{,}{...}{,}\zeta_P) \phi_n(\gamma_1{,}{...}{,}\gamma_Q)
% & K(\zeta_1{,\ldots,}\zeta_P; \gamma_1,\cdots, \gamma_Q) \nonumber \\
% & = \sum_{n}^ \infty \sigma_n \psi_n(\zeta_1,\cdots,\zeta_P) \phi_n(\gamma_1,\cdots, \gamma_Q)
\end{align}
%
where $\mathbb{E}\{\sigma_n \sigma_n'\} {=} \lambda_n \delta_{nn'}$. $\lambda_n$ is the $n$\textsuperscript{th} eigenvalue and $\psi_n(\zeta_1,\cdots,\zeta_P)$ and $\phi_n(\gamma_1,\cdots, \gamma_Q)$ are $P$ and $Q$ dimensional eigenfunctions respectively.
% \rood{Say what $y_i$ and $x_j$ are... Are they the random variables corresponding to each degree of freedom/ dimension.}
\end{theorem}
\end{minipage}}
% \begin{proof}
% The proof is provided in Appendix~\ref{app:hogmt}.
% \end{proof}

The proof is provided in Appendix~B-B in \cite{appendix_link}. 
% Then the decomposition of the spatio-temporal non-WSSUS channel kernel $\mathcal{H}(t, f ; \tau, \nu))$ is given by \eqref{},
% \begin{align}
% \mathcal{H}(t, f ; \tau, \nu)=\sum_{n}^{\infty} \sigma_{n} \psi_{n}(t, f) \phi_{n}(\tau, \nu)    
% \end{align}
% where $\mathbb{E}\left\{\sigma_{n} \sigma_{n}^{\prime}\right\}=\lambda_{n} \delta_{n n^{\prime}} . \quad \lambda_{n}$ is the $n^{\text {th }}$ eigenvalue, and $\psi_{n}(t, f)$ and $\phi_{n}(\tau, \nu)$ are both 2-dimensional eigenfunctions.
Theorem~\ref{thm:hogmt} is applicable to any $M$ dimensional channel kernel. Examples of such channel kernels may include 1-D time-varying channels, 2-D time-frequency kernels for doubly dispersive channels \cite{2003MatzDP}, user, antenna dimensions in MU-MIMO channels and angles of arrivals and departures %AoAs and AoDs 
in mmWave channels.
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/theorem_proof_sketch.pdf}
    \vspace{-10pt}
    \caption{Derivation of High Order Generalized Mercer's Theorem for channel decomposition}
    \vspace{-10pt}
    \label{fig:thm}
\end{figure}
Theorem~\ref{thm:hogmt} ensures that the 4-D channel kernel in \eqref{eq:compute_H} is decomposed as in \eqref{eq:channel_kernel_decomp} into 2-D eigenfunctions that are jointly orthonormal in the time-frequency dimensions as in \eqref{eq:properties}.
\begin{align}
\label{eq:channel_kernel_decomp}
&\mathcal{H}(t, f ; \tau, \nu) = \sum\nolimits_{n{=1}}^\infty \sigma_n \psi_n(t, f) \phi_n(\tau, \nu)\\
% \end{equation}
% with the following orthonormal properties,
% Finally, we get the desired decomposition \textit{corollary}~\ref{col:svdforNSchannel}, where the 4-D channel kernel is decomposed to 2-D eigenfunctions with orthonormal properties
% \begin{align}
\label{eq:properties}
&\begin{aligned}
&& \iint \psi_n(t, f) \psi_{n'}^*(t, f) ~dt ~df {=} \delta_{nn'}  \\
&& \iint \phi_n(\tau, \nu) \phi_{n'}^*(\tau, \nu) ~d\tau ~d\nu {=} \delta_{nn'}
\end{aligned}
\end{align}
% \note{Notice $\iint \mathcal{H}(t,f;\tau,\nu) \phi_n^*(\tau,\nu) ~d\tau~d\nu = \sigma_n \psi_n(t,f)$, we call $\phi_n$ and $\psi_n$ a pair of dual eigenfunctions.}
% Moreover, from \eqref{eq:channel_kernel_decomp} and \eqref{eq:properties} we have that, $\iint \mathcal{H}(t{,}f{;}\tau{,}\nu) \phi_n^*(\tau{,}\nu)d\tau d\nu {=} \sigma_n \psi_n(t{,}f)$. 
Moreover, from \eqref{eq:channel_kernel_decomp} and \eqref{eq:properties} we have that, 
\begin{align}
    \iint \mathcal{H}(t{,}f{;}\tau{,}\nu) \phi_n^*(\tau{,}\nu)~d\tau ~d\nu {=} \sigma_n \psi_n(t{,}f)
    \label{eq:duality}
\end{align}
% $\iint \mathcal{H}(t{,}f{;}\tau{,}\nu) \phi_n^*(\tau{,}\nu)d\tau d\nu {=} \sigma_n \psi_n(t{,}f)$. 
\eqref{eq:duality} suggests that %means that 
% Alternatively, 
when the eigenfunction, $\phi_n^*(\tau,\nu)$ is transmitted through the channel a different eigenfunction, $\psi_n(t,f)$ is received with $\sigma_n$. 
Therefore, we refer to $\phi_n$ and $\psi_n$ as a pair of \textit{dual} eigenfunctions.
% Further, these dual eigenfunctions represent flat-fading sub-channels of the channel $H$ as they are jointly orthogonal. each sub-channel is just a scaling of dual eigenfunctions.
By definition, these eigenfunctions are constituent sub-channels of the channel kernel that only undergo a scaling when transmitted over channel.
Therefore, the dual eigenfunctions are referred to as \textit{flat-fading sub-channels} of $H$.
% \note{Since, by definition each dual eigenfunction only undergoes a scaling when transmitte
% these dual eigenfunctions represent flat-fading sub-channels of the channel $H$ as they are jointly orthogonal. each sub-channel is just a scaling of dual eigenfunctions.}

\subsection{Unified Characterization Using Channel Statistics}
\label{sec:stat}
% \rood{Starting para: If the unified characterization is defined by the statistics, which statistics are important and why.}
% The extracted 2-D eigenfunctions and eigenvalues are use

Wireless channels are fully characterized by their (second order) statistics, which we calculate using the extracted eigenvalues and 2-D eigenfunctions.
The CCF is calculated as the correlations of $\mathcal{H}(t, f ; \tau, \nu)$~\cite{Matz2005NS} and is given by,
% The CCF can be interpreted as the correlation of $\mathcal{H}(t, f ; \tau, \nu)$~\cite{Matz2005NS}
\begin{align}
    & \abs{ \mathcal{R}(\Delta t, \Delta f;\Delta \tau, \Delta \nu) } \label{eq:CCF3}\\
    &{=}  \Bigl| {\iiiint} \mathbb{E}\{\mathcal{H}^*(t {\shortminus} {\smallDelta} t{,} f {\shortminus} {\smallDelta} f{;} \tau {\shortminus} {\smallDelta} \tau{,} \nu {\shortminus} {\smallDelta} \nu) %{\times} 
    \mathcal{H}(t{,}f{;}\tau{,} \nu)\} d t d f d \tau d \nu \Bigr|  \nonumber \\
    % &{=}  \Bigl| {\iiiint} \mathbb{E}\{\mathcal{H}^*(t {-} \Delta t{,} f {-} \Delta f{;} \tau {-} \Delta \tau{,} \nu {-} \Delta \nu) %{\times} 
    % \mathcal{H}(t{,}f{;}\tau{,} \nu)\} d t d f d \tau d \nu \Bigr|  \nonumber \\
    &{=} \sum\nolimits_{n{=1}}^\infty \lambda_n \abs{R_{\psi_n}(\Delta t,\Delta f)}  |R_{\phi_n}(\Delta \tau,\Delta \nu)| \label{eq:CCF2}
\end{align}
where \eqref{eq:CCF2} is obtained by substituting \eqref{eq:duality} in \eqref{eq:CCF3}. 
$R_{\psi_n}(\Delta t,\Delta f)$ and $R_{\phi_n}(\Delta \tau,\Delta \nu)$ are the correlations of $\psi_n(t, f)$ and $\phi_n(\tau, \nu)$, respectively. 
The LSF reveals the non-stationarities (in time or frequency) in a wireless channel and is given by the 4-D Fourier transform ($\mathbb{F}^{4}$) of the CCF as, 
% 
% in \eqref{eq:LSF_eigen},
% 
% Substitute \eqref{eq:col} in \eqref{eq:CCF}, the CCF can be expressed as 
% \begin{align}
% \label{eq:CCF}
%     & \abs{ \mathcal{A}(\Delta t, \Delta f;\Delta \tau, \Delta \nu) }\nonumber \\
%     & {=} \sum_{n}^ \infty \lambda_n \abs{R_{\psi_n}(\Delta t,\Delta f)}  |R_{\phi_n}(\Delta \tau,\Delta \nu)|
% \end{align}
% where $\lambda_n {=} \langle \sigma_n, \sigma_n \rangle$ is eigenvalue. $R_{\psi_n}(\Delta t,\Delta f)$ and $R_{\phi_n}(\Delta \tau,\Delta \nu)$ are correlation of $\psi_n(t, f)$ and $\phi_n(\tau, \nu)$, respectively. LSF is the 4-D Fourier relation with CCF
\begin{align}
\label{eq:LSF_eigen}
    & \mathcal{C}_H(t, f; \tau, \nu) {=} \mathbb{F}^{4}\left\{\mathcal{R}({\smallDelta} t{,} {\smallDelta} f{;}{\smallDelta} \tau{,} {\smallDelta} \nu)\right\} \nonumber\\
    & {=} \iiiint \mathcal{R}({\smallDelta} t{,} {\smallDelta} f{;}{\smallDelta} \tau{,} {\smallDelta} \nu)
    \mathrm{e}^{{\shortminus}j 2 \pi(t \Delta \nu{\shortminus}f \Delta \tau{+}\tau \Delta f{\shortminus}\nu \Delta t)} \mathrm{d} t \mathrm{d} f \mathrm{d} \tau \mathrm{d} \nu \nonumber \\ 
    & {=} \sum\nolimits_{n{=1}}^\infty \lambda_n |\psi_n( \tau,\nu)|^2 |\phi_n(t, f)|^2
    % & C_H(t, f; \tau, \nu) {=} \mathbb{F}^{4}\left\{\mathcal{A}(\Delta t, \Delta f;\Delta \tau, \Delta \nu)\right\} \nonumber\\
    % & {=} \iiiint \mathcal{A}(\Delta t, \Delta f;\Delta \tau, \Delta \nu) \nonumber\\
    % & \times \mathrm{e}^{-j 2 \pi(t \Delta \nu-f \Delta \tau+\tau \Delta f-\nu \Delta t)} \mathrm{d} t \mathrm{~d} f \mathrm{~d} \tau \mathrm{~d} \nu \nonumber \\ 
    % & {=} \sum_{n}^ \infty \lambda_n |\psi_n( \tau,\nu)|^2 |\phi_n(t, f)|^2
\end{align}
where 
$|\psi_n( \tau,\nu)|^2$ and $|\phi_n(t, f)|^2$ represent the spectral density of $\psi_n(t,f)$ and $\phi_n(\tau,\nu)$, respectively.
% LSF can describe the non-stationarity of LTV channel. 
% 
Then, the %induced channel statistics
\textit{global (or average) scattering function} $\overline{C}_H(\tau, \nu)$ and (local) TF path gain $\rho_H^2 (t,f)$ \cite{Matz2005NS} are calculated in \eqref{eq:GSF} and \eqref{eq:rho},
% 
% The induced channel statistics \textit{global (or average) scattering function} $\overline{C}_H(\tau, \nu)$ and (local) TF path gain $\rho_H^2 (t,f)$ are also given by~\cite{Matz2005NS}
\begin{align}
\label{eq:GSF}
% \vspace{10pt}
    & \overline{C}_H(\tau, \nu) {=} \mathbb{E}\{|S_H(\tau, \nu)|^2\} = \iint \mathcal{C}_H(t, f; \tau, \nu) ~dt ~df  \\
    & \rho_H^2 (t,f) {=}  \mathbb{E}\{|L_H(t, f)|^2\} = \iint \mathcal{C}_H(t, f; \tau, \nu) ~d\tau ~dv 
\label{eq:rho}
\end{align}
\eqref{eq:GSF} and \eqref{eq:rho} are re-expressed in terms of the spectral density of eigenfunctions by using \eqref{eq:LSF_eigen} and the properties in \eqref{eq:properties},  
% Substituting in \eqref{eq:LSF_eigen} and using the properties in \eqref{eq:properties}, \eqref{eq:GSF} and \eqref{eq:rho} is expressed in terms of the spectral density of eigenfunctions as,
% Substituting \eqref{eq:LSF_eigen} and notice the properties \eqref{eq:properties}, they can be expressed by the spectral density of eigenfunctions

\begin{align}
    &\overline{C}_H(\tau, \nu) {=} \mathbb{E}\{|S_H(\tau, \nu)|^2\} {=} \sum\nolimits_{n{=1}}^\infty \lambda_n |\psi_n( \tau,\nu)|^2 \\
    &  \rho_H^2 (t,f) {=} \mathbb{E}\{|L_H(t, f)|^2\} {=} \sum\nolimits_{n{=1}}^\infty \lambda_n |\phi_n(t, f)|^2 
\end{align}


Finally, the \textit{total transmission gain} $\mathcal{E}_H^2$ is obtained by integrating the LSF out with respect to all four variables, 
\begin{align}
\label{TFgain}
    & \mathcal{E}_H^2 = \iiiint \mathcal{C}_H(t, f; \tau, \nu) ~dt ~df ~d \tau ~d\nu = \sum\nolimits_{n{=}1}^ \infty \lambda_n
\end{align}
Therefore, the statistics of the non-stationary channel is completely characterized by its eigenvalues and eigenfunctions %that are 
obtained by the decomposition of $\mathcal{H}(t,f;\tau,\nu)$, which are summarized in Table~\ref{tab:cha}.
% 
\setlength{\textfloatsep}{0.1cm}
\setlength{\tabcolsep}{0.2em}
\begin{table}[h]
\caption{Unified characterization of the non-stationary channel}
\renewcommand*{\arraystretch}{1.2}
\centering
\begin{tabular}{|l|l|}
\hline
Statistics & Eigen Characterization \\ \hline
CCF $|\mathcal{R}(\Delta t, \Delta f;\Delta \tau, \Delta \nu)|$             &   ${\sum} \lambda_n |R_{\psi_n}(\Delta t{,}\Delta f)| |R_{\phi_n}(\Delta \tau{,}\Delta \nu)|$                     \\ \hline
LSF  $\mathcal{C}_H(t, f; \tau, \nu)$             &         ${\sum} \lambda_n |\psi_n( \tau,\nu)|^2 |\phi_n(t, f)|^2$               \\ \hline
Global scattering function   $\overline{C}_H(\tau{,} \nu)$               &        ${\sum} \lambda_n |\psi_n( \tau,\nu)|^2 $                \\ \hline
Local TF path gain $\rho_H^2 (t,f)$
    & ${\sum} \lambda_n |\phi_n( t, f)|^2 $  \\ \hline
Total transmission gain     $\mathcal{E}_H^2$                          &     ${\sum} \lambda_n$                   \\ \hline
\end{tabular}
\label{tab:cha}
\vspace{-10pt}
\end{table}
% \rood{The unified characterization of the second-order statistics of wireless channels allows us to... list the benefits.}
% \rood{Zhibin: Check if eqs (7)--(19) are directly relevant to the rest of the paper. If they are we need to show some relevant results if possible. }
% 
% \begin{table}[h]
% \caption{Characterization of non-WSSUS channel.}
% \renewcommand*{\arraystretch}{1.2}
% \centering
% \begin{tabular}{|l|l|}
% \hline
% Statistics & Eigen Characterization \\ \hline
% CCF $|\mathcal{A}(\Delta t, \Delta f;\Delta \tau, \Delta \nu)|$             &   $\sum_{n}^ \infty \lambda_n |R_{\psi_n}(\Delta t,\Delta f)| |R_{\phi_n}(\Delta \tau,\Delta \nu)|$                     \\ \hline
% LSF  $C_H(t, f; \tau, \nu)$             &         $\sum_{n}^ \infty \lambda_n |\psi_n( \tau,\nu)|^2 |\phi_n(t, f)|^2$               \\ \hline
% Global scattering function   $\overline{C}_H(\tau, \nu)$               &        $\sum_{n}^ \infty \lambda_n |\psi_n( \tau,\nu)|^2 $                \\ \hline
% Local TF path gain $\rho_H^2 (t,f)$
%     & $\sum_{n}^ \infty \lambda_n |\phi_n( t, f)|^2 $  \\ \hline
% Total transmission gain     $\mathcal{E}_H^2$                          &     $\sum_{n}^ \infty \lambda_n$                   \\ \hline
% \end{tabular}
% \label{tab:cha}
% \end{table}

==> precoding_icc22.tex <==
\section{Joint Spatio-Temporal Precoding} %\ingreen{or GMT Based Precoding}}
\label{sec:Precoding}
% \rood{
% \noindent Intro: Why and How? Precoding for non-WSSUS channels is particularly challenging and unprecedented, since interference may exist in the joint space-time domain as well. Thus, we precode the non-WSSUS channel by leveraging eigenfunctions. Why joint space-time precoding?}

% \note{Zhibin: Is this a different channel equation than eq (1)/ (2). Better to have one definition in Section II. Also make sure the Notations are consistent with the rest of the paper. Also is it better to start directly with the Multi-user channel for this paper?} \ingreen{$h(t,\tau)$ defined at section 2. Need to consider if it will lose generality if begin with space-time domain.}
% The channel $H$ in \eqref{eq:h_tau} can be extended to incorporate multiple users as,
The kernel $\mathcal{H}(t, f ; \tau, \nu)$ in \eqref{eq:compute_H} describes the time-frequency delay-Doppler response of the channel from \eqref{eq:h_relation} and is essential to extract the statistics of the non-stationary channel $H$ for a single user as they depend on the same 4 dimensions.
% While the input-output relation can still denote as \eqref{eq:h_relation}. 
% While the input-output relation can still denote as \eqref{eq:h_relation}. 
For precoding, we express the spatio-temporal channel response %\cite{2011Hlawatsch} 
% is expressed 
by extending the time-varying response $h(t,\tau)$ to incorporate multiple users, i.e., $h_{u,u'}(t,\tau)$ \cite{2017GhazalNSmodel,almers2007survey}, which denotes the time-varying impulse response between the $u'$\textsuperscript{th} transmit antenna and the $u$\textsuperscript{th} user, where each user has a single antenna. The 4-D spatio-temporal channel estimation is widely investigated \cite{2020CESrivastava,2005CEXiaoli,2008CEMilojevic} . In this paper we assume perfect CSI at transmit. Thus the received signal in \eqref{eq:h_relation} is extended as
% by extending the time-varying response $h(t,\tau)$ to incorporate multiple users, i.e., $h_{u,u'}(t,\tau)$ \cite{2017GhazalNSmodel}, where $u$ is the antenna index of combined all receivers and $u'$ is the antenna index of the transmit. The 4-D spatio-temporal channel estimation is widely investigated \cite{2020CESrivastava,2005CEXiaoli,2008CEMilojevic} . In this paper we assume perfect CSI at transmit. Thus the received signal in \eqref{eq:h_relation} is extended as}
% \ingreen{The kernel $\mathcal{H}(t, f ; \tau, \nu)$ in \eqref{eq:compute_H} is used to extract the statistics for non-stationary channel $H$ which across time-frequency delay-Doppler domain. While the input-output relation can still denote as \eqref{eq:h_relation}. The spatio-temporal channel response \cite{MATZ20111} %\cite{2011Hlawatsch} 
% is expressed by extending \eqref{eq:h_relation} to incorporate multiple users as in \eqref{eq:MU}},
\begin{align}
    \label{eq:MU}
    r_u (t) &= \int \sum\nolimits_{u'} h_{u,u'}(t,\tau) s_{u'}(t-\tau) d\tau + v_{u}(t) \nonumber \\
    & = \int \sum\nolimits_{u'}  k_{u,u'}(t,t') s_{u'}(t') dt' + v_{u}(t)
    % r_u (t) &= \sum_{u'} h_{u,u'}(t,\tau) s_{u'}(t-\tau) + v_{u}(t) \nonumber \\
    % & = \sum_{u'} k_{u,u'}(t,t') s_{u'}(t') + v_{u}(t)
\end{align}
where $v_u(t)$ is the noise, $s_u(t)$ is the data signal and $k_{u,u'} (t, t') {=} h_{u,u'}(t, t{-}\tau)$ is the channel kernel.
Then, the relationship between the transmitted and received signals is obtained by rewriting \eqref{eq:MU} in its continuous form in \eqref{eq:MU2}.
% Rewriting~\eqref{eq:MU} in the continuous form, we obtain the space-time input-output relation of the channel as,
\begin{align}
    \label{eq:MU2}
    & r(u,t) = \iint k_H(u,t;u',t') s(u',t')~du'~dt' + v(u,t)
\end{align}

 %, then the received symbols is given by,
% \begin{align}
% \label{eq:k_H}
%  r(t) = \int k_H (t,t') s(t') ~d t'
% \end{align}
Let $x(u,t)$ be the precoded signal, then the corresponding received signal is $Hx(u,t)$. The aim of precoding in this work is to minimize the interference, i.e., to minimize the least square error, $\|s(u,t) {-} Hx(u,t)\|^2$.


\begin{comment}
The time-frequency input-output relation for non-WSSUS channel $H$ can be expressed as~\cite{Flandrin1998TF}
\begin{equation}
\label{eq:k}
    r(t,f) = \iint k_{H} (t,f; t', f') s(t', f') ~d t' ~d f' + v(t,f)
\end{equation}
where $v(t,f)$ is noise and $k_H (t,f; t', f')$ is channel kernel and can be obtained by
\begin{align}
\label{eq:LTF}
k_H (t,f; t', f') = L_H (t-t',f-f') e^{-j2\pi (f-f')t'}
\end{align}
\end{comment}

\begin{comment}
From \eqref{eq:atomic} and \eqref{eq:compute_H}, we have the OFDM input-output relation proposition specific to non-WSSUS channel.
\end{comment}

\begin{comment}
\begin{prop}
\label{prop:I/O}
Defining local TF transfer function $k_H(t,f; t', f')$, the time-frequency domain non-WSSUS channel input-output relation can be expressed as
\begin{equation}
\label{eq:k}
    r(t,f) = \iint k_H (t,f; t', f') s(t', f') ~d t' ~d f' + v(t,f)
\end{equation}
where $v(t,f)$ is noise and $k_H (t,f; t', f')$ can be obtained by
\begin{align}
\label{eq:LTF}
k_H (t,f; t', f') = L_{\mathbf{H}} (t-t',f-f') e^{-j2\pi (f-f')t'}
\end{align}
where $L_{\mathbf{H}}$ is the TF transfer function of non-WSSUS channel ${\mathbf{H}}$.
%
$h(t,f; t', f') \triangleq \mathcal{H}({-}t, {-}f{-}f' ; t', f')$ and 
\begin{align}
   &\mathcal{H}(-t, -f-f' ; t', f') =\iint \mathcal{H}(t', f' ; \tau', \nu') \nonumber \\ 
   &\mathrm{e}^{-j 2 \pi\left(\nu' t-\tau' (f+f^{\prime})\right)} \mathrm{d} \tau^{\prime} \mathrm{d} \nu^{\prime}
\end{align}
\end{prop}
\end{comment}
%

% \note{Check Lemma 1 and the explanation text.}
\begin{lemma}
\label{lemma:bestprojection}
Given a non-stationary channel $H$ with kernel $k_H(u{,}t{;}u'{,}t')$, if each projection in $\{H \varphi_n(u{,}t)\}$ are orthogonal to each other, there exists a precoded signal 
scheme 
$x(u,t)$ that ensures %achieves 
interference-free communication at the receiver, %i.e.,
\begin{align}
    & \|s(u,t) - Hx(u,t)\|^2 = 0 
\label{eq:obj}
\end{align}
where $\varphi_n(u,t)$ is the eigenfunction of $x(u,t)$, obtained by KLT decomposition as $x(u,t) {=} \sum_{n=1}^\infty x_n \varphi_n(u,t)$.
% \ingreen{here is KLT not inverse KLT as we don't construct x but decompose x in lemma 1}}.
\vspace{-5pt}
\end{lemma}
The proof is provided in Appendix C-A in \cite{appendix_link}.
% \begin{proof}
% See Appendix~\ref{app:lem1}.
% \end{proof}
% 
Therefore, precoding using $\{\varphi_n\}{=}\{\phi_n\}$ or $\{\varphi_n\}{=}\{\psi_n\}$) obtained by decomposing the %asymmetric 4-D 
channel kernel using Theorem \eqref{thm:hogmt}, (i.e., constructing $x(u,t)$ using $\{\phi_n\}$ or $\{\psi_n\}$ with coefficients $x_n$ using inverse KLT, eventually leads to interference-free communication, as it satisfies \eqref{eq:obj} by ensuring that $\{H \varphi_n(u,t)\}$ are orthogonal using the properties in \eqref{eq:properties}.
% \note{Lemma~\ref{lemma:bestprojection} shows that %the necessary condition 
% for interference-free communication in \eqref{eq:obj}, each projection of the channel onto the eigenfunctions of the transmitted signal, i.e., $\{H \varphi_n(u,t)\}$ should be orthogonal to each other.
% % \ingreen{Lemma~\ref{lemma:bestprojection} shows that the necessary condition for interference-free communication is the projections of the channel onto the eigenfunctions of the transmitted signal are orthogonal.} 
% % If the projections, $\{H \varphi_n(u,t)\}$ are also eigenfunctions, the above condition is satisfied (as eigenfunctions are orthogonal to each other by definition) and hence \eqref{eq:obj} is also %consequently 
% % satisfied.
% % Consequently, these eigenfunctions have t
% Therefore, precoding using one set of the eigenfunctions ($\phi_n$ or $\psi_n$) obtained by decomposing the %asymmetric 4-D 
% channel kernel using Theorem \eqref{thm:hogmt}, eventually leads to interference-free communication (i.e., it satisfies \eqref{eq:obj}), as it ensures that $\{H \varphi_n(u,t)\}$ are orthogonal using the properties in \eqref{eq:properties}.} 

% \ingreen{Therefore, if $\{\varphi_n\}$ is one set of the eigenfunctions ($\{\phi_n\}$ or $\{\psi_n\}$) obtained by decomposing the %asymmetric 4-D 
% channel kernel using Theorem \eqref{thm:hogmt}, i.e., construct $x(u,t)$ by $\{\phi_n\}$ or $\{\psi_n\}$ with certain coefficients $x_n$ by inversing KLT, eventually leads to interference-free communication (i.e., it satisfies \eqref{eq:obj}), as it ensures that $\{H \varphi_n(u,t)\}$ are orthogonal using the properties in \eqref{eq:properties}.}

\begin{comment}
\note{Lemma~\ref{lemma:bestprojection} shows that %the necessary condition 
for interference-free communication in \eqref{eq:obj}, each projection of the channel onto the eigenfunctions of the transmitted signal, i.e., $\{H \varphi_n(u,t)\}$ should be orthogonal to each other.
% \ingreen{Lemma~\ref{lemma:bestprojection} shows that the necessary condition for interference-free communication is the projections of the channel onto the eigenfunctions of the transmitted signal are orthogonal.} 
% If the projections, $\{H \varphi_n(u,t)\}$ are also eigenfunctions, the above condition is satisfied (as eigenfunctions are orthogonal to each other by definition) and hence \eqref{eq:obj} is also %consequently 
% satisfied.
% Consequently, these eigenfunctions have t
Therefore, precoding using one set of the eigenfunctions ($\phi_n$ or $\psi_n$) obtained by decomposing the %asymmetric 4-D 
channel kernel using Theorem \eqref{thm:hogmt}, eventually leads to interference-free communication (i.e., it satisfies \eqref{eq:obj}), as it ensures that $\{H \varphi_n(u,t)\}$ are orthogonal using the properties in \eqref{eq:properties}.} 
\ingreen{Therefore, if $\{\varphi_n\}$ is one set of the eigenfunctions ($\{\phi_n\}$ or $\{\psi_n\}$) obtained by decomposing the %asymmetric 4-D 
channel kernel using Theorem \eqref{thm:hogmt}, i.e., construct $x(u,t)$ by $\{\phi_n\}$ or $\{\psi_n\}$ with certain coefficients $x_n$ by inversing KLT, eventually leads to interference-free communication (i.e., it satisfies \eqref{eq:obj}), as it ensures that $\{H \varphi_n(u,t)\}$ are orthogonal using the properties in \eqref{eq:properties}.}
% Since, Theorem~\ref{thm:hogmt} decomposes the asymmetric 4-D channel kernel into dual eigenfunction pairs, precoding using one set of eigenfunctions leads to interference-free communication.
% If the projections $\{H \varphi_n(u,t)\}$ are also eigenfunctions, this condition is satisfied, which leads to property~\eqref{eq:properties} and Theorem~\ref{thm:hogmt}, where the asymmetric 4-D kernel can be decomposed to dual eigenfunction sets.
% Therefore, precoding using one set of dual eigenfunctions leads to interference-free communication.
% } 
\end{comment}

% Finally, we have non-WSSUS channel precoding theorem:

\noindent
\fbox{\begin{minipage}{0.97\linewidth}
\begin{theorem}
\label{thm:thm2}
(HOGMT-based precoding) Given a non-stationary channel $H$ with kernel $k_H(u,t;u',t')$, the precoded signal $x(u,t)$ that ensures interference-free communication at the receiver is constructed by inverse KLT as,
\begin{align}
\label{eq:x}
    x(u{,}t) {=} \sum_{n{=}1}^\infty x_n \phi_n^*(u{,}t),\text{where},
    x_n {=} \frac{{\langle} s(u{,}t){,} \psi_n(u{,}t) {\rangle}}{\sigma_n}
    % x(u,t) = \sum_n^\infty x_n \phi_n^*(u,t)\\
    % x_n = \frac{\langle s(u,t), \psi_n(u,t) \rangle}{\sigma_n}
\end{align}
where %$s(t)$ is the data signal. 
$\{ \sigma_n \}$, $\{ \psi_n\}$ and $\{ \phi_n\} $ are obtained by decomposing the kernel $k_H(u,t;u',t')$ using Theorem~\ref{thm:hogmt} as in \eqref{eq:thm2_decomp},
\begin{align}
\label{eq:thm2_decomp}
% k_H(u,t;u',t') = \sum_{n{=1}}^\infty  \sigma_n \psi_n(u,t) \phi_n(u',t')
&k_H(u,t;u',t') = \sum\nolimits_{n{=1}}^\infty  \sigma_n \psi_n(u,t) \phi_n(u',t')
\end{align}
with properties as in \eqref{eq:thm2_decomp_pty},
\begin{align}
\label{eq:thm2_decomp_pty}
\begin{aligned}
&\iint \psi_n(u, t) \psi_{n'}^*(u, t) ~du ~dt {=} \delta_{nn'}  \\
&\iint \phi_n(u', t') \phi_{n'}^*(u', t') ~du' ~dt' {=} \delta_{nn'}
\end{aligned}
\end{align}
% \note{Zhibin: (24) seems very similar to (9). If you think it'd be better to merge, you can do that or leave it.}
% \rood{Maybe, we should directly say that (27) is Theorem 2 for this paper.}
\end{theorem}
\end{minipage}}
% \begin{proof}
% See Appendix~\ref{app:thm_2}
% \end{proof}
The proof is provided in Appendix C-B in \cite{appendix_link}. 
Although precoding involves a linear combination of $\phi_n^*(u,t)$ with $x_n$ it is a non-linear function ($\mathcal{W}(\cdot)$) with respect to the data signal $s(u,t)$, i.e., $x(u,t) {=} \mathcal{W}(\{\phi_n(u,t)\} ; \{\psi_n(u,t)\}, \{\sigma_n\}, s(u,t))$. \eqref{eq:thm2_decomp} and \eqref{eq:thm2_decomp_pty} suggest that the 4-D kernel is decomposed into jointly orthogonal sub-channels $\{\psi_n(u,t)\}$ and $\{\phi_n(u',t')\}$.
Therefore, the precoding in Theorem \ref{thm:thm2} can be explained as transmitting the eigenfunctions $\{\phi_n^*(u,t)\}$ after multiplying with specific coefficients $\{x_n\}$.
% 
Consequently, when transmitted through the channel $H$, it transforms $\{\phi_n(u,t)\}$ to its dual eigenfunctions $\{\psi_n(u,t)\}$ with $\{\sigma_n\}$ as in \eqref{eq:them2_duality},
\begin{align}
    \iint k_H(u,t;u',t') \phi_n^*(u', t') ~du' ~dt' {=} \sigma_n \psi_n(u, t).
    \label{eq:them2_duality}
\end{align}
which means that, $H \phi_n^*(u,t){=}\sigma_n \psi_n(u,t)$, as proved in Appendix C-B in \cite{appendix_link}.
% The precoding in Theorem \ref{thm:thm2} can be explained as transmitting the eigenfunctions $\{\phi_n^*(u,t)\}$ after multiplying with specific coefficients\footnote{Although precoding involves a linear combination of $\phi_n^*(u,t)$ with $x_n$ it is a non-linear function ($\mathcal{W}(\cdot)$) with respect to the data signal $s(u,t)$, i.e., $x(u,t) {=} \mathcal{W}(\{\phi_n(u,t)\} ; \{\psi_n(u,t)\}, \{\sigma_n\}, s(u,t))$.} $\{x_n\}$.
% Consequently, when transmitted through the channel $H$, it transforms $\{\phi_n(u,t)\}$ to its dual eigenfunctions $\{\psi_n(u,t)\}$ with $\{\sigma_n\}$ as in \eqref{eq:duality}, i.e., $H \phi_n^*(u,t){=}\sigma_n \psi_n(u,t)$ (as proved in Appendix D-B in \cite{appendix_link}). 
% 
Then the data signal $s(u,t)$ is directly reconstructed at the receiver (to the extent of noise $v_u(t)$) as the net effect of precoding and propagation in the channel ensures that from \eqref{eq:MU}, $r(u,t){=}Hx(u,t){+}v_u(t){\rightarrow}s(u,t){+}v_u(t){=}\hat{s}(u,t)$ using Lemma \ref{lemma:bestprojection}, 
% when precoded with infinite eigenfunctions, 
where $\hat{s}(u,t)$ is the estimated signal. %as $n{\rightarrow}\infty$.}  
%the combination of the precoding coefficients $\{x_n\}$ with {$\{\sigma_n \psi_n(u,t)\}$}.}
% Then, the data signal can be reconstructed at the receiver by combining {$\{\sigma_n \psi_n(u,t)\}$} with the coefficients $\{x_n\}$. 
Therefore, the spatio-temporal decomposition of the channel in Theorem \ref{thm:hogmt} allows us to precode the signal such that all interference in the spacial domain, time domain and joint space-time domain are cancelled when transmitted through the channel, leading to a joint spatio-temporal precoding scheme. 
Further, this precoding ensures that the data signal is reconstructed directly at the receiver with an estimation error that %is equivalent to 
of $v_u(t)$, %the level of AWGN noise, 
thereby completely pre-compensating the spatio-temporal fading/ interference in non-stationary channels to the level of AWGN noise.
Therefore, this precoding does not require complementary decoding at receiver, which vastly reducing its hardware and computational complexity compared to state-of-the-art precoding methods like Dirty Paper Coding (DPC) or linear precoding (that require a complementary decoder \cite{vu2006exploiting}).
% When the channel act on $\{\phi_n(t)\}$, it transfer $\{\phi_n(t)\}$ to another eigenfunctions $\{\psi_n(t)\}$, which can automatic construct the data signal with coefficient $\{\sigma_n\}$ and $\{x_n\}$. The proposed method doesn't need decoding step at receiver.

\begin{comment}
The proof is provided in Appendix D-B in \cite{appendix_link}.
The precoding in Theorem \ref{thm:thm2} involves a linear combination of $\phi_n^*(u,t)$ with coefficients $x_n{=}\frac{\langle s(u,t), \psi_n(u,t) \rangle}{\sigma_n}$, but is a non-linear function ($\mathcal{W}(\cdot)$) with respect to the data signal $s(u,t)$, i.e., $x(u,t) {=} \mathcal{W}(\{\phi_n(u,t)\} ; \{\psi_n(u,t)\}, \{\sigma_n\}, s(u,t))$.
% The proposed precoding method can be interpreted as a function, $x(t) {=} \mathcal{W}(\{\phi_n(t)\} ; \{\psi_n(t)\}, \{\sigma_n\}, s(t))$ which is non-linear with respect to data signal $s(t)$.

The precoding %mechanism 
in Theorem \ref{thm:thm2} can be explained as transmitting the eigenfunctions $\{\phi_n^*(u,t)\}$ after multiplying with specific coefficients $\{x_n\}$ that are calculated corresponding to the desired data signal $s(u,t)$ in \eqref{eq:x}. 
\note{Consequently, when transmitted through the channel $H$, it transforms $\{\phi_n(u,t)\}$ to its dual eigenfunctions $\{\psi_n(u,t)\}$ with $\{\sigma_n\}$. 
% The channel $H$ transforms $\{\phi_n(u,t)\}$ to a different set of eigenfunctions $\{\psi_n(u,t)\}$ with random variables $\{\sigma_n\}$.
% We further observe that combining $\{\psi_n(u,t)\}$ with $\{\sigma_n\}$ and the coefficients $\{x_n\}$ directly reconstructs that data signal $s(u,t)$ as in \eqref{}.
% Consequently, when $\{x_n.\phi_n(u,t)\}$ is transmitted through the channel $H$, $\{x_n.\sigma_n.\psi_n(u,t)\}$ is received at the receiver, which serves as our estimate of the data symbol.
Then, the data signal can be reconstructed at the receiver by combining {$\{\sigma_n \psi_n(u,t)\}$} with the coefficients $\{x_n\}$}. 
Therefore, the spatio-temporal decomposition of the channel in Theorem \ref{thm:hogmt} allows us to precode the signal such that all interference in the spacial domain, time domain and joint space-time domain are cancelled when transmitted through the channel, leading to a joint space-time precoding scheme. 
Further, the proposed precoding does not require complementary decoding at receiver, which vastly reducing its hardware and computational complexity compared to state-of-the-art precoding methods like Dirty Paper Coding (DPC) or linear precoding (that require a complementary decoder \cite{vu2006exploiting}).
% When the channel act on $\{\phi_n(t)\}$, it transfer $\{\phi_n(t)\}$ to another eigenfunctions $\{\psi_n(t)\}$, which can automatic construct the data signal with coefficient $\{\sigma_n\}$ and $\{x_n\}$. The proposed method doesn't need decoding step at receiver.
\end{comment}

\begin{figure}[t]
\begin{subfigure}{.225\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/boxplot.pdf}
  \caption{Distribution of mean channel gains at each time instance. 
%   \note{Say absolute on y-axis.}
  } %at channel delay taps}
  \label{fig:stat}
\end{subfigure}
\begin{subfigure}{.26\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/Joint_space_time_interference.pdf}
  \caption{Channel kernel $k_H(u,t;u',t')$ for $u {=} 1$ and $t {=} 50$}
  \label{fig:joint_interference_kernel}
\end{subfigure}
  \caption{Non-stationary channel statistics and kernel}
  \label{fig:ns_channel}
\end{figure}
% The precoding %mechanism 
% in Theorem \ref{thm:thm2} can be explained as transmitting the eigenfunctions $\{\phi_n^*(u,t)\}$ after multiplying with specific coefficients $\{x_n\}$ that are calculated corresponding to the desired data signal $s(u,t)$ in \eqref{eq:x}. 
% Consequently, when transmitted through the channel $H$, it transforms $\{\phi_n(u,t)\}$ to a different set of eigenfunctions $\{\psi_n(u,t)\}$ with $\{\sigma_n\}$. 
% Then, the data signal can be automatic reconstructed at the receiver by combining the received signal ({$\{\sigma_n \psi_n(u,t)\}$}) with the coefficients $\{x_n\}$. 
% Therefore, the spatio-temporal decomposition of the channel in Theorem \ref{thm:hogmt} allows us to precode the signal such that all interference in the spacial domain, time domain and joint space-time domain are cancelled when transmitted through the channel, leading to a joint space-time precoding scheme. 
% Further, the proposed precoding does not require complementary decoding at receiver, which vastly reducing its hardware and computational complexity compared to state-of-the-art precoding methods like Dirty Paper Coding (DPC) or linear precoding (that require a complementary decoder \cite{vu2006exploiting}).
% % When the channel act on $\{\phi_n(t)\}$, it transfer $\{\phi_n(t)\}$ to another eigenfunctions $\{\psi_n(t)\}$, which can automatic construct the data signal with coefficient $\{\sigma_n\}$ and $\{x_n\}$. The proposed method doesn't need decoding step at receiver.

% \rood{Make the remaining text more direct.}

% \note{Check if relevant. Also don't mention MIMO unless we are doing MIMO. 

\begin{comment}
\textbf{Space domain:} SVD is known to achieve MIMO capacity. However it needs to whiten channel at receiver side, which prevent it from MU-MIMO case, as each user can not obtain the global channel information. 
\end{comment}
% }

% \noindent
% \textbf{Degeneration case:} 
Theorem~\ref{thm:thm2} does not make any assumptions on the type, dimensions or size of the channel kernel. 
% An example application of Theorem \ref{thm:thm2} is shown for  
% To demonstrate the application of Theorem \ref{thm:thm2} to other channel kernels, 
Corollary \ref{col:EP_space} demonstrates the application of Theorem \ref{thm:thm2} to an example of a deterministic multi-user channel where only spatial interference from other users' exist. The received signal is given by $r_u{=}\sum_{u'} h_{u,u'} s_{u'} {+} v_n$ and its continuous form is given by, % in \eqref{eq:h_space},}   
% consider an example of a deterministic (no temporal variation) multi-user where only spatial interference exists. Then the received symbols is given as,
\begin{align}
\label{eq:h_space}
    r(u){=} {\int} k_H (u{,}u') s(u')d u' + v(u)
    % \label{eq:k_H}
\end{align}
% Following the similar precoding method in Theorem~\ref{thm:thm2}, the spatial precoding is given in Corollary~\ref{col:EP_space}.
\begin{corollary}
\label{col:EP_space}
Given a deterministic multi-user channel kernel $k(u,u')$, the precoded signal $x(u)$ that warrants spatial interference-free reception is given by \eqref{eq:xut}. 
\begin{equation}
\label{eq:xut}
    x(u) = \sum_{n{=}1}^\infty \frac{\langle s(u), \psi_n(u) \rangle}{\sigma_n} \phi_n^*(u) 
\end{equation}
where $\{ \sigma_n \}$, $\{ \psi_n\}$ and $\{ \phi_n\} $ follow from Theorem~\ref{thm:hogmt} for the 2-D case, i.e., $k_H(u;u'){=}\sum_{n{=}1}^\infty  \sigma_n \psi_n(u) \phi_n(u')$.
% \begin{equation}
% % k_H(u;u') = \sum_{n}^\infty  \sigma_n \psi_n(u) \phi_n(u')
% \end{equation}
\end{corollary}
%
Proof of Corollary \ref{col:EP_space} is provided in Appendix C-C of \cite{appendix_link}.
The precoding in Corollary \ref{col:EP_space} holds for any other 2-D channel kernels like the stationary/non-stationary single-user channel kernel given by $k_H(t,t')$ by replacing $k_H(u,u')$ with $k_H(t,t')$.
% We also observe that for other 2-D channel kernels like the non-stationary single-user channel kernel given by $k_H(t,t')$, the precoding in Corollary \ref{col:EP_space} still holds by replacing $k_H(u,u')$ with $k_H(t,t')$. %by replacing $u$ and $u'$ with $t$ and $t'$ respectively.
% We also observe that for other 2-D channel kernels like the non-stationary single-user channel kernel given by $k_H(t,t')$, the precoding in Corollary \ref{col:EP_space} still holds by replacing $k_H(u,u')$ with $k_H(t,t')$. %by replacing $u$ and $u'$ with $t$ and $t'$ respectively.
% A similar derivation as Corollary~\ref{col:EP_space} also holds for other 2-D channel kernels. time domain with changing the kernel of time $k_H(u,u')$ to kernel of space $k_H(t,t')$. 
% \noindent
% \textbf{Joint space-time precoding:} unlike SVD which is spatial decomposition and memoryless for time domain while theorem~\ref{thm:GMT} can achieve space-time decomposition which gives opportunity to cancel space-time joint interference. MU-MIMO LTV input-output relation can be expressed as


\begin{comment}
% Consequently, the extension of Theorem~\ref{thm:thm2} to precode signals in the joint space-time domain is given by,
\note{Corollary 2: Temporal Precoding: Say how this degenerate case follows from Theorem 2... If we have results.}
\note{May not need: The time varying response is given by,}
\end{comment}


\begin{comment}
\begin{equation}
\begin{split}
y(t) & = \int_{-\infty}^{\infty} h(t, \tau) x(t-\tau) d \tau\\
 & = \int_{-\infty}^{\infty} \int_{-\infty}^{\infty} S_{H}(\tau, v) x(t-\tau) e^{j 2 \pi v t} d \tau d v
\end{split}
\end{equation}

Where $S_{H}$ is the spreading function of channel $H$. Given $P$ discrete propagation paths and the corresponding gain $h_p$ of path $p$, $S_{H}(\tau,v)$ describes the overall gain associated with all paths of delay $\tau$ and Doppler $v$, and is given by %In WSSUS case, $S_{H}$ is a white process and is given by
\begin{equation}
S_{H}(\tau, v)=\sum_{p=1}^{P} h_{p} \delta(\tau -\tau_p) \delta\left(v-v_{p}\right) .
\end{equation}

For MIMO case, let $\mathbf{x}(t)$ be a $M_T \times 1$ transmit signal vector, and $\mathbf{y}(t)$ be a $M_R \times 1$ receive vector, the input-output relation is $\mathbf{y}(t){=}(\mathbf{Hs})(t)$. 
Assuming uniform linear arrays at the transmitter and the receiver with antenna separation $\Delta_T \lambda_c$ and $\Delta_R \lambda_c$, respectively. The transmit array steering vector $\mathbf{a}_{T}$ for AoA $\theta_A$ and receive array steering vector $\mathbf{a}_{R}$ for AoD $\theta_D$ are given by
\begin{equation}
\mathbf{a}_{T}(\theta_A)=\frac{1}{\sqrt{M_{T}}}\left(\begin{array}{c}
1 \\
e^{-j 2 \pi \Delta_{T} \cos (\theta_A)} \\
\vdots \\
e^{-j 2 \pi\left(M_{T}-1\right) \Delta_{T} \cos (\theta_A)}
\end{array}\right),
\end{equation}

\begin{equation}
\mathbf{a}_{R}(\theta_D)=\frac{1}{\sqrt{M_{\mathrm{R}}}}\left(\begin{array}{c}
1 \\
\mathrm{e}^{-j 2 \pi \Delta_{\mathrm{R}} \cos (\theta_D)} \\
\vdots \\
\mathrm{e}^{-j 2 \pi\left(M_{\mathrm{R}}-1\right) \Delta_{\mathrm{R}} \cos (\theta_D)}.
\end{array}\right).
\end{equation}


The spreading function matrix can be obtained as
\begin{equation}
\mathbf{S}_{\mathbf{H}}(\tau, v)=\sum_{p=1}^{P} \mathbf{H}_{p} \delta\left(\tau-\tau_{p}\right) \delta\left(\nu-v_{p}\right), 
\end{equation}
with $\mathbf{H}_{p}{=}h_{p} \mathbf{a}_{\mathrm{R}}\left(\theta_{D,p}\right) \mathbf{a}_{\mathrm{T}}^{T}\left(\theta_{A,p}\right)$. 

% In non-WSSUS case, $S_{H}$ is a nonwhite process, i.e., scatters with different delay/Doppler are correlated. 

% \begin{equation}
% \mathbf{S}_{\mathbf{H}}(\tau, v)= \mathbf{H}_{p} g\left(\tau-\tau_{0}\right) \Gamma\left(\nu-v_{0}\right).
% \end{equation}

In WSSUS case, spreading function is white process and its 2-D correlation function is given by
\begin{equation}
\mathrm{E}\left\{\mathbf{S}_{\mathbf{H}}(\tau, \nu) \mathbf{S}_{\mathbf{H}}^{H}\left(\tau^{\prime}, \nu^{\prime}\right)\right\}=\mathbf{C}_{\mathbf{H}}(\tau, \nu) \delta\left(\nu-\nu^{\prime}\right) \delta\left(\tau-\tau^{\prime}\right)
\end{equation}
where, $\mathbf{C}_{\mathbf{H}}$ is the scattering function matrix. 

In non-WSSUS case, the channel correlations/nonstationarities can be described via the 4-D correlation function
\begin{equation}
R_{S}(\tau, \nu ; \Delta \tau, \Delta \nu) \triangleq \mathrm{E}\left\{S_{\mathbf{H}}(\tau, \nu+\Delta \nu) S_{\mathbf{H}}^{*}(\tau-\Delta \tau, \nu)\right\}
\end{equation}

The local scattering function (LSF) is defined as
\begin{equation}
\begin{array}{l}
\mathcal{C}_{\mathbf{H}}(t, f ; \tau, \nu) \triangleq \iint R_{S}(\tau, \nu ; \Delta \tau, \Delta \nu) \mathrm{e}^{j 2 \pi(t \Delta \nu-f \Delta \tau)} \mathrm{d} \Delta \tau \mathrm{d} \Delta \nu
\end{array}
\end{equation}

For WSSUS channel, the LSF is consistent with the scattering function, $\mathcal{C}_{\mathbf{H}}(t, f ; \tau, \nu){=}C_{\mathbf{H}}(\tau, \nu)$. 

\end{comment}
% \inred{
% \noindent
% \textbf{To address:}\\
% 1. How to enforce orthogonality of eigenfunctions in the time-frequency domains.\\
% 2. Is it feasible to address temporal THP.\\

% }

\begin{comment}
\note{\noindent
How to get CSI:

OTFS paper gives twist convolution lemma and  delay-Doppler input-output relation theorem. Matzs' paper gives second order statistic I/O relation of non-WSSUS channel. Do convolution at receiver with channel $S(\tau,\nu)$, if we can get $S(t,f;\tau,\nu)$ and prove the theorem of non-WSSUS I/O relation 
\begin{align}
   r(t,f) = \iint S_H(t, f; \tau, \nu) s(\tau,\nu) ~d\tau ~dv
\end{align}
Then we can do precoding with CSI $S_H(\tau, \nu)$. $S_H(t, f; \tau, \nu)$ should be the second order of $h(t, f; \tau, \nu)$ and $C(t,f;\tau, \nu)$ should be $\mathbb{E}\{S_H(t, f; \tau, \nu)\}$.

Moreover, if above theorem can be proved, in section~\ref{sec:Precoding}, we can use the same technique to deal with two kinds of CSI. 

\begin{itemize}
    \item Given SCI $S_H(t,f; \tau, \nu)$, we can achieve least square error $\|s(t,f) {-} Hx(t,f) \|^2$ with minimal power.
    \item Given statistic CSI $C_H(t,f;\tau,\nu)$, we can achieve least square error for average signal $\|\mathbb{E}\{s(t,f)\} {-} \mathbb{E}\{Hx(t,f\}\|^2$ with minimal power. (The performance is not good as minimal $\|s(t,f) {-} Hx(t,f) \|^2$, because CSI is relaxed to statistics CSI. Consider there is no precoding technique can deal with statistics CSI for NS channel, it's worth a try)
\end{itemize}
}
\end{comment}


==> primer.tex <==
\section{Primer \& Motivation}
\label{sec:primer}

\begin{figure}[h]
    \centering
    \includegraphics[width=2.5in]{figures/joint_trilemma.pdf}
    \caption{Comparison with existing methods. Notation: Technology/Modulation -- Technique/Decomposition}
    \label{fig:joint_trilemma}
\end{figure}

Motivate the following with evidence from literature or using analysis or toy examples. 

\subsection{Why Joint Space-Time-Frequency Precoding?}
\note{
Mention why not seperate precoding/ equalization. Why would these fail: e.g., joint IUI-ICI-ISI cancelation. 

What is ISI here? For OFDM it can be due to time-varying ICI or residual ISI because of limited CP or ISI due to IUI or IAI.

\note{Time-varying ICI is actually NS (frequency-varying ISI is also NS), since the Doppler spread/ shift (relative acceleration) changes over time. See figures ~\ref{fig:fig2},\ref{fig:fig3},\ref{fig:fig4}.}

\begin{figure}{h}
    \centering
    \includegraphics[width=3.5in]{figures/fig3.png}
    \caption{\inred{fig2}}
    \label{fig:fig2}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=3.5in]{figures/fig4.png}
    \caption{\inred{fig2}}
    \label{fig:fig3}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=3.5in]{figures/fig2.png}
    \caption{\inred{Just a place holder: We will show this using a toy example.}}
    \label{fig:fig4}
\end{figure}
}

\inred{\textbf{Stationary channel precoding know the ICI}, but they will also transmit multiple OFDM symbles within one precoding, which means each packet data over different k is precoded with same ICI.}

\note{
- Notice that for different subcarriers $p$, the delay-Doppler can change with time, and consequently the ISI changes over frequency. 
The frequency-varying ISI and time-varying ICI are both caused by NS variations in the channel.


- Joint ICI-ISI means if $s(k_1,p_1)$ has ICI $\Delta c_{k_1,p_1-p_2}$ to $s(k_1,p_2)$ and $s(k_1,p_2)$ has ISI $\Delta s_{p_2,k_1-k_2}$ to $s(k_2,p_2)$, then $\Delta c_{k_1,p_2-p_1}$ will also has ISI $\Delta cs_{(k_1,p_1)-(k_2,p_2)}$ to $s(k_2,p_2)$. $\Delta cs_{(k_1,p_1)-(k_2,p_2)}$ called joint ICI-ISI from $s(k_1,p_1)$ to $s(k_2,p_2)$. 

- Joint ISI-ICI is similar. First $s(k_1,p_1)$ give ISI to $s(k_2,p_1)$, and then this ISI also has ICI to $s(k_2,p_2)$, which is ISI-ICI from $s(k_1,p_1)$ to $s(k_2,p_2)$.  

- To simplify, we combined them and call it joint time-frequency interference.

- It's straightforward to combine it with IUI.

- Note: We use CP to reduce ISI and we can also use CP at frequency domain to reduce ICI, but both of them will increase overhead.
}

\subsection{Why Eigenfunctions?}

\note{
Mention why not eigenvectors or anything like THP, and where exactly would these fall short?

If NS, then eigenfunctions are already motivated. Just mention the model as in our previous model and preliminaries.
}


\subsection{Tensor Notations \& Algebra}













%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%OLD MODEL%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
% \newpage
\section{Models and Preliminaries}
\label{sec:model}
% \vspace{-10pt}
% \noindent
% \textbf{Notations:}
The basic communications system consists of a transmitter, a channel, and a receiver.
At the transmitter, the uncoded messages, $m{\in}[1,M]$ are modulated and the symbols, $s_m$ are transmitted over the channel, where $M$ is the order of the modulation scheme. 
The stochastic behavior of the wireless channel is represented by the conditional likelihood of receiving a random vector $\boldsymbol{r}$ when symbol ${s}_m$ is transmitted, i.e., $p(\boldsymbol{r}{\mid}{s}_m)$ \cite{Proakis2007Book}.
% $d$ is the dimensionality of $\boldsymbol{r}$ and typically $d{=}2K$ which consists of streams of I/Q samples for each $K$, where $K$ is the number of antennas at the receiver.
In general, %the received vector, 
$\boldsymbol{r}{\in}\mathbb{R}^{2K}$ consists of real and imaginary streams for each antenna $k{\in}[1,K]$, where $K$ is the number of antennas at the receiver.
% The transmitter communicate one out of M possible messages s ∈ M = {1, 2,..., M} to the receiver making n discrete uses of the channel. 
% Let {\tmap} and {\tnn} represent a classical MAP-based and NN-based receiver respectively as shown in figure \ref{fig:whole}. 
Upon reception of $\boldsymbol{r}$, {\tmap} and {\tnn} receivers apply the transformations $\fmap$ and $\fnn$ to produce the estimates $\mmap$ and $\mnn$ of the transmitted message.
    % Let {\tmap} and {\tnn} represent a classical MAP-based and NN-based receiver respectively as shown in figure \ref{fig:whole}. 
    % The stochastic behaviour of the wireless channel is represented by the conditional likelihood of receiving a random vector $\boldsymbol{r}$ when symbols ${s}_m$ is transmitted, i.e., $p(\boldsymbol{r}{\mid}{s}_m)$ \cite{Proakis2007Book}. %The input to the receiver is $\boldsymbol{r}$ and the goal of a 
% {\tmap} and {\tnn} detect the transmitted symbols and the messages, $\mmap$ and $\mnn$ from the uncoded signal that is corrupted by the channel. 
% a noisy version of the codeword is received and the task of the decoder is to recover the corresponding information bits. 
% The design of capacity achieving and deterministic coding, modulation and signal processing schemes for the transmitter have been well-studied, therefore, we believe that the opportunities for improvement are at the receiver, where taming the unknown stochasticity of the channel is still an issue. 
The benefits of coding are complementary to this work, and yield an added gain in the error rate using existing coding schemes. 
% In comparison to iterative decoding, 

\noindent  
\textbf{Classical Receiver:}    
An optimal {\tmap} receiver using conventional classical theory strives to achieve minimum probability of error, also referred to as the \textit{Bayesian Risk} given by $P_{e}{=}\mathrm{P}[\hat{m}{\neq}m]$, by maximizing the posterior probability (MAP) to estimate the most likely transmitted symbol 
% $\hat{m}={ \arg \max }_m\  \mathrm { P } \left[ \boldsymbol {s_m } | \boldsymbol {r} \right]$
or the likelihood under the assumption of equal prior.
% $\hat { m } = { \arg \max }_m\  \mathrm { P } ( \boldsymbol { r } | \boldsymbol { s_m } )$, 
% Alternately, {\tmap} %optimum receiver is one which 
% achieves in the minimum probability of error also referred to as the \textit{Bayesian Risk} given by $P_{err}{=}P[\hat{m}{\neq} m]$, which is achieved by the maximum a posteriori probability (MAP) receiver, {\tmap} (or equivalently the maximum likelihood receiver under equal prior probabilities of $s_m$). 
The estimated message $\mmap$ of {\tmap} is given by,
\begin{align}
    %\mmap=\argmax_{m} \mathrm{P}[s_m\mid\boldsymbol{r}],\  m{\in}[1,M]
    {\mmap}{=}{\argmax_{m}}\fmap(\boldsymbol{r}); \ %\text{where,} \ 
    \fmap(\boldsymbol{r}){:=}\mathrm{P}[s_m{\mid}\boldsymbol{r}], %\  m{\in}[1,M]
    \label{eq:MAP_receiver}
\end{align}
% where, $\boldsymbol{r}$  is the received symbol vector for the transmitted symbol, $\boldsymbol{s_m}$, and 
% where $M$ is the order of the modulation scheme of the transmitted symbols. 
% Figure \ref{fig:whole} shows the modular block structure of the {\tmap} receiver, where the signal processing is split into a chain of independent blocks, each executing a well-defined isolated function (\eg channel estimation, equalization and detection). This modular approach has led to the optimal, versatile and controllable classical communication systems we have today.
% We show that a single feed forward deep neural network as shown in figure \ref{fig:whole} can replace the entire classical receiver while achieving equivalent error rate of classical receivers.     
% 
% 
% 
% \note{
where $\fmap(\boldsymbol{r})$ denotes the mapping from the input $\boldsymbol{r}$ to the output of {\tmap} and is equal to the posterior probability of each symbol, $s_m$. 
% , that maximizes the posterior distribution $p(f(\boldsymbol{r}) \mid \boldsymbol{r})$ as in \eqref{eq:f_MAP},
% \begin{align}
% \fmap(\boldsymbol{r})=\argmax_{f} p(f(\boldsymbol{r}) \mid \boldsymbol{r})   
% \label{eq:f_MAP}
% \end{align}
% Alternatively $\fmap(\boldsymbol{r})$ is the function that achieves the minimum Bayesian risk $\mathcal{R}(f)$ given by \eqref{eq:risk_MAP}, 
% \begin{align}
% \mathcal{R}_{MAP}:=\mathcal{R}(\fmap)=\inf_{f} \mathcal{R}(f)
% \label{eq:risk_MAP}
% \end{align}
% where the infimum is over all measurable functions $f{\in}\mathbb{R}$.
% However, a closed-form expression for $\fmap(\boldsymbol{r})$ does not often exist for various channel conditions \cite{Proakis2007Book} and consequently the {\tmap} receiver, is in general non-optimal and computationally prohibitive. 
% While the {\tmap} receiver is theoretically optimal in minimizing the BER, it requires mathematically accurate channel models, and for most channel conditions there exists no computationally tractable (polynomial-time) algorithms for practical realization \cite{simeone2018very}. 
While the low-complexity nearest neighbour symbol detection algorithm is provably optimal for Additive white Gaussian noise (AWGN) channels, there is a lack of closed-form expressions for $\fmap(\boldsymbol{r})$ for most practical channels (\eg with unknown or non-Gaussian distributions) \cite{Proakis2007Book}.
% While {\tmap} is theoretically optimal in minimizing the BER, it requires mathematically accurate channel models, and for most practical channels, a closed-form expression for $\fmap(\boldsymbol{r})$ does not exist and consequently is computationally prohibitive for practical realization \cite{simeone2018very}. 
% For example, although the low-complexity nearest neighbour decoding algorithm for symbol detection is provably optimal for Additive white Gaussian noise (AWGN) channels, there is a lack of computationally tractable and optimal algorithms for unknown or non-Gaussian channels \cite{Proakis2007Book}.
Moreover, the complexity of {\tmap} grows exponentially with the number of antennas and constellation size \cite{MAP_complexity}, and consequently the {\tmap} receiver is often computationally prohibitive %(lacks polynomial time algorithms)
for practical realization and requires mathematically accurate channel models for optimal realization.
% Hence, the benefit of achieving equivalence in this category is to implement low-complexity NN algorithms. 
% Figure \ref{fig:whole} shows the modular block structure of the {\tmap} receiver, where the signal processing is split into a chain of independent blocks, each executing a well-defined isolated function (\eg channel estimation, equalization and detection). This modular approach has led to the optimal, versatile and controllable classical communication systems we have today.
Therefore, practical implementations of {\tmap} relies on a modular structure with additional signal processing blocks, (\eg Channel estimation and Equalization) as shown in figure \ref{fig:whole}, to whiten the noise by estimating and mitigating distortions due to fading and interference, to employ the nearest neighbour decoder. 
However, we show that there exists a {\tnn} receiver that is equivalent to {\tmap}, which is determined by learning a deterministic mapping function $\fnn(\boldsymbol{r})$ and hence is computationally tractable.
% Let $\fmap(\boldsymbol{r})$ denote the mapping from the input to the {\tmap} receiver, $\boldsymbol{r}$ to its output $\mmap$, that maximizes the posterior distribution $p(f(\boldsymbol{r}) \mid \boldsymbol{r})$ as in \eqref{eq:f_MAP},
% \begin{align}
% \fmap(\boldsymbol{r})=\argmax_{f} p(f(\boldsymbol{r}) \mid \boldsymbol{r})   
% \label{eq:f_MAP}
% \end{align}
% Alternatively $\fmap(\boldsymbol{r})$ is the function that achieves the minimum Bayesian risk $\mathcal{R}(f)$ given by \eqref{eq:risk_MAP}, 
% \begin{align}
% \mathcal{R}_{MAP}:=\mathcal{R}(\fmap)=\inf_{f} \mathcal{R}(f)
% \label{eq:risk_MAP}
% \end{align}
% where the infimum is over all measurable functions $f{\in}\mathbb{R}$.
% Unfortunately a closed-form expression for $\fmap(\boldsymbol{r})$ does not often exist for various channel conditions \cite{Proakis2007Book} and hence the above optimization is computationally prohibitive. However, we show that it is possible to find a NN equivalent of {\tmap} denoted by {\tnn} which is determined by a deterministic mapping function $\fnn(\boldsymbol{r})$, and hence is computationally tractable.
% }




    % The overall goal of the wireless receiver is to observe the received vector $\boldsymbol{r}$ and after certain signal processing (\eg channel estimation and channel equalization) make an optimal decision about which message $m$, $1{\leqslant} m{\leqslant}M$ was transmitted, where $M$ is the order of the modulation scheme. An optimum decision is one which results in the minimum error probability given as $P_{err}{=}P[\hat{m}{\neq} m]$, which is referred to as the maximum a posteriori probability (MAP) rule (or equivalently the maximum likelihood rule under equal prior probabilities of $s_m$). 
%     The estimated message $m$ of the MAP receiver is given by,
% \begin{align}
%     \mmap=\argmax_{m} p(s_m|\boldsymbol{r}), m=1,2, \ldots M
%     \label{eq:MAP_receiver}
% \end{align}

% An optimal receiver using conventional communication theory strives to maximize the posterior probability to estimate the most likely transmitted symbol 
% %$\hat { m } = \underset { 1 \leq m \leq M } { \arg \max }_m\  \mathrm { P } \left[ \boldsymbol {s_m } | \boldsymbol {r} \right]$ 
% $\hat { m } = { \arg \max }_m\  \mathrm { P } \left[ \boldsymbol {s_m } | \boldsymbol {r} \right]$
% or the likelihood under the assumption of equal prior, 
% %$\hat { m } = \underset { 1 \leq m \leq M } { \arg \max }\  \mathrm { P } ( \boldsymbol { r } | \boldsymbol { s_m } )$, where, $\boldsymbol{r}$ 
% $\hat { m } = { \arg \max }_m\  \mathrm { P } ( \boldsymbol { r } | \boldsymbol { s_m } )$, where, $\boldsymbol{r}$ 
% is the received symbol for the transmitted symbol, $\boldsymbol{s_m}$. 
% An optimum decision is one which achieves the minimum probability of error also referred to as the \textit{Bayesian Risk} given by $P_{err}{=}P[\hat{m}{\neq} m]$, which is obtained by the maximum posteriori probability (MAP) rule. 
% Figure \ref{fig:sys} shows the modular block structure of the optimal MAP receiver, {\tmap}: One of the guiding principles of classical receiver design is to split the signal processing into a chain of multiple independent blocks; each executing a well defined and isolated function (e.g., source/channel coding, modulation, channel estimation, equalization). This modular approach has led to the optimal, versatile and controllable classical communication systems we have today.
% We show that a single feed forward deep neural network can replace the entire classical receiver while achieving equivalent error rate of classical receivers. 
% In neural network terms, $P_{err}$ is referred to as the \textit{Bayesian risk} \cite{ML_Probability_book_Murphy} that is analogous to a measure of the Bit Error Rate (BER). 
% We define and design the {\tnn} that is equivalent to the optimal classical receiver, {\tmap} that achieves provable performance guarantees in terms of BER and model complexity. This is achieved by deriving the loss function of {\tnn} that guarantees the equivalence individually and collectively with each block of {\tmap} and implementing the corresponding equivalent optimum structure of {\tnn}.
% Figure \ref{fig:sys} shows the modular block structure of {\tmap}: One of the guiding principles of communications systems design is to split the signal processing into a chain of multiple independent blocks; each executing a well defined and isolated function (e.g., source/channel coding, modulation, channel estimation, equalization). This modular approach has led to the optimal, versatile and controllable classical communication systems we have today. Thus, we start by designing the equivalent structure of {\tnn} for each communication block as in figure \ref{fig:sys} and then focus on the end-to-end architecture of {\tnn} to jointly optimize the end-to-end system. 


% \noindent
% \textbf{Notations:}
%     Let {\tnn} and {\tmap} represent a NN-based receiver and a classical MAP receiver respectively. 
%     The most general wireless channel model is to represent it as a conditional likelihood of receiving a random vector $\boldsymbol{r}$ when symbols $\mathbf{s}_m$ is transmitted, i.e., $p(\boldsymbol{r}|\mathbf{s}_m)$ \cite{Proakis2007Book}. %The input to the receiver is $\boldsymbol{r}$ and the goal of a 
%     The overall goal of the wireless receiver is to observe the received vector $\boldsymbol{r}$ and after certain signal processing (\eg channel estimation and channel equalization) make an optimal decision about which message $m$, $1{\leqslant} m{\leqslant}M$ was transmitted, where $M$ is the order of the modulation scheme. An optimum decision is one which results in the minimum error probability given as $P_{err}{=}P[\hat{m}{\neq} m]$, which is referred to as the maximum a posteriori probability (MAP) rule (or equivalently the maximum likelihood rule under equal prior probabilities of $s_m$). 
%     The estimated message $m$ of the MAP receiver is given by,
% \begin{align}
%     \mmap=\argmax_{m} p(s_m|\boldsymbol{r}), m=1,2, \ldots M
%     \label{eq:MAP_receiver}
% \end{align}

    % The error probability $P_{err}$ is referred to as the \textit{Bayesian risk} \cite{ML_Probability_book_Murphy} or the Bit Error Rate (BER) \cite{Proakis2007Book}.
    % The objective is to first design the optimal receiver of the {\tnn}, by establishing the equivalence between {\tnn} and {\tmap} at the receiver.
    % We consider the equivalent design of the various components of the receiver: a) Channel Estimation, b) Channel Equalization, and c) Symbol Detection (Decoding).

% The optimal classical transceiver {\tmap} relies on the maximum a posteriori (MAP) estimator or predictor which is determined by finding the mapping $\fmap(\boldsymbol{r})$ of the input $\boldsymbol{r}$ that maximizes the posterior distribution $p(f(\boldsymbol{r}) \mid \boldsymbol{r})$ as in \eqref{eq:f_MAP},
% \begin{align}
% \fmap(\boldsymbol{r})=\argmax_{f} p(f(\boldsymbol{r}) \mid \boldsymbol{r})   
% \label{eq:f_MAP}
% \end{align}
% Alternatively $\fmap(\boldsymbol{r})$ is the function that achieves the minimum Bayesian risk $\mathcal{R}(f)$ given by \eqref{eq:risk_MAP}, 
% \begin{align}
% \mathcal{R}_{MAP}:=\mathcal{R}(\fmap)=\inf_{f} \mathcal{R}(f)
% \label{eq:risk_MAP}
% \end{align}
% where the infimum is over all measurable functions $f{\in}\mathbb{R}$.
% Unfortunately a closed-form expression for $\fmap(\boldsymbol{r})$ does not often exist for various channel conditions \cite{Proakis2007Book} and hence the above optimization is computationally prohibitive. However, we show that it is possible to find a NN equivalent of {\tmap} denoted by {\tnn} which is determined by a deterministic mapping function $\fnn(\boldsymbol{r})$, and hence is computationally tractable.
\noindent
\textbf{Neural Network based Receiver:}
The {\tnn} receiver is derived by training a NN model to determine its parameters, $\delta_n^*$ that minimizes an \textit{Empirical risk}, ${\mathcal{R}}(\fnn(\boldsymbol{r};\delta_n))$ for a given training dataset $\mathcal{D}$ by using \eqref{eq:NN_risk},
\begin{align}
\label{eq:NN_risk}
&{\delta_n^{*}}{=}\argmin_{\delta_n}\left[{\mathcal{R}}(\fnn(\boldsymbol{r};\delta_n))\right]  \ \text{where,} \\ 
&\mathcal{R}(\fnn(\boldsymbol{r};\delta_n)){=}\frac{1}{n}\sum_n[\mathcal{L}(\fnn(\boldsymbol{r};\delta_n))]\nonumber
% \tilde{\mathcal{R}}(\mathcal{D}, \delta) &= \left[\mathcal{R}(\mathcal{D}, \delta)+ C(\delta)\right]   &&\text{and,} \enskip %\\    
% \mathcal{R}(\mathcal{D}, \delta) = \mathbb{E}[\mathcal{L}(\mathcal{D}, \delta)]
% {\delta}^{*}&=\argmin_{\delta}\left[\tilde{\mathcal{R}}(\mathcal{D}, \delta)\right] \quad &&\text{where,}\\
% \tilde{\mathcal{R}}(\mathcal{D}, \delta) &= \left[\mathcal{R}(\mathcal{D}, \delta)+ C(\delta)\right]  \quad &&\text{and,}\\    
% \mathcal{R}(\mathcal{D}, \delta) &= \mathbb{E}[\mathcal{L}(\mathcal{D}, \delta)]
% \hat{\delta}_{\lambda}&=\argmin_{\delta}\left[\tilde{\mathcal{R}}(\mathcal{D}, \delta)\right]
% \fnn(x,\delta)&=\sigma\left(\mathbf{W}_{\ell} \boldsymbol{r}_{\ell-1}+\mathbf{b}_{\ell}\right)    
\end{align}
where $\mathcal{R}(f_{NN}(\boldsymbol{r};\delta_n))$ is the average value of a loss function, $\mathcal{L}(f_{NN}(\boldsymbol{r};\delta_n))$,  $\fnn$ is the mapping from the inputs $\boldsymbol{r}$ to the outputs of the {\tnn} receiver, and $n{=}|\mathcal{D}|$ is the number of training samples.
% and , where $\mathbb{E}[.]$ is the expectation with respect to the underlying probability distribution of the channel. 
$\mathcal{R}(\fnn(\boldsymbol{r};\delta_n))$ is an empirical measure of the error in the estimated and true symbols of the {\tnn} receiver such as the mean absolute error, mean-squared error (MSE) or the cross-entropy loss \cite{ML_Probability_book_Murphy}. 
% The parameters, $\delta^*$ are determined by 
Gradient descent and the backpropagation algorithm \cite{ML_Probability_book_Murphy} is used to determine the parameters, ${\delta_n^{*}}$ 
%and the mapping, $\fnn$ 
that minimizes \eqref{eq:NN_risk} among all possible parameters with $n$ training samples, $\delta_n$. 
% \eqref{eq:NN_risk} is minimized %the risk function 
% over the training set, $\mathcal{D}$ by using gradient descent and the backpropagation algorithm \cite{ML_Probability_book_Murphy} to determine parameters, $\delta^*$.
% \eqref{eq:NN_risk} is minimized %the risk function 
% over the training set, $\mathcal{D}$ by using gradient descent and the backpropagation algorithm \cite{ML_Probability_book_Murphy} to determine parameters, $\delta^*$.
% The parameters, $\delta^*$ are determined by minimizing the risk function over the training set, $\mathcal{D}$ by using gradient descent and the backpropagation algorithm \cite{ML_Probability_book_Murphy}. 
%and is a measure of the Bayesian Risk. 
% $C(\delta)$ is a measure of the complexity of the {\tnn} receiver such as the norm-loss $\|\delta\|$, and trades-off the accuracy with the complexity of the {\tnn} receiver \cite{ML_Probability_book_Murphy}. 
% $\lambda$ is a parameter that can be tuned to trade-off the accuracy and complexity of the NN \cite{ML_Probability_book_Murphy}.
% Typical examples of $\mathcal{R}(\mathcal{D}, \delta)$ are the mean absolute error, mean-squared error (MSE) and the cross-entropy, while examples of $C(\delta)$ include the L1 norm or L2 norm of the NN parameters. 

\end{comment}

\begin{comment}
\noindent
\textbf{Neural Network based Receiver:}
The {\tnn} receiver is derived by training a NN model to determine its parameters, $\delta^*$ that minimizes an Empirical risk function, ${\mathcal{R}}(\mathcal{D}, \delta_n)$ for given training dataset $\mathcal{D}$ by using \eqref{eq:NN_risk},
\begin{align}
\label{eq:NN_risk}
{\delta}^{*}{=}\argmin_{\delta_n}\left[{\mathcal{R}}(\mathcal{D}; \delta_n)\right]  \enskip \text{where,} \enskip 
\mathcal{R}(\mathcal{D}; \delta_n){=}\frac{1}{n}\sum_n[\mathcal{L}(\mathcal{D}; \delta_n)]
% \tilde{\mathcal{R}}(\mathcal{D}, \delta) &= \left[\mathcal{R}(\mathcal{D}, \delta)+ C(\delta)\right]   &&\text{and,} \enskip %\\    
% \mathcal{R}(\mathcal{D}, \delta) = \mathbb{E}[\mathcal{L}(\mathcal{D}, \delta)]
% {\delta}^{*}&=\argmin_{\delta}\left[\tilde{\mathcal{R}}(\mathcal{D}, \delta)\right] \quad &&\text{where,}\\
% \tilde{\mathcal{R}}(\mathcal{D}, \delta) &= \left[\mathcal{R}(\mathcal{D}, \delta)+ C(\delta)\right]  \quad &&\text{and,}\\    
% \mathcal{R}(\mathcal{D}, \delta) &= \mathbb{E}[\mathcal{L}(\mathcal{D}, \delta)]
% \hat{\delta}_{\lambda}&=\argmin_{\delta}\left[\tilde{\mathcal{R}}(\mathcal{D}, \delta)\right]
% \fnn(x,\delta)&=\sigma\left(\mathbf{W}_{\ell} \boldsymbol{r}_{\ell-1}+\mathbf{b}_{\ell}\right)    
\end{align}
where the \textit{Empirical risk} function $\mathcal{R}(\mathcal{D}, \delta)$ is the expected value of the loss function $\mathcal{L}(\mathcal{D}, \delta_n)$, $\fnn$ is the mapping from the inputs $\boldsymbol{r}$ to the outputs of the {\tnn} receiver, 
and $n{=}|\mathcal{D}|$ is the number of training samples.
% and , where $\mathbb{E}[.]$ is the expectation with respect to the underlying probability distribution of the channel. 
$\mathcal{R}(\mathcal{D}, \delta_n)$ is an empirical measure of the error in the estimated and true symbols of the {\tnn} receiver such as the mean absolute error, mean-squared error (MSE) or the cross-entropy loss \cite{ML_Probability_book_Murphy}.  %and is a measure of the Bayesian Risk. 
% $C(\delta)$ is a measure of the complexity of the {\tnn} receiver such as the norm-loss $\|\delta\|$, and trades-off the accuracy with the complexity of the {\tnn} receiver \cite{ML_Probability_book_Murphy}. 
% $\lambda$ is a parameter that can be tuned to trade-off the accuracy and complexity of the NN \cite{ML_Probability_book_Murphy}.
% Typical examples of $\mathcal{R}(\mathcal{D}, \delta)$ are the mean absolute error, mean-squared error (MSE) and the cross-entropy, while examples of $C(\delta)$ include the L1 norm or L2 norm of the NN parameters. 
\end{comment}

\begin{comment}
\noindent
\textbf{Neural Network based Receiver:}
Training a {\tnn} receiver involves finding the NN model (with parameters $\delta^*$) that minimizes a regularized risk, $\tilde{\mathcal{R}}(\mathcal{D}, \delta)$ for given training dataset $\mathcal{D}$ by using \eqref{eq:NN_risk},
\begin{align}
\label{eq:NN_risk}
{\delta}^{*}&=\argmin_{\delta}\left[\tilde{\mathcal{R}}(\mathcal{D}, \delta)\right]  &&\text{where,}\\
\tilde{\mathcal{R}}(\mathcal{D}, \delta) &= \left[\mathcal{R}(\mathcal{D}, \delta)+ C(\delta)\right]   &&\text{and,} \enskip %\\    
\mathcal{R}(\mathcal{D}, \delta) = \mathbb{E}[\mathcal{L}(\mathcal{D}, \delta)]
% {\delta}^{*}&=\argmin_{\delta}\left[\tilde{\mathcal{R}}(\mathcal{D}, \delta)\right] \quad &&\text{where,}\\
% \tilde{\mathcal{R}}(\mathcal{D}, \delta) &= \left[\mathcal{R}(\mathcal{D}, \delta)+ C(\delta)\right]  \quad &&\text{and,}\\    
% \mathcal{R}(\mathcal{D}, \delta) &= \mathbb{E}[\mathcal{L}(\mathcal{D}, \delta)]
% \hat{\delta}_{\lambda}&=\argmin_{\delta}\left[\tilde{\mathcal{R}}(\mathcal{D}, \delta)\right]
% \fnn(x,\delta)&=\sigma\left(\mathbf{W}_{\ell} \boldsymbol{r}_{\ell-1}+\mathbf{b}_{\ell}\right)    
\end{align}
where the \textit{Empirical risk} function $\mathcal{R}(\mathcal{D}, \delta)$ is the expected value of the loss function $\mathcal{L}(\mathcal{D}, \delta)$, and Let $\fnn$ denote the mapping from the inputs $\boldsymbol{r}$ to the outputs of the {\tnn} receiver. $\mathcal{R}(\mathcal{D}, \delta)$ is an empirical measure of the error in the estimated and true symbols of the {\tnn} receiver such as the mean absolute error, mean-squared error (MSE) or the cross-entropy loss.  %and is a measure of the Bayesian Risk. 
$C(\delta)$ is a measure of the complexity of the {\tnn} receiver such as the norm-loss $\|\delta\|$, and trades-off the accuracy with the complexity of the {\tnn} receiver \cite{ML_Probability_book_Murphy}. 
% $\lambda$ is a parameter that can be tuned to trade-off the accuracy and complexity of the NN \cite{ML_Probability_book_Murphy}.
% Typical examples of $\mathcal{R}(\mathcal{D}, \delta)$ are the mean absolute error, mean-squared error (MSE) and the cross-entropy, while examples of $C(\delta)$ include the L1 norm or L2 norm of the NN parameters. 

% 
% 
% Let $\fnn$ denote the mapping from the inputs $\boldsymbol{r}$ to the outputs of the {\tnn} receiver.
For a fully-connected feed-forward deep neural network of depth $L$, $\fnn$ is a composition of $L$ functions, ${f}_{1}{,\ldots,}{f}_{L}$, that describe the transitions between neurons via $L{-}1$ intermediate hidden layers. 
Each function ${f}_{l}$ is determined by the parameters $\delta_{n,l}{=}\left\{\boldsymbol{W}_{l}, \boldsymbol{b}_{l}\right\}$ and modeled as $f_{l}\left(\boldsymbol{u}_{l-1};\delta_{l}\right){=}\phi_{l}\left(\boldsymbol{W}_{l} \boldsymbol{u}_{l-1}{+}\boldsymbol{b}_{l}\right)$, where $\boldsymbol{W}_{l}$ is the weight matrix, $\boldsymbol{b}_{l}$ is the bias vector, and $\phi_{l}$ is a non-linear function referred to as an activation function.
% , that is critical to improving the expressive power of NNs. 
% Each function ${f}_{l}$ is determined by the parameters $\delta_{l}{=}\left\{\boldsymbol{W}_{l}, \boldsymbol{b}_{l}\right\}$ and modeled as $f_{l}\left(\boldsymbol{u}_{l-1};\delta_{l}\right){=}\phi_{l}\left(\boldsymbol{W}_{l} \boldsymbol{u}_{l-1}{+}\boldsymbol{b}_{l}\right)$, where $\boldsymbol{W}_{l}$ is the weight matrix, $\boldsymbol{b}_{l}$ is the bias vector, and $\phi_{l}$ is a non-linear function that is called an activation function. 
$\boldsymbol{u}_{l-1}$ is the input to the $l$\textsuperscript{th} layer and $\boldsymbol{u}_{0}{=}\boldsymbol{r}$.
% Then the NN function $\fnn$ that describes the mapping of {\tnn} from input to output is given by \eqref{eq:f_NN},
% From the above notations 
Therefore, $\fnn$ is given by \eqref{eq:f_NN},
\begin{align}
\label{eq:f_NN}
\fnn(\boldsymbol{r};\delta_n)={f}_{L}\left({\ldots}\left({f}_{2}\left({f}_{1}\left(\boldsymbol{r}{;}{\delta}_{n,1}\right){;}{\delta}_{n,2}\right){\ldots}\right){;} {\delta}_{n,L}\right)
% &\text{where,} \ \delta_n{=}\{\delta_{n,l}\}, \ l{\in}[1,L]
\end{align}
% 
% \noindent
% \textbf{Step 1:} We initially design the risk term $\mathcal{R}(\mathcal{D}, \delta)$ to achieve equivalence of {\tnn} and {\tmap} in Section \ref{sec:equivalence}.\\
% % The structural risk minimization principle \cite{ML_Probability_book_Murphy} is often used to determine $\lambda$ as $\hat{\lambda}=\underset{\lambda}{\operatorname{argmin}} \hat{\mathcal{R}}\left(\hat{\delta}_{\lambda}\right)$ where $\hat{\mathcal{R}}(\delta)$ is an estimate of the risk. We use theoretical upper bounds on the risk to determine $\lambda$ in the generalization bounds section.\\
% \textbf{Step 2:} We determine the BER and complexity bounds for {\tnn} in Section \ref{sec:generalization}.\\
% \textbf{Step 3:} Next we use the above results to design the inverse architecture of {\tnn} for certain performance guarantees in Section \ref{sec:inverse_design}.\\
% \textbf{Step 4:} Finally we the design of the complexity term $C(\delta)$ to improve the ability of {\tnn} to generalize to various channels, by minimizing the generalization error in Section \ref{sec:generalization}. 
% \ref{sec:inverse_design}. 
% 
% By the use of gradient descent optimization method and the backpropagation algorithm [3], weights of the NN can be found which minimize the loss function over the training set.
where $\delta_n{=}\{\delta_{n,l}\}$, for $l{\in}[1,L]$.
To understand the internal mechanism of {\tnn} and compare its performance to {\tmap} over stochastic wireless channels, we define the concept of \textit{probabilistic equivalence} between {\tnn} and {\tmap} receiver. 
% Since the behaviour of the wireless channel is described by its probability distribution, we first define the notion of \textit{probabilistic equivalence} of  {\tnn} and {\tmap} receiver. 
% Since the optimal classical transceivers ({\tmap}) rely on Bayesian optimal techniques such as MAP, we are interested in achieving \textit{probabilistic equivalence} between NNs and such techniques, i.e., the equivalence of {\tnn} and {\tmap}. 
% Since the optimal classical transceivers ({\tmap}) rely on Bayesian optimal techniques such as MAP, we are interested in achieving \textit{probabilistic equivalence} between NNs and such techniques, i.e., the equivalence of {\tnn} and {\tmap}. 
% Two kernels are defined to be equivalent if they produce the same output distribution under the same input distribution. 
% This is defined below  
%
\begin{definition}
\label{def:equivalence}
(Equivalence of {\tnn} and {\tmap}). A {\tnn} receiver with associated function $\fnn$ and {\tmap} with associated function $\fmap$, are equivalent if and only if,
% (Equivalence of {\tnn} and {\tmap}). A {\tnn} receiver with associated function $\fnn{:} \mathbb{C}^{d} \rightarrow \mathbb{R}$ and {\tmap} with associated function $\fmap{:} \mathbb{C}^d \rightarrow \mathbb{R}$, are equivalent if,
%\vspace{-10pt}
%\useshortskip
\begin{align}
% \small
%\vspace{-5pt}
&\fnn(\boldsymbol{r};\delta_n)\stackrel{P}{\longrightarrow} \fmap(\boldsymbol{r}) \enskip \text{or,} \enskip\nonumber\\ &\lim_{n{\rightarrow}\infty}\mathrm{P}\left[|\fnn(\boldsymbol{r};\delta_n)-\fmap(\boldsymbol{r})|\right]{\rightarrow}0
\label{eq:equivalence}
\end{align}\normalsize
% $p(\fnn(\boldsymbol{r})|\boldsymbol{r})=p(\fmap(\boldsymbol{r})|\boldsymbol{r})$, 
% where $\boldsymbol{r}{\in}\mathbb{C}^{d}$ is a random vector and $d$ is its dimensionality, and 
where $\stackrel{P}{\longrightarrow}$ refers to convergence in probability \cite{ML_Probability_book_Murphy}.
%. %of $\boldsymbol{r}$. % , and $n=|\mathcal{D}|$ is the number of training samples.
\end{definition}
Therefore, a {\tnn} %with associated function $\fnn$ 
and {\tmap} receiver %with associated function $\fmap$, 
are defined as equivalent if their outputs converge in probability. %\cite{ML_Probability_book_Murphy}. %as in \eqref{eq:equivalence}. 
% 
\textit{Due to space constraint, the complete proofs of Theorems and Lemmas are provided in an anonymous external document in \cite{appendix_link}.}

\subsection{Impact of Training on Equivalence}

Establishing equivalence of the {\tnn} and {\tmap} receiver is not a straightforward task because the output of conventional neural networks are deterministic estimates and not Bayesian probabilities, and the difficulty lies in bridging the gap between empirical approaches (\eg data-driven {\tnn} receiver) and Bayesian approaches (\eg model-driven {\tmap} receiver). 
% The difficulty in establishing equivalence of the {\tnn} and {\tmap} receiver lies in bridging the gap between empirical or data-driven techniques and Bayesian or model-driven techniques \cite{ML_Probability_book_Murphy}. 
The disparity of these techniques are investigated under complete and incomplete training of the {\tnn} receiver.  

\subsubsection{Complete Training}
This represents the scenario where the {\tnn} receiver is trained on a sufficiently rich dataset that is representative of the entire channel distribution.
Due to the difficulty in establishing effective measures of the quality of training data that is robust to various channel models, complete training is guaranteed asymptotically as $n{\rightarrow}{\infty}$. 
Therefore, under complete training criteria \eqref{eq:NN_risk} is represented by \eqref{eq:complete},
% 
\vspace{-5pt}
% \abovedisplayshortskip=-5pt
\begin{align} \label{eq:complete}
% \small
    &\delta^{*}=\lim_{n{\rightarrow}\infty}\argmin_{\delta_n} [\mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n))] \ \text{where,} \\
    &{\lim_{n{\rightarrow}\infty}} \mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n))=\mathbb{E}[\mathcal{L}(\fnn(\boldsymbol{r}{;}\delta_n))] \nonumber
    % \label{eq:lln}\\
    % &\small \mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n)){=} \frac{1}{n}{\sum_n}\mathcal{L}(\fnn(\boldsymbol{r}{;}\delta_n)){=}\mathbb{E}[\mathcal{L}(\fnn(\boldsymbol{r}{;}\delta_n))]\label{eq:lln}\\
    % &\small \mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n)){=} \frac{1}{n}{\sum_n}\mathcal{L}(\fnn(\boldsymbol{r}{;}\delta_n)){=}\mathbb{E}[\mathcal{L}(\fnn(\boldsymbol{r}{;}\delta_n))]\label{eq:lln}\\
    % &\small \mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n)){\stackrel{P}{\rightarrow}}\mathcal{R}(\fnn(\boldsymbol{r})){\implies}
    % \fnn(\boldsymbol{r}{;}\delta_n){\stackrel{P}{\rightarrow}}\fnn(\boldsymbol{r})\label{eq:universal}
\end{align}
%
%Later we investigate metrics to determine the degree of completeness of the training data. 
% Under complete training 
\eqref{eq:complete} is supported by the law of large numbers, %\cite{ML_Probability_book_Murphy}, %whose validity does not require independence of data samples
where the average over the data in \eqref{eq:NN_risk} is replaced by the statistical expectation, $\mathbb{E}[.]$ over the underlying channel distribution.
Furthermore, from \eqref{eq:complete} due to the capacity of a feed-forward NN model to approximate any nonlinear function to a desired level of accuracy \cite{Cybenko1989ApproximationBS,ML_Probability_book_Murphy}, we can conclude \eqref{eq:universal},
\begin{align}% \label{eq:complete}
\small{\lim_{n{\rightarrow}\infty}}\mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n)){\stackrel{P}{\rightarrow}}\mathcal{R}(\fnn(\boldsymbol{r}))
{\implies}
    {\lim_{n{\rightarrow}\infty}}\fnn(\boldsymbol{r}{;}\delta_n){\stackrel{P}{\rightarrow}}\fnn(\boldsymbol{r})\label{eq:universal} 
\end{align}
% \begin{subequations}\label{eq:complete}
% \begin{align}% \label{eq:complete}
% % \small
%     &\delta^{*}=\lim_{n{\rightarrow}\infty}\argmin_{\delta_n} [\mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n))] \ \text{where,} \\
%     &\small \mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n)){=} \frac{1}{n}{\sum_n}\mathcal{L}(\fnn(\boldsymbol{r}{;}\delta_n)){=}\mathbb{E}[\mathcal{L}(\fnn(\boldsymbol{r}{;}\delta_n))]\label{eq:lln}\\
%     % &\small \mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n)){=} \frac{1}{n}{\sum_n}\mathcal{L}(\fnn(\boldsymbol{r}{;}\delta_n)){=}\mathbb{E}[\mathcal{L}(\fnn(\boldsymbol{r}{;}\delta_n))]\label{eq:lln}\\
%     &\small \mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n)){\stackrel{P}{\rightarrow}}\mathcal{R}(\fnn(\boldsymbol{r})){\implies}
%     \fnn(\boldsymbol{r}{;}\delta_n){\stackrel{P}{\rightarrow}}\fnn(\boldsymbol{r})\label{eq:universal}
% \end{align}
% \end{subequations}
% Two approximations hold to bridge the gap between data and model-driven approaches: a) \eqref{eq:lln} is supported by the law of large numbers \cite{ML_Probability_book_Murphy}, %whose validity does not require independence of data samples
% where the average over the data is replace by the statistical expectation, $\mathbb{E}[.]$ over the underlying channel distribution, and
% b) \eqref{eq:universal} is supported by the %Universal approximation theorem 
% capacity of a feed-forward NN model to approximate any nonlinear function to a desired level of accuracy \cite{Cybenko1989ApproximationBS}.  
% % Two approximations hold to bridge the gap between data and model-driven approaches: a) \eqref{eq:lln} is supported by the law of large numbers \cite{ML_Probability_book_Murphy}, %whose validity does not require independence of data samples
% % where the average over the data is replace by the statistical expectation, $\mathbb{E}[.]$ over the underlying channel distribution, and
% % b) \eqref{eq:universal} is supported by the %Universal approximation theorem 
% % capacity of a feed-forward NN model to approximate any nonlinear function to a desired level of accuracy \cite{Cybenko1989ApproximationBS}.  
Therefore to guarantee equivalence as in \eqref{eq:equivalence}, it suffices to show that $\fnn$ and $\fmap$ converge over the same input $\boldsymbol{r}$, i.e.,  $\fnn(\boldsymbol{r})\stackrel{P}{\longrightarrow}\fmap(\boldsymbol{r})$.
In practice, $n$ is finite, therefore complete training is approximately guaranteed by \textit{empirically} determining a value $n_{emp}$, such that if $n{\geqslant}n_{emp}$ the \textit{Structural Risk} of the {\tnn} receiver (defined in Section \ref{sec:ber_bounds}) is approximately zero, %or below a target threshold value 
as explained further in Section \ref{sec:results}. 

% Alternatively probabilistic equivalence is guaranteed by ensuring stronger condition: A unique global minimum exists for $\mathcal{R}_{NN}{:=}\mathcal{R}({f}_{NN})$ that is equal to that of $\mathcal{R}_{MAP}$.
    % , defined as Problem \ref{prob:model_driven}.
% This is also referred to as asymptotic equivalence or convergence in distribution \cite{ML_Probability_book_Murphy}. Alternatively probabilistic equivalence is guaranteed by ensuring stronger conditions: 
% \begin{itemize}
%     \item A unique global minimum exists for $\mathcal{R}_{NN}{:=}\mathcal{R}({f}_{NN})$ that is equal to that of $\mathcal{R}_{MAP}$.
%     % , defined as Problem \ref{prob:model_driven}.
%     \item Consistency (convergence in probability) which describes how close the optimal Bayesian error $\mathcal{R}_{MAP}$ can be approximately reached by $\mathcal{R}({f}_{NN})$. i.e., the excess error $\lim_{n{\rightarrow}\infty}[\mathcal{R}({f}_{NN})){-}\mathcal{R}_{MAP}] \rightarrow 0$, where $n$ is the number of data samples. 
%     % Later defined as Problem \ref{prob:data_driven}.
% \end{itemize}
%
% Therefore, a {\tnn} with associated function $\fnn$ and {\tmap} with associated function $\fmap$, are defined as equivalent if their outputs converge in probability as in 
% \eqref{eq:equivalence},
% %\vspace{-10pt}
% %\useshortskip
% \begin{align}
% \small
% %\vspace{-5pt}
% \lim_{n{\rightarrow}\infty}\mathrm{P}\left[|\fnn(\boldsymbol{r};\delta_n)-\fmap(\boldsymbol{r})|\right]{\rightarrow}0.
% \label{eq:equivalence}
% \end{align}\normalsize
%

% Consequently the {\tnn} receiver that achieves the minimum Bayesian risk is the optimal architecture for the NN-based transceiver as defined below,

% \begin{definition}
% \label{def:optimality}
% (Optimality of {\tnn}). A neural network that achieves the minimum Bayesian risk is the optimal NN architecture for {\tnn} as given by \eqref{eq:risk_NN},
% \begin{align}
% \label{eq:risk_NN}
% \mathcal{R}_{NN}^{*}&=\inf _{f} \mathcal{R}_{NN}(f) \quad \text{where,} \quad \\
% \mathcal{R}_{NN}(f)&=\mathbb{E} [\mathcal{L}(\fnn(\boldsymbol{r}), \bar{\boldsymbol{s}})] \nonumber
% % \mathcal{R}_{NN}(f)&=\mathbb{E}_{\boldsymbol{r}, \bar{\boldsymbol{s}}} [\mathcal{L}(\fnn(\boldsymbol{r}), \bar{\boldsymbol{s}})] \nonumber
% % \mathcal{R}_{\phi}^{*}=\inf _{f} \mathcal{R}_{\phi}(f) \quad \text{where,} \quad 
% % \mathcal{R}_{\phi}(f)=\mathbb{E}_\phi(Y f(X))
% \end{align}
% where $\bar{\boldsymbol{s}}$ is the desired output of {\tnn}. 
% \end{definition}

% In other words \eqref{eq:risk_NN} means that there exists a NN with a mapping function $f^{*}_{NN}{\in}\{\fnn\}$ for which the Bayesian risk is minimum. 
% % 
% Definitions \ref{def:equivalence} and \ref{def:optimality} can be used to derive the relationship between {\tnn} and {\tmap} in terms of the Bayesian risk as given by the claim below. 

% \begin{claim}
% For known and stationary channel distributions, {\tnn} cannot outperform {\tmap} in terms of the Bayesian risk, i.e.,
% \begin{align}
%     \mathcal{R}_{MAP}\leqslant \mathcal{R}_{NN}^{*}\leqslant \mathcal{R}_{NN}
%     %\mathcal{R}_{NN}^{*}\geqslant \mathcal{R}^{*}
%     \label{eq:risk_NN_ML}
% \end{align}
% \label{claim:risk_NN_ML}
% \end{claim}

% \begin{proof}
% From the definition of $\mathcal{R}_{NN}^{*}$ in \eqref{eq:risk_NN} and $f^{*}_{NN}{\in}\{\fnn\}$ we have $\mathcal{R}_{NN}^{*}{\leqslant} \mathcal{R}_{NN}$. Moreover, {\tmap} is the system which achieves the minimum Bayesian risk given by  $\mathcal{R}_{MAP}=\inf_{f} \mathcal{R}(f)$, where the infimum is over all measurable functions $f{\in}\mathbb{R}$ in the subset $\{f\}$. Since it is clear that $\{f^{*}_{NN}\}{\in}\{f\}{\subset}\mathbb{R}$ we also obtain $\mathcal{R}_{MAP}{\leqslant} \mathcal{R}_{NN}^{*}$. This proves Claim \ref{claim:risk_NN_ML}. 
% % $\mathcal{R}_{NN}^{*}$ in \eqref{eq:risk_NN} is defined over the subset $\{\fnn\}$ and the optimum Bayes risk $R^{*}=\inf_{f} R(f),$ where the infimum is over all measurable functions $f{\in}\mathbb{R}$ in the subset $\{f\}$. Since it is clear that $\{\fnn\}{\subset}\{f\}{\subset}\mathbb{R}$ we obtain \eqref{eq:risk_NN_ML}. 
% \end{proof}

% \begin{remark}
% From Claim \ref{claim:risk_NN_ML} for known and stationary channel distributions the optimal design for {\tnn} is equivalent to {\tmap}, in terms of the Bayesian risk.
% \end{remark}
% Thus, our goal is to design NN that achieve equivalence with optimal classical transceivers. 
% This is achieved by: first, designing the loss function of {\tnn} to achieve equivalence with {\tmap} in terms of the Bayes risk, 
% determining the bounds on the BER under complete and incomplete training, 
% and finally use this equivalence for the inverse design of the NN architecture.

% \note{
% \subsection{Impact of Amount of Training}

% Establishing equivalence of the {\tnn} and {\tmap} receiver is not a straightforward task because the output of conventional neural networks are deterministic estimates and not Bayesian probabilities, and the difficulty lies in bridging the gap between empirical approaches (\eg data-driven {\tnn} receiver) and Bayesian approaches (\eg model-driven {\tmap} receiver). 
% % The difficulty in establishing equivalence of the {\tnn} and {\tmap} receiver lies in bridging the gap between empirical or data-driven techniques and Bayesian or model-driven techniques \cite{ML_Probability_book_Murphy}. 
% The disparity of these techniques are studied under complete and incomplete training of the {\tnn} receiver.  

% \subsubsection{Complete Training}
% This represents the scenario where the {\tnn} receiver is trained on a sufficiently rich dataset that is representative of the entire channel distribution.
% Due to the difficulty in establishing effective measures of the quality of training data that is robust to various channel models, complete training is guaranteed asymptotically as $n{\rightarrow}{\infty}$. 
% Therefore, the complete training criteria for \eqref{eq:NN_risk} is represented by \eqref{eq:complete},
% \begin{subequations}\label{eq:complete}
% \begin{align}% \label{eq:complete}
% % \small
%     &\delta^{*}=\lim_{n{\rightarrow}\infty}\argmin_{\delta_n} [\mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n))] \ \text{where,} \\
%     &\mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n)){=} \frac{1}{n}{\sum_n}[\mathcal{L}(\fnn(\boldsymbol{r}{;}\delta_n))]{=}\mathbb{E}[\mathcal{L}(\fnn(\boldsymbol{r}{;}\delta_n))]\label{eq:lln}\\
%     &\mathcal{R}(\fnn(\boldsymbol{r}{;}\delta_n))\stackrel{P}{\rightarrow}\mathcal{R}(\fnn(\boldsymbol{r})){\implies}
%     \fnn(\boldsymbol{r}{;}\delta_n)\stackrel{P}{\rightarrow}\fnn(\boldsymbol{r})\label{eq:universal}
% \end{align}
% \end{subequations}
% %
% %Later we investigate metrics to determine the degree of completeness of the training data. 
% Under complete training two simultaneous approximations hold to accommodate a data-driven setup: a) \eqref{eq:lln} is supported by the Law of Large Numbers \cite{ML_Probability_book_Murphy}, %whose validity does not require independence of data samples
% where the average over the data is replace by the statistical expectation, $\mathbb{E}[.]$ over the underlying channel distribution, and
% b) \eqref{eq:universal} is supported by the %Universal approximation theorem 
% fact that a feed-forward NN model can approximate any nonlinear function to a desired level of accuracy \cite{Cybenko1989ApproximationBS}.  
% Therefore to guarantee equivalence as in \eqref{eq:equivalence}, it suffices to show that $\fnn$ and $\fmap$ converge over the same input $\boldsymbol{r}$, i.e.,  $\fnn(\boldsymbol{r})\stackrel{P}{\longrightarrow}\fmap(\boldsymbol{r})$.
% In practice, $n$ is finite, therefore complete training is approximately guaranteed by \textit{empirically} determining a value $n_{th}$, such that if $n{\geqslant}n_{th}$ the loss of the {\tnn} receiver is approximately zero %or below a target threshold value 
% as explained further in Section \ref{sec:results}.  
% : this approximation is supported by the Law of Large Numbers whose validity does not require independence of data samples, and 
% b) replacing the general function $f(\boldsymbol{r})$ with the output $f(\boldsymbol{r},\delta^*)$ of a neural network with $\delta^*$ summarizing the parameters of {\tnn}: this approximation is supported by the Universal approximation theorem which states that a neural network can closely approximate any nonlinear function provided \cite{Cybenko1989ApproximationBS}. 
% Under these approximations, the optimization problem in \eqref{eq:NN_risk} is transformed into a classical optimization over the parameters $\delta^*$. 
% Under these conditions $\mathcal{R}(f(\boldsymbol{r},\delta^*)){\rightarrow}\mathcal{R}(f(\boldsymbol{r}))$ when $n{\rightarrow}\infty$, where $\mathcal{R}(f(\boldsymbol{r},\delta^*)){=} \frac{1}{n}\sum[\mathcal{L}(f(\boldsymbol{r},\delta^*))]{=}\mathbb{E}[\mathcal{L}(f(\boldsymbol{r},\delta))]$.
% Therefore, complete training in \eqref{eq:NN_risk} is represented by \eqref{eq:complete},
% \begin{align}
%     \delta^{*}&=\lim_{n{\rightarrow}\infty}\argmin_{\delta_n} \{\mathcal{R}(\fnn(\boldsymbol{r};\delta_n),\bar{\boldsymbol{s}})\}
%     \label{eq:complete}
% \end{align}
\subsubsection{Incomplete Training}
This represents the scenario, where the {\tnn} is trained on a finite dataset that is not representative of the entire channel distribution.
% For a given dataset $\mathcal{D}$, $n{=}|\mathcal{D}|$, where $|.|$ represents the cardinality of a set. 
% \note{
Under incomplete training, where $n$ is finite (in practice, $n{<}n_{emp}$), it is difficult to bridge the gap between Empirical and Bayesian approaches \cite{ML_Probability_book_Murphy}. Therefore, we derive the expected risk of the {\tnn} receiver, and use this to quantify the disparity between {\tnn} and {\tmap}.
% Therefore, incomplete training is given by \eqref{eq:incomplete},
% \begin{align}
%     \delta^{*}&=\argmin_{\delta_n} \{\mathcal{R}(\fnn(\boldsymbol{r};\delta_n),\bar{\boldsymbol{s}})\}
%     \label{eq:incomplete}
% \end{align}

% The typical NN loss function is designed to minimize a regularized risk to fit the NN model (parameters $\delta$) for a given complexity penalty $C(\delta)$, by using
% \begin{align*}
% \hat{\delta}_{\lambda}=\underset{\delta}{\operatorname{argmin}}\left[R_{emp}(\mathcal{D}, \delta)+\lambda C(\delta)\right]    
% \end{align*}
% where $R_{emp}(\mathcal{D}, \delta)$ measures the error estimation error, $C(\delta)$ measures the complexity of the prediction function $\delta(\boldsymbol{r})$ and $\lambda$ controls the strength of the complexity penalty. 
% We initially focus on designing the first term to achieve equivalence of {\tnn} and {\tmap}.
% Then we design focus on the design of the latter term to improve the generalization capability by minimizing the generalization error. 
% The structural risk minimization principle \cite{ML_Probability_book_Murphy} is often used to determine $\lambda$ as $\hat{\lambda}=\underset{\lambda}{\operatorname{argmin}} \hat{R}\left(\hat{\delta}_{\lambda}\right)$ where $\hat{R}(\delta)$ is an estimate of the risk. We use theoretical upper bounds on the risk to determine $\lambda$ in the generalization bounds section. 
% The structural risk minimization principle \cite{ML_Probability_book_Murphy} is often used to determine $\lambda$ as $\hat{\lambda}=\underset{\lambda}{\operatorname{argmin}} \hat{R}\left(\hat{\delta}_{\lambda}\right)$ where $\hat{R}(\delta)$ is an estimate of the risk. We use theoretical upper bounds on the risk to determine $\lambda$ in the generalization bounds section. 

% Therefore, in order to design {\tnn} receivers that achieve equivalence with {\tmap} transceivers, we first derive the loss function of {\tnn} that guarantees equivalence, and use this in determining the tight lower and upper bounds on the BER under complete and incomplete training. 
% }
\end{comment}






















%---------------------------------------OLD MODEL--------------------------------------------%
\begin{comment}

%\newpage
\section{Models and Preliminaries}
\label{sec:system}
% \begin{figure}
%         \begin{subfigure}[b]{0.21\textwidth}
%                 \includegraphics[width=\textwidth]{anomaly1.pdf}
%                 \caption{Anomaly Detection.}
%                 \label{fig:anomaly}
%         \end{subfigure}s
%         %\quad
%         \begin{subfigure}[b]{0.24\textwidth}
%                 \includegraphics[width=\textwidth]{blockchain.pdf}
%                 \caption{Block creation by validators.}
%                 \label{fig:blockchain}
%         \end{subfigure}
% 	\caption{The functions of the validators in {\abbrev}. }
% 	\label{fig:sys}
% 	\vspace{-5pt}
% \end{figure}
% \begin{comment}
% \begin{figure}
%         \centering
%         \begin{subfigure}[b]{0.23\textwidth}
% 		\includegraphics[width=\textwidth]{figures/Pf_SNR.pdf}
%                 \caption{Effect of degree of falsification in SNR.}
%                 \label{fig:arch}
%         \end{subfigure}% 
%         \quad 
%         \begin{subfigure}[b]{0.23\textwidth}
%                 \includegraphics[width=\textwidth]{figures/Pf_Loc.pdf}
%                 \caption{Effect of degree of falsification in Location.}
%                 \label{fig:func}
%         \end{subfigure}
% 	\caption{\note{Put correct caption}}
% 	\label{fig:netarch}
% 	\vspace{-5pt}
% \end{figure}
% \end{comment}
% \begin{comment}
% We propose a system that detects anomalies in the sensing reports from sensors and assigns reputation to sensors in a distributed manner, towards achieving trustworthy (more reliable) inference (data fusion).
% Central to the idea of reputation based sensing systems, is the ability to maintain information about a sensors' behaviour and assess the reputation in a purely distributed manner among trustless entities. Distributed Ledger Technologies (DLT) like Blockchain provide immutability and distributed consensus for transactions among participating entities, which enables the dissemination and aggregation of data and  among untrustworthy entities. Hence, a blockchain is used to record the activities of sensors (transactions) and assess their reputation towards achieving more reliable inference.
% \end{comment}

\noindent \textbf{System Model: }
Let $\mathbf{s}=\{s_m\}$ denote the modulated signal vector of order $M$ and $s(t)$ be the transmitted signal in the time domain. Let $\textbf{r}$ and $\textbf{r}(t)$ be the received signal vector and time domain signal. Let $h(t)$ denote the response of the channel.\\

\noindent \textbf{Deep Learning Basics and Notations: }
A feedforward NN with $L$ layers describes a mapping $f\left(\mathbf{x}_{0} ; \boldsymbol{\theta}\right): \mathbb{R}^{N_{0}} \mapsto \mathbb{R}^{N_{L}}$ of an input vector $\mathbf{x}_{0} \in \mathbb{R}^{N_{0}}$ to an output vector $y=\mathbf{x}_{L} \in \mathbb{R}^{N_{L}}$ through $L$ iterative processing steps: $\mathbf{x}_{\ell}=f_{\ell}\left(\mathbf{x}_{\ell-1} ; \theta_{\ell}\right), \quad \ell=1, \ldots, L$. Here $f_{\ell}\left(\mathbf{x}_{\ell-1} ; \theta_{\ell}\right): \mathbb{R}^{N_{\ell-1}} \mapsto \mathbb{R}^{N_{\ell}}$ is the mapping carried out by the $\ell$ th layer. This mapping depends on the output vector $\mathbf{x}_{\ell-1}$ from the previous layer and a set of parameters $\theta_{\ell}$. The $\ell$ th layer is referred to as dense or fully-connected if $f_{\ell}\left(\mathbf{x}_{\ell-1} ; \theta_{\ell}\right)$ takes the form
\begin{align}
f_{\ell}\left(\mathbf{x}_{\ell-1} ; \theta_{\ell}\right)=\sigma\left(\mathbf{W}_{\ell} \mathbf{x}_{\ell-1}+\mathbf{b}_{\ell}\right)    
\end{align}
where $\mathbf{W}_{\ell} \in \mathbb{R}^{N_{\ell} \times N_{\ell-1}}$ are the weights, $\mathbf{b}_{\ell} \in \mathbb{R}^{N_{\ell}}$ are the biases, and $\sigma(\cdot)$ is an activation function. The set of parameters for this layer is $\theta_{\ell}=\left\{\mathbf{W}_{\ell}, \mathbf{b}_{\ell}\right\}$. 
NNs are generally trained using labeled training data, i.e., a set of input-output vector pairs $\left(\mathbf{x}_{0, i}, \mathbf{x}_{L, i}^{*}\right), i=1, \ldots, S,$ where $y_i=\mathbf{x}_{L, i}^{*}$ is the desired output of the neural network when $\mathbf{x}_{0, i}$ is used as input. The goal of the training process is to minimize the loss
\begin{align}
L(\boldsymbol{\theta})=\frac{1}{S} \sum_{i=1}^{S} l\left(y_i, \mathbf{x}_{L, i}\right)
\end{align}
with respect to the parameters in $\theta$, where $l(\mathbf{u}, \mathbf{v}): \mathbb{R}^{N_{L}} \times \mathbb{R}^{N_{L}} \mapsto \mathbb{R}$ is the loss function and $\mathbf{x}_{L, i}$ is the output of the NN when $\mathbf{x}_{0, i}$ is used as input.


% Moreover, the mapping can be stochastic,
% i.e., $f_{\ell}$ can be a function of some random variables. We use $\boldsymbol{\theta}=\left\{\theta_{1}, \ldots, \theta_{L}\right\}$ to denote the set of all parameters of the network. The $\ell$ th layer is called dense or fully-connected if $f_{\ell}\left(\mathbf{r}_{\ell-1} ; \theta_{\ell}\right)$ has the form
% \[
% f_{\ell}\left(\mathbf{r}_{\ell-1} ; \theta_{\ell}\right)=\sigma\left(\mathbf{W}_{\ell} \mathbf{r}_{\ell-1}+\mathbf{b}_{\ell}\right)
% \]

\noindent \textbf{Classical Transceiver: }


\noindent \textbf{NN-based Transceiver: }\\

% \noindent
% \textbf{Threat Model:} \underline{\textit{1) Malicious Sensors (Sensing threat):}}
% The sensors may falsify either their reported SNR, their reported location or both. 
% %\noindent
% \underline{\textit{2) Malicious Validators (Validation threat):}}
% The validators may forge information in the block they create by falsifying the confidence scores. 
% Since, the validators may assume the role of a sensor, whose reputation depends on the reputation-weighted fusion of reports from other sensors, the validators are intrinsically discouraged from falsifying. 
% % i.e., the validators have a stake in the system. 
% %\note{There is no section on threat analysis or incentives in the paper. I think that is important. It could be here as well as a preliminary or model since we don't analyze or evaluate on those two.}

% %\vspace{30pt}
% \noindent \textbf{Protocol:} %\note{May refer to fig \ref{fig:proto} above}
% There are three key phases of activity in {\abbrev} that each of the entity in the system adheres to: 1) Sensing Phase: the sensors sense the target and report their findings to the validators in the vicinity, 2) Validation Phase: the validators assess the truthfulness of the reports and creates a block by aggregating the reports, and 3) Blockchain Phase: the validators broadcast mined blocks to arrive at consensuses on the Blockchain before calculating the reputation of sensors. 

% In the sensing phase, each sensor $s_i\in \mathcal{S}$ %with an identity $id^i$ 
% senses the target $\mathcal{T}$, and creates a report with its perceived signal-to-noise ratio (SNR), $SNR^i$ and an estimate of its location, $Loc^i$ and broadcasts the report, $[SNR, Loc]^i$ to all the validators.
% Additionally, the sensors may report other sensing parameters depending on the application of interest. 
% %E.g., probability of detection and probability of false alarms in the sensing of spectrum infractions.
% However, for applications in wireless communications, the SNR and the location are identified as fundamental sensing parameters that all sensors must report. A sketch of the protocol steps is shown in figure \ref{fig:proto}. It is to be noted that there is not explicit synchrony in the network and all nodes will converge at the same Blockchain state eventually by employing the \textit{most-difficult-chain} rule described in subsequent sections.

\end{comment}

==> questions.tex <==
\section{Questions}

\textbf{Question 1:} Any LTV channel can be built by the atomic channel $\mathbf{G}$ at equation (10) (all equations cited are in paper "On non-WSSUS wireless fading channels")
\begin{equation}
    \mathbf{H} = \iiiint \mathcal{H}^{(\mathbf{G})}(t,f; \tau,\nu) \mathbf{G}_{t,f}^{\tau, \nu} ~dt ~df ~d\tau ~d\nu
\end{equation}
which has the similar form with 
\begin{equation}
    \mathbf{H} = \iint S_{\mathbf{H}}(\tau, \nu) \mathbf{S}_{\tau, \nu} ~d\tau ~d\nu
\end{equation}
where $\mathbf{S}_{\tau, \nu}$ is TF-shif operator, which can be deduced from equation (1).

For a non-WSSUS channel $\mathcal{H}$,

\noindent
1) what's the physical means of $\mathcal{H}^{(\mathbf{G})}$ and can it be observed?

\noindent
2) can $\mathbf{G}_{t,f}^{\tau, \nu}$ be seen as a time-frequency delay-Doppler 4-D shift operator and $\mathcal{H}^{\mathbf{G}}$ as 4-D response? 

\vspace{20pt}

\textbf{Question 2:}
In equation (6), there is a statistics I/O relation for LSF.
\begin{equation}
\bar{W}_{r}(t, f)=\iint \widetilde{\mathcal{C}}_{\mathbf{H}}\left(t, f ; t^{\prime}, f^{\prime}\right) \bar{W}_{s}\left(t^{\prime}, f^{\prime}\right) \mathrm{d} t^{\prime} \mathrm{d} f^{\prime}
\end{equation}

LSF is the second order statistics of $\mathcal{H}^{\mathbf{G}}$. Input and output are also second order statistics of input and output signals, respectively.

\noindent
 1) Is there a similar I/O relation for  $\mathcal{H}^{(\mathbf{G})}$? For example:

\begin{equation}
    r(t,f) = \mathbf{H}s(t,f) = \iint \mathcal{H}^{(\mathbf{G})}(t,f; \tau,\nu) s(\tau, \nu) ~d\tau ~d\nu
\end{equation}
where $s(t,f)$ and $r(t,f)$ are time-frequency domain symbols. 



\textbf{Question 3:}

\noindent
1) Can $\mathcal{H}^{(\mathbf{G})}$ be visualized like Fig. 6 in paper "On non-WSSUS wireless fading channels" or Fig 1.6 in book "Wireless communications over rapidly time-varying channels"?  

\noindent
2) If it is possible, could you share the toy codes of Fig 1.2, 1.3, 1.4, 1.5 and 1.6 in the book?

Thanks a lot!

==> related.tex <==
% \newpage
\section{Related Work}
\label{sec:related}

% The related 

\noindent
\textbf{Neural Network based Transceivers:}
% Deep Learning has emerged as a versatile tool for physical layer communication due to its proficiency in systems with model and algorithm deficit \cite{simeone2018very}, and has been used to replace individual blocks in communication systems for optimized performance for a given dataset. 
Despite the increasing interest of DL to replace classical communication systems, these systems have come at the cost of increased training time and model complexity and have at best approached the error rate of classical methods \cite{kim2018communication,gruber2017deep}. 
% The stringent requirements on reliability and achievable throughput in xG propagation environments demand wireless communication systems that achieve provable performance guarantees over a variety of channels. 
So far, much of the effort has been focused on replacing individual blocks \cite{tan2018improving,klautau2018detection} or the end-to-end chain~\cite{DeepSig2,aoudia2018endtoend} in classical transceivers using ``black-box" neural networks to achieve a target error rate for a specific dataset.
These fixed function implementations that fits a particular dataset cannot be generalized to other scenarios.
This has limited the wide-spread practical adoption of neural network based communication systems, due to their lack of explainability \cite{guo2020explainable6G} and performance guarantees on the error rate or the complexity (training or hardware complexity). 
% Fueled by the promising results shown in other domains, wireless researchers have adopted a learning based approach in order to tame the stochasticity of the wireless channel. 
In order to make wireless communications explainable, we take the first step towards understanding what happens inside a NN-based receiver that eventually performs equivalent to a classical receiver. 
We use this knowledge to derive tight bounds on the BER of NN-based receivers that achieve strict communication guarantees essential for practical adaptation. 
% Moreover, we de


\noindent
\textbf{Explainable Neural Networks:}
% The very first results have demonstrated the universal approximation of DNNs, that is, any continuous function defined on a compact set can be approximated at any precision using a DNN [20], [21]. Recently, some effort has been made to analyze how the structural properties of DNNs, mainly depth and width, contribute to their powerful capability of modeling functions, i.e., expressive power of DNNs [22]–[24]. These works converge to a similar conclusion that the expressive power of a DNN grows exponentially with its depth, which is compelling and provides some meaningful theoretical insights into superior performance of DNNs in practice. However, previous research seldom involves with the theoretical interpretation on the performance of DL embedded communication systems.
% A majority of DL approaches rely on a black-box approach to replace classical transceivers with neural networks and achieve comparable performance, while lacking guarantees or the robustness to generalize beyond the trained data.
% We outline the literature that have attempted to move away from this black-box data-driven approach by primarily relying on model-driven techniques.
% The end-to-end autoencoder-based system has been extended to multi-user communication over interference channels, OFDM systems with multipath channels in \cite{felix2018ofdmautoencoder}. In \cite{ye2018channel}, the purely data-driven DL method has been used in transceiver optimization without using accurate CSI. 
The explainability of neural network based transceivers is very rare in the literature, attributed primarily due to their black-box implementation. 
Of particular relevance here, is the literature that instead rely on model-driven techniques to avoid the black box approach, and incorporate expert knowledge into autoencoder-based communication systems with the radio transformer network~\cite{o'shea2016radio} and the OFDM-autoencoder~\cite{felix2018ofdmautoencoder}. 
\cite{felix2018ofdmautoencoder} combines an autoencoder with a classical OFDM system to inherit its advantages, including robustness to synchronization errors and multipath equalization.
The model-driven OFDM receiver in~\cite{gao2018comnet} combines DL with expert knowledge and implements two subnets for channel estimation and symbol detection modular structure similar to classical systems. 
% involves two subnets for channel estimation and symbol detection which are combined in a block-by-block manner similar to classical systems. 
% Model-driven DL shows a competitive performance with data-driven approaches but with a lower number of trainable variables than the black box architecture. 
However these approaches are limited by the flexibility and accuracy of the underlying model and the trained weights, which limits their applicability to specific channel conditions. 
% This limits the generality of these approaches to a wide variety of channel conditions and limit their ability to adapt online to changes in channel conditions. 
% \cite{qiang2020deep} present initial interpretation of neural networks for channel estimation tasks, that approaches the performance of classical channel estimators.  
In contrast, we achieve guarantees on the performance of data-driven NN-based receivers by explaining their internal mechanisms and deriving their structure that achieves equivalence to MAP receiver.
This allows for low-complexity NN-based receivers that are robust to various channels.  
% \note{To be included: 
% 1/2-1 column.}





% \newpage

==> related_NLP.tex <==
\section{Related work}
\label{App:related_NLP}

% \inred{Maqsood: Trim only to material relevant to this work.}

We categorize the related work into three categories:

\noindent
\textbf{Characterization of Non-Stationary Channels:}
% \note{Zhibin: Include relevant references...}
% Although many literature attempt to characterize the channel they are often impractical as they rely on several statistics, by we do something different... Add citations and more context.
Wireless channel characterization in the literature typically require several local and global (in space-time dimensions) higher order statistics to characterize or model non-stationary channels, due to their time-varying statistics. 
These statistics cannot completely characterize the non-stationary channel, however are useful in reporting certain properties that are required for the application of interest such as channel modeling, assessing the degree of stationarity etc.
Contrarily, we leverage the 2-dimensional eigenfunctions that are decomposed from the most generic representation of any wireless channel as a spatio-temporal channel kernel.
These spatio-temporal eigenfunctions can be used to extract any higher order statistics of the channel as demonstrated in Section \rom{3}, and hence serves as a complete characterization of the channel.
Furthermore, since this characterization can also generalize to stationary channels, it is a unified characterization for any wireless channel.
Beyond characterizing the channel, these eigenfunctions are the core of the precoding algorithm.
% Therefore, this serves as a complete characterization of any non-stationary 
% Decomposition is essential for precoding but also allows us to completely characterize the wireless channel by explaining its statistics, without having to calculate all the statistics as in the literature. 
% Additionally, the decomposition that is most useful to ensure interference-free communication is one that preserves orthogonality ... Why is 4-D to 2-D decomposition important?

\noindent
\textbf{Precoding Non-Stationary Channels:}
Although precoding non-stationary channels is unprecedented in the literature \cite{AliNS0219}, we list the most related literature for completeness. 
The challenge in precoding non-stationary channels is the lack of accurate models of the channel and the (occasional) CSI feedback does not fully characterize the non-stationarities in its statistics. This leads to suboptimal performance using state-of-the-art precoding techniques like Dirty Paper Coding which assume that complete and accurate knowledge of the channel is available, while the CSI is often outdated in non-stationary channels. 
While recent literature present  attempt to deal with imperfect CSI by modeling the error in the CSI \cite{HatakawaNLP2012, HasegawaTHP2018, GuoTHP2020, DietrichTHP2007, CastanheiraPGS2013, WangTHP2012, MazroueiTDVP2016, Jacobsson1DAC2017}, they are limited by the assumption the channel or error statistics are stationary or WSSUS at best.
Another class of literature, attempt to deal with the impact of outdated CSI~\cite{AndersonLP2008,Zeng2012LP} in time-varying channels by quantifying this loss or relying statistical CSI. These methods are not directly suitable for non-stationary channels, as the time dependence of the statistics may render the CSI (or its statistics) stale, consequently resulting in precoding error. 
% The key to such precoding is extracting accurate eigenfunctions of the channel, however it is often impractical due to the high computational complexity and the availability of limited CSI at the transmitter \cite{}, especially when the channel is NS. 
% The paper \cite{} showed eigenfunctions are optimal to cancel interference but impractical. 

% Second is the completeness of CSI. DPC can achieve the optimal weighted sum rate because each user's signal can be coded by treating precoded users' signals as noncausally known interference to completely cancel out interference, where the perfect CSI is needed. Imperfect CSI will significantly affect the performance of  NLP. However, though nonlinear precoding will degradation with imperfect CSI,~\cite{HatakawaNLP2012, HasegawaTHP2018, GuoTHP2020, DietrichTHP2007, CastanheiraPGS2013, WangTHP2012, MazroueiTDVP2016, Jacobsson1DAC2017} shows nonlinear precoding can still achieve better performance than linear precoding with certain imperfect CSI. In NS channel, the perfect CSI is not achievable. This work will work with the statistics CSI (S-CSI), whose change should be relative to channel non-stationarity. In this manner, we can investigate the performance gap with respect to channel non-stationarity (which will degrade to stationary channel with zero non-stationarity). 


% Both linear and nonlinear precoding suffer from throughput loss with the outdated CSI.~\cite{AndersonLP2008} quantified this loss and proposed a linear precoder based on channel distribution information in time-varying downlink MIMO system. The method is robust to temporal variations so as to reduce the CSI feedback frequency.~\cite{LuLP2019} proposed robust linear precoders in massive MIMO downlink system with imperfect CSI. The available imperfect CSI for each UE obtained at the BS is modeled as statistical CSI under a jointly correlated channel model with both channel mean and channel variance information. The expected weighted sum-rate is very complicated and thus very difficult to be optimized directly. Minorize–maximize(MM) algorithm is used to find a stationary point of the optimization problem.~\cite{Zeng2012LP} investigated the linear precoding in MIMO fading channel with statistics CSI, such as the spatial correlation of channel, known at transmitted and perfect CSI known at receiver. The lower bound and upper bound of the mutual information with finite-alphabet inputs are derived. Then the optimal design for the left singular vector, power allocation vector and right singular vector are alternatively derived by maximizing the lower bound. The precoder combining three optimized vectors achieves near global optimal performance.

\noindent
\textbf{Space-Temporal Precoding:}
While, precoding has garnered significant research, spatio-temporal interference is typically treated as two separate problems, where spatial precoding at the transmitter aims to cancel inter-user and inter-antenna interference, while equalization at the receiver mitigates inter-carrier and inter-symbol interference.
% \ingreen{Alternately, \cite{hadani2018OTFS} proposes an orthogonal time frequency OTFS modulation scheme that make symbols experience minimal cross-interference by signal processing at the transmitter and receiver. However, equalizer is still needed to cancel 2-D intersymbol interference especially for non-staitonary channels.}
Alternately, \cite{hadani2018OTFS} proposes to modulate the symbols such that it reduces the cross-symbol interference in the delay-Doppler domain, but requires equalization at the receiver to completely cancel such interference in practical systems. %by introducing additional signal processing at the transmitter and receiver. 
Moreover, this approach cannot completely minimize the joint spatio-temporal interference that occurs in non-stationary channels since their statistics depend on the time-frequency domain in addition to the delay-Dopper domain (explained in Section \rom{2}).
% , and it requires equalization at the receiver to completely cancel the cross-symbol interference in the delay-Doppler domain for practical systems \cite{hadani2018OTFS}.
While spatio-temporal block coding techniques are studied in the literature \cite{Cho2010MIMObook} they add redundancy and hence incur a communication overhead to mitigate interference, which we avoid by precoding. 
These techniques are capable of independently canceling the interference in each domain, however are incapable of mitigating interference that occurs in the joint spatio-temporal domain in non-stationary channels. 
We design a joint spatio-temporal precoding that leverages the extracted 2-D eigenfunctions from non-stationary channels to mitigate interference that occurs on the joint space-time dimensions, which to the best of our knowledge is unprecedented in the literature. 

% Therefore, joint spatio precoding is unprecedented in the literature.




% Precoding at the transmitter is advantageous due to the ability to achieve higher capacity and lower BER compared to equalization at the receiver, which typically suffers from noise enhancement \cite{vu2006exploiting,Cho2010MIMObook}. 
% Further, it significantly reduces the computational burden on the user equipment. 
% % SVD-based precoding schemes are popular due to reduced complexity 
% % Further, precoding algorithms preferably shou
% While, precoding has attracted significant research, space-time-frequency interference is typically treated as two separate problems, where spatial precoding at the transmitter aims to cancel inter-user and inter-antenna interference, while equalization at the receiver mitigates ICI and ISI.
% Alternately, \cite{} proposes an orthogonal time frequency OTFS modulation scheme that aims at mitigating ISI and ICI. 
% While space-time-frequency block coding techniques are studied in the literature \cite{} they add redundancy and hence incur a communication overhead to mitigate space-time-frequency interference, which we avoid by precoding. 
% Therefore, joint space-time-frequency precoding is unprecedented in the literature.

% Linear precoding is the sub-optimal technique for weighted sum capacity with low complexity~\cite{LeeDPC2007}, which treats all transmitted signals as interference, except for the desired one. 
% Nonlinear precoding is motivated by Dirty Paper Coding (DPC)~\cite{CostaDPC1983}, which codes the data by known channel interference. The coded transmitted signals of previous antennas are needed through feedback. It is approved to achieve capacity region of downlink MIMO channel~\cite{WeingartenDPC2006}.
% To conclude, learning based precoding has significant advantages for solving non-convex optimization and high complexity problem. However, instead of focusing on specific model training, though it may achieve good performance in specific MIMO system, we have more interests on a general and explainable learning based method. 

% \noindent
% \textbf{Complexity:}
% Recently, quantized precoding techniques are proposed for massive MU MIMO~\cite{Jacobsson1DAC2017}, which aims to reduce the hardware complexity and circuit power consumption. It shows that low-resolution DACs can be applied at BS without a significant loss in terms of rates and BER. It also compared the linear-quantized precoding (ZF, WF, WFQ and MRT) and nonlinear-quantized precoding (SDR1, SDRr, SQUID and SP), showing that linear-quantized precoding can achieve sufficient performance for 3 to 4 bits DACs, but is much worse than nonlinear precoding for 1-bit DACs.~\cite{Jacobsson1DAC2018} is the latter work of ~\cite{Jacobsson1DAC2017}, which investigated the SQUID-OFDM technique. It is capable of supporting oversampling DACs and OFDM, and outperforms than linear-quantized precoding, but increases complexity and needs perfect CSI.~\cite{Chu1DAC2019} proposed another 1-bit DACs nonlinear precoding. It supports the MU-MIMO system with higher-modulation modes and can achieve comparable BER performance with SDR while being much faster.


% It is well known that NLP usually achieves better performance than LP but suffers from high complexity. DPC is impractical due to the prohibitive complexity. As the practical implementation of DPC, THP can achieve sub-optimal performance due to energy loss in modulo, which outperforms LP but still has much higher complexity. 
% Some modified NLP techniques proposed to reduce the complexity and meanwhile achieve comparative performance such as THP like precoding~\cite{HasegawaTHP2018}, D2VP precoding~\cite{MaD2VP2016} and quantized 1-DAC precoding~\cite{Chu1DAC2019}, where the latter two methods require perfect CSI.
% Recently, deep learning attracts a lot of interests in communication system and shows the excellence in solving non-convex problems and reducing complexity~\cite{Goodfellow2016DL}. It can help to implement expensive techniques like Karhunen-Loeve transform (KLT), which is considered optimal but very undesirable~\cite{Ke2004SVD}. 
% Compared with classic precoding techniques, which were looking for a good trade off between performance and complexity, deep learning as a new tool in precoding field, give us an opportunity to achieve outperform in both performance and complexity. 
% The idea and the goal of this work is to use deep learning to solve optimal but undesirable channel decomposition method (KLT) to achieve a general (feasible to both perfect/imperfect CSI and stationary/non-stationary channel) practical nonlinear precoding technique.


%%%%%%%%%%%%%%%% OLD RELATED WORK %%%%%%%%%%%%%%%%%%%%%
\begin{comment}
We categorize the related work into two categories:

\noindent
\textbf{Space-Time-Frequency Precoding:}
Precoding at the transmitter is advantageous due to the ability to achieve higher capacity and lower BER compared to equalization at the receiver, which typically suffers from noise enhancement \cite{vu2006exploiting,Cho2010MIMObook}. 
Further, it significantly reduces the computational burden on the user equipment.
While, precoding has attracted significant research, space-time-frequency interference is typically treated as two separate problems, where spatial precoding at the transmitter aims to cancel inter-user and inter-antenna interference, while equalization at the receiver mitigates ICI and ISI.
Alternately, \cite{} proposes an orthogonal time frequency OTFS modulation scheme that aims at mitigating ISI and ICI. 
While space-time-frequency block coding techniques are studied in the literature \cite{} they add redundancy and hence incur a communication overhead to mitigate space-time-frequency interference, which we avoid by precoding. 
Therefore, joint space-time-frequency precoding is unprecedented in the literature.


Linear precoding is the sub-optimal technique for weighted sum capacity with low complexity~\cite{LeeDPC2007}, which treats all transmitted signals as interference, except for the desired one. 
Nonlinear precoding is motivated by Dirty Paper Coding (DPC)~\cite{CostaDPC1983}, which codes the data by known channel interference. The coded transmitted signals of previous antennas are needed through feedback. It is approved to achieve capacity region of downlink MIMO channel~\cite{WeingartenDPC2006}.


To conclude, learning based precoding has significant advantages for solving non-convex optimization and high complexity problem. However, instead of focusing on specific model training, though it may achieve good performance in specific MIMO system, we have more interests on a general and explainable learning based method. 

\noindent
\textbf{Precoding for Non-Stationary Channels:}
The key to such precoding is extracting accurate eigenfunctions of the channel, however it is often impractical due to the high computational complexity and the availability of limited CSI at the transmitter \cite{}, especially when the channel is NS. 
% The paper \cite{} showed eigenfunctions are optimal to cancel interference but impractical. 

Second is the completeness of CSI. DPC can achieve the optimal weighted sum rate because each user's signal can be coded by treating precoded users' signals as noncausally known interference to completely cancel out interference, where the perfect CSI is needed. Imperfect CSI will significantly affect the performance of  NLP. However, though nonlinear precoding will degradation with imperfect CSI,~\cite{HatakawaNLP2012, HasegawaTHP2018, GuoTHP2020, DietrichTHP2007, CastanheiraPGS2013, WangTHP2012, MazroueiTDVP2016, Jacobsson1DAC2017} shows nonlinear precoding can still achieve better performance than linear precoding with certain imperfect CSI. In NS channel, the perfect CSI is not achievable. This work will work with the statistics CSI (S-CSI), whose change should be relative to channel non-stationarity. In this manner, we can investigate the performance gap with respect to channel non-stationarity (which will degrade to stationary channel with zero non-stationarity). 


Both linear and nonlinear precoding suffer from throughput loss with the outdated CSI.~\cite{AndersonLP2008} quantified this loss and proposed a linear precoder based on channel distribution information in time-varying downlink MIMO system. The method is robust to temporal variations so as to reduce the CSI feedback frequency.~\cite{LuLP2019} proposed robust linear precoders in massive MIMO downlink system with imperfect CSI. The available imperfect CSI for each UE obtained at the BS is modeled as statistical CSI under a jointly correlated channel model with both channel mean and channel variance information. The expected weighted sum-rate is very complicated and thus very difficult to be optimized directly. Minorize–maximize(MM) algorithm is used to find a stationary point of the optimization problem.~\cite{Zeng2012LP} investigated the linear precoding in MIMO fading channel with statistics CSI, such as the spatial correlation of channel, known at transmitted and perfect CSI known at receiver. The lower bound and upper bound of the mutual information with finite-alphabet inputs are derived. Then the optimal design for the left singular vector, power allocation vector and right singular vector are alternatively derived by maximizing the lower bound. The precoder combining three optimized vectors achieves near global optimal performance.

\noindent
\textbf{Complexity:}
Recently, quantized precoding techniques are proposed for massive MU MIMO~\cite{Jacobsson1DAC2017}, which aims to reduce the hardware complexity and circuit power consumption. It shows that low-resolution DACs can be applied at BS without a significant loss in terms of rates and BER. It also compared the linear-quantized precoding (ZF, WF, WFQ and MRT) and nonlinear-quantized precoding (SDR1, SDRr, SQUID and SP), showing that linear-quantized precoding can achieve sufficient performance for 3 to 4 bits DACs, but is much worse than nonlinear precoding for 1-bit DACs.~\cite{Jacobsson1DAC2018} is the latter work of ~\cite{Jacobsson1DAC2017}, which investigated the SQUID-OFDM technique. It is capable of supporting oversampling DACs and OFDM, and outperforms than linear-quantized precoding, but increases complexity and needs perfect CSI.~\cite{Chu1DAC2019} proposed another 1-bit DACs nonlinear precoding. It supports the MU-MIMO system with higher-modulation modes and can achieve comparable BER performance with SDR while being much faster.


It is well known that NLP usually achieves better performance than LP but suffers from high complexity. DPC is impractical due to the prohibitive complexity. As the practical implementation of DPC, THP can achieve sub-optimal performance due to energy loss in modulo, which outperforms LP but still has much higher complexity. 
Some modified NLP techniques proposed to reduce the complexity and meanwhile achieve comparative performance such as THP like precoding~\cite{HasegawaTHP2018}, D2VP precoding~\cite{MaD2VP2016} and quantized 1-DAC precoding~\cite{Chu1DAC2019}, where the latter two methods require perfect CSI.
Recently, deep learning attracts a lot of interests in communication system and shows the excellence in solving non-convex problems and reducing complexity~\cite{Goodfellow2016DL}. It can help to implement expensive techniques like Karhunen-Loeve transform (KLT), which is considered optimal but very undesirable~\cite{Ke2004SVD}. 
Compared with classic precoding techniques, which were looking for a good trade off between performance and complexity, deep learning as a new tool in precoding field, give us an opportunity to achieve outperform in both performance and complexity. 
The idea and the goal of this work is to use deep learning to solve optimal but undesirable channel decomposition method (KLT) to achieve a general (feasible to both perfect/imperfect CSI and stationary/non-stationary channel) practical nonlinear precoding technique.
\end{comment}


%%%%%%%%%%%%%%%%COMPLETE RELATED WORK%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Introduction to precoding}
\label{ssec:1_1}
Precoding techniques attract significant interests in MIMO system as it outperforms post-equalization, which suffers from noise enhancement~\cite{Cho2010MIMObook}. \cite{vu2006exploiting} shows that by exploiting CSI at the transmitter side, precoding can achieve higher capacity and lower BER. Meanwhile, downlink MIMO precoding can reduce the complexity load on the user equipment (UE). 


% classic
\noindent
\textbf{Linear precoding}
Linear precoding is the sub-optimal technique for weighted sum capacity with low complexity~\cite{LeeDPC2007}, which treats all transmitted signals as interference, except for the desired one. It aims to nullify or minimize interference by linear combination of information signals. The conventional linear precoding methods include the zero-forcing (ZF) technique and minimum mean square error (MMSE) technique. Unlike conventional linear precoders based on minimizing variants MSE criterion,~\cite{WieselLP2006} gives a strategy which models the optimization problem as two steps. First, the transmitted power is minimized subject to SINR constraints. In the second, the worst case SINR is maximized subject to a power constraint. The optimization is shown to be a conic optimization problem and can be directly solved. However, the strategy is subject to perfect CSI. By exploiting CSI at transmitter,~\cite{Stankovic2008lp} proposed a generalized precoding scheme in MU MIMO. It separates the multi-user inference (MUI) cancellation and system performance optimization. In the first step, conventional BD method will have poor performance if the row subspaces of users' channel matrices overlap significantly, so regularized block diagonalization (RBD) is proposed to reduce the overlap of the row spaces. In the second step, it assumes the channel are parallel SU MIMO channels by RBD. Then different criteria can be achieved by combining target precoding scheme. For example, by combining RBD and THP, regularized successive optimization THP precoding (RSO THO) can reach DPC bound when the dimensionality constraint is satisfied, though the BER performance is not very good with high MUI. 
Here, the general precoding means RBD can combine with different scheme to achieve different criteria. However, our paper aims to design a general precoding technique which adapts to both stationary and non-stationary channel. Similarly, we also divide the precoding design into two steps. First, we design an autoencoder to achieve nonlinear decomposition based on Karhunen–Loève transform (KLT). Second, we can design a precoding technique with KLT decomposition or combine it with other exist precoding techniques for different criteria. 

Both linear and nonlinear precoding suffer from throughput loss with the outdated CSI.~\cite{AndersonLP2008} quantified this loss and proposed a linear precoder based on channel distribution information in time-varying downlink MIMO system. The method is robust to temporal variations so as to reduce the CSI feedback frequency.~\cite{LuLP2019} proposed robust linear precoders in massive MIMO downlink system with imperfect CSI. The available imperfect CSI for each UE obtained at the BS is modeled as statistical CSI under a jointly correlated channel model with both channel mean and channel variance information. The expected weighted sum-rate is very complicated and thus very difficult to be optimized directly. Minorize–maximize(MM) algorithm is used to find a stationary point of the optimization problem.~\cite{Zeng2012LP} investigated the linear precoding in MIMO fading channel with statistics CSI, such as the spatial correlation of channel, known at transmitted and perfect CSI known at receiver. The lower bound and upper bound of the mutual information with finite-alphabet inputs are derived. Then the optimal design for the left singular vector, power allocation vector and right singular vector are alternatively derived by maximizing the lower bound. The precoder combining three optimized vectors achieves near global optimal performance.

Compared with our method, the above linear precoding techniques are subject to stationary channel. Even the channel is generalized to stationary, our method can still achieve better performance within certain CSI error due to nonlinearity. The most significant advantage of linear precoding is low complexity, but it will be mitigated by deep learning techniques. 

\noindent
\textbf{Nonlinear precoding}
Nonlinear precoding is motivated by Dirty Paper Coding (DPC)~\cite{CostaDPC1983}, which codes the data by known channel interference. The coded transmitted signals of previous antennas are needed through feedback. It is approved to achieve capacity region of downlink MIMO channel~\cite{WeingartenDPC2006}. \cite{LeeDPC2007} investigated the throughput of DPC and linear precoding at high SNR region and shows that by multiuser interference pre-canceling, multi-user(MU) MIMO DPC can be equivalent to one point-to-point MIMO without lose degree of freedom while linear precoding incurs relative penalty. DPC is considered as impractical due to its high complexity. Tomlinson–Harashima Precoding (THP) is the sub-optimal implementation of DPC, which is the combination of DPC and modulo operation~\cite{TomlinsonTHP1971}. With perfect CSI, THP is shown to significantly outperform linear precoding. However, THP is more sensitive to CSI error, and it is even outperformed by linear precoding with large CSI error~\cite{HatakawaNLP2012, HasegawaTHP2018}. \cite{GuoTHP2002} investigated a robust THP in multi-beam satellite downlink systems. This method uses norm-bounded error (NBE) model to bound the channel uncertainty and aims at maximizing the worst case of energy efficiency (EE). \cite{DietrichTHP2007} proposed the robust THP for MU MIMO BC channel. It can achieve better performance than both linear ZF precoding and traditional THP with partial or statistics CSI. However, this method needs a specific receiver knowing perfect CSI.

In addition to THP like nonliner precoding, ~\cite{CastanheiraPGS2013} investigated the performance of proposed projected Gauss-Seidel (PGS) nonlinear scheme and linear ZF with three power allocations for multicell multiuser MIMO-OFDM based systems. It shows per-BS PGS can achieve better performance as linear precoding needs full inversion of channel correlation matrix, while PGS only inverts part of the channel correlation matrix, leading to a better conditioned matrix.~\cite{WangTHP2012} consider a nonlinear precoding design for MIMO amplify-and-forward two-way relay systems. The nonlinear source coding design for fixed-relay is proven to be convex. However, jointly design problem is non-convex. Then two iterative algorithms are proposed to solve the problem. The source nonlinear joint precoding outperforms linear joint precoding but is sensitive to CSI error. This paper only considers nonlinear relay precoding since the nonlinear precoding design needs to jointly design the precoding matrix at the source.~\cite{MazroueiTDVP2016} investigated the performance of time-domain vector perturbation(TBVP) precoding in large-size system with imperfect CSI. It shows for large antennas array, TBVP is inferior to ZF. The conventional VP method search the entire Euclidean space for the global optimum point, while~\cite{MaD2VP2016} proposed degree-2 vector perturbation (D2VP) which break down the optimization process into several iterations in two optimally selected subspaces to achieve local optimization. This paper shows the local optimum point can be found in a closed form and reduce the complexity. However, this method requires perfect CSI.

Recently, quantized precoding techniques are proposed for massive MU MIMO~\cite{Jacobsson1DAC2017}, which aims to reduce the hardware complexity and circuit power consumption. It shows that low-resolution DACs can be applied at BS without a significant loss in terms of rates and BER. It also compared the linear-quantized precoding (ZF, WF, WFQ and MRT) and nonlinear-quantized precoding (SDR1, SDRr, SQUID and SP), showing that linear-quantized precoding can achieve sufficient performance for 3 to 4 bits DACs, but is much worse than nonlinear precoding for 1-bit DACs.~\cite{Jacobsson1DAC2018} is the latter work of ~\cite{Jacobsson1DAC2017}, which investigated the SQUID-OFDM technique. It is capable of supporting oversampling DACs and OFDM, and outperforms than linear-quantized precoding, but increases complexity and needs perfect CSI.~\cite{Chu1DAC2019} proposed another 1-bit DACs nonlinear precoding. It supports the MU-MIMO system with higher-modulation modes and can achieve comparable BER performance with SDR while being much faster.

All above nonlinear precoding techniques (except for TBVP in large-size system) show better capacity or BER performance than linear precoding in MIMO system with perfect or even imperfect CSI. However, these methods are still subject to stationary MIMO. The performance gap in non-stationary MIMO is worth studying. Generally nonlinear precoding suffers from high complexity. Though some modified techniques are looking for a good tradeoff between the performance and complexity, they may have other constraints such as perfect CSI. Our method aims to design a general precoder which targets imperfect CSI, non-stationary channel, comparative performance and low complexity. 

\noindent
\textbf{Learning based precoding}
Deep learning, as an excellent tool for the nonlinear problem with low complexity~\cite{Goodfellow2016DL} is successfully applied on precoding techniques.~\cite{Huang2019DLP} gives a deep neural network (DNN) based hybrid precoding in mmWave massive MIMO system. This paper use Saleh-Valenzuela (SV) channel model and adopt the GMD method to decompose the channel matrix. The loss function aim to reduce the difference between output precoder and GMD-based precoder.~\cite{Elbir2020DLP} designed a convolutional neural network(CNN) for multi-user mmWave MIMO system, which accepts imperfect channel matrix of users as inputs and output analog precoders and combiners. The training stage is offline and needs very large training data. The array response is only needed in the training stage.~\cite{Zhang2019DLP} proposed an offline DNN precoding for MIMO Gaussian wiretap channel and assume the number of antennas at the eavesdropper is known. The method can learn a sophisticated mapping between the channel matrix and the corresponding covariance matrix.~\cite{Sohrabi2021DLP} designed a distributed source coding (DSC) scheme for channel compression and jointly precoding in FDD massive MIMO. The framework has three phases, which jointly design the pilot in the downlink training phase, the channel estimation and feedback strategy adopted at users, and the multiuser precoding scheme at the BS. 

To conclude, learning based precoding has significant advantages for solving non-convex optimization and high complexity problem. However, instead of focusing on specific model training, though it may achieve good performance in specific MIMO system, we have more interests on a general and explainable learning based method. 

\subsection{Limitations and benefits of nonlinear precoding}
\label{ssec:1_2}
Nonlinear precoding is fully studied and has shown excellent performance in stationary MIMO system. However, to our best knowledge, few paper studies nonlinear precoding in non-stationary(NS) channel. Our paper aims to design a practical nonlinear precoding technique in NS channel due to following motivations:

\noindent
\textbf{Importance of non-stationary channel:}
In the next generation (xG) wireless communication system~\cite{Wang20206G}, a significant number of channels shows non-stationarity due to the distance-dependent path loss, shadowing, delay or Doppler drift and time-varying propagation, like UAV channel~\cite{Khuwaja2018UAV, Khawaja2019UAV} (urban, suburban, rural, and open field), maritime channel~\cite{Wang2018maritime} (UAV-to-ship, ship-to-ship, and ship-to-land), HST channel~\cite{HST} (open space, hilly terrain, viaduct, tunnels, cutting, stations, and intra-wagon), V2X channel~\cite{Mecklenbrauker2011} (highway, urban street, open area, university campus, and parking lot) and ultra-massive channel~\cite{CarvalhoNS2020, AliNS0219} (indoor and outdoor).
These scenarios are widely existed in real life, but the precoding technique for NS channels is rarely studied due to the difficulty of analyzing NS channels. This shows the novelty and significance of our work.

\noindent
\textbf{Performance gap:}
The performance gap between LP and NLP is influenced by two main aspects. 

One is the antenna size. When the number of transmitter antennas is not much larger than receiver antennas, i.e., $M\simeq KN$, the nonlinear precoding significantly outperforms linear precoding~\cite{LeeDPC2007}, but the advantage will quickly diminish with the number of transmitter antennas grows~\cite{Rusek2013MIMO}. However, there is still a performance gap between LP and NLP in large-scale MIMO with highly dense antennas array~\cite{MasourosVP2014}. From this property, though NLP may not achieve much outperformance in NS channels where the non-stationarity is caused by extra-large-scale MIMO with visibility region~\cite{CarvalhoNS2020, AliNS0219}, the performance gap in other NS channels is still remained.




The state of the art precoding techniques are categorized in Table~\ref{tab:1}. We classify precoding techniques into the classical precoding and the learning based precoding. The classical precoding usually solves criteria optimization problem and gives the expression of the solution, while learning based precoding use data to fit the solution. They are simply introduced in Section~\ref{ssec:1_1}. We evaluate the precoding techniques from four dimensions: NS channel, imperfect CSI, nonlinear and complexity. The importance of NS channel is discussed in Section~\ref{ssec:1_2}. However, all mentioned state of the art precoding assume the channel is stationary, which shows the most novelty of our work. Then the following two columns are discussed in performance gap. In the imperfect CSI column, some papers studied the precoding feasible to statistics CSI, while others studied the precoding robust to imperfect CSI (CSI error, outdated CSI). We classify these properties into the same column as they all aim to good performance with imperfect CSI. More detailed CSI assumption and criteria for the precoding are shown in Table~\ref{tab:2}. Table~\ref{tab:3} shows the complexity of each precoding method.


\begin{table}[h]
\centering
\scriptsize
\caption{\inred{Comparison of precoding techniques}}
\label{tab:1}
\begin{tabular}{|l|c|c|c|}
\hline
Precoding Type  & NS channels & Imperfect CSI & Nonlinear/Linear \\ 
 & (Stationarity) & (CSI Completeness) & (Precoding Alg.)\\ 
\hline \hline
\textbf{Classical} & & & \\
\begin{tabular}[]{@{}l@{}} Linear:\\\cite{WieselLP2006, Stankovic2008lp}\\ \cite{ AndersonLP2008, LuLP2019, Zeng2012LP}\end{tabular} &         &      \makecell[c]{ \\\ \\\checkmark}          &                   \\ 
\begin{tabular}[]{@{}l@{}} DPC/THP-like:\\\cite{CostaDPC1983, TomlinsonTHP1971}\\ \cite{ DietrichTHP2007, GuoTHP2020}\end{tabular} &         &      \makecell[c]{ \\\ \\\checkmark}          &      \makecell[c]{ \\\checkmark \\\checkmark}               \\ 
\begin{tabular}[]{@{}l@{}} Quantized:\\\cite{Jacobsson1DAC2018}\\ \cite{ Jacobsson1DAC2017, Chu1DAC2019}\end{tabular} &         &      \makecell[c]{ \\\ \\\checkmark}          &      \makecell[c]{ \\\checkmark \\\checkmark}               \\ 
\begin{tabular}[]{@{}l@{}} VP-based:\\\cite{MaD2VP2016}\\ \cite{ MazroueiTDVP2016}\end{tabular} &         &      \makecell[c]{ \\\ \\\checkmark}          &      \makecell[c]{ \\\checkmark \\\checkmark}               \\ 
PSG:~\cite{CastanheiraPGS2013} & &\checkmark &\checkmark            \\ 
Relay:~\cite{WangTHP2012} & &\checkmark &\checkmark            \\ 
\hline\hline
\textbf{Learning based} & & &\\
\begin{tabular}[]{@{}l@{}} Data driven:\\\cite{Huang2019DLP, Vu2021ML}\\ \cite{ Sohrabi2021DLP, Elbir2020DLP, Ma2020deep}\end{tabular} &         &      \makecell[c]{ \\\ \\\checkmark}          &   \makecell[c]{ \\\checkmark\\\checkmark}                    \\ 
\begin{tabular}[]{@{}l@{}} Model driven:\\\cite{Zhang2019DLP, Lei2021deep, He2020deepFA}\\ \cite{He2020deepCE}\end{tabular} &         &      \makecell[c]{ \\ \\\checkmark}          &   \makecell[c]{ \\\checkmark\\\checkmark}                    \\ \hline\hline
This paper & \checkmark & \checkmark & \checkmark\\ \hline
\end{tabular}
\end{table}

\noindent
\note{To include:
1. Why not treat the NS channel as many QS or WSSUS channels and use existing methods.
2. Why not use MIMO precoding methods that account for CSI error to deal with NS CSI: These approaches (\eg robust THP) typically deal with CSI error caused by error in channel estimation and hence cannot account for obsolete (i.e., outdated or out of distribution) CSI feedback in the case of NS channels \cite{}. 
% Book: https://www.google.com/books/edition/MIMO\_Systems/KyyaDwAAQBAJ?hl=en&gbpv=0, "MIMO Systems Theory and Applications", By Hossein Khaleghi Bizaki · 2011
}
\end{comment}

\begin{comment}
\begin{table}[h]
\centering
\tiny
\caption{Current precoding techniques}
\label{tab:2}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Paper  & Channel & CSI & Nonlinear/Linear & Criterion & Digital/Hybrid & Learning \\
& Stationarity & Completeness & Algorithm &  & Precoding & Architecture \\ 
\hline \hline
Wiesel et al.~\cite{WieselLP2006} & Stationary & Perfect CSI & Linear & Maximizing SINR & Digital & Non-learning \\
Stankovic et al.~\cite{Stankovic2008lp} & Stationary & Perfect CSI & Linear/nonlinear & Successive MMSE & Digital & Non-learning \\
Anderson et al.~\cite{AndersonLP2008} & Stationary & Outdated CSI & Linear & Maximizing rate & Digital & Non-learning\\
Lu et al.~\cite{LuLP2019} & Stationary &Statistical CSI &Linear & Maximizing expected weighted sum rate & Digital & Non-learning\\
Zeng et al.~\cite{Zeng2012LP} & Stationary &Statistical CSI &Linear & Maximizing lower bound of average mutual information & Digital & Non-learning\\
Costa~\cite{CostaDPC1983} & Stationary & Perfect CSI & Nonlinear & Maximizing mutual information & Digital & Non-learning\\
Tomlinson~\cite{TomlinsonTHP1971} & Stationary & Perfect CSI & Nonlinear & Maximizing mutual information & Digital & Non-learning\\
Ma et al.~\cite{MaD2VP2016} & Stationary & Perfect CSI & Nonlinear&
Maximizing EE& Digital & Non-learning\\
Jacobsson et al.~\cite{Jacobsson1DAC2018}& Stationary & Perfect CSI& Nonlinear & Minimizing MSE &Digital& Non-learning\\
Chu et al.~\cite{Chu1DAC2019}& Stationary & Perfect CSI& Nonlinear & Minimizing MSE &Digital& Non-learning \\ 
Castanheira~\cite{CastanheiraPGS2013}&Stationary& Perfect CSI& Nonlinear & Miniminzing BER& Digital &Non-learning\\ 
Dietriche et al.~\cite{DietrichTHP2007}& Stationary &Statistical CSI & Nonlinear& Minimizing MSE& Digital &Non-learning\\
Guo et al.~\cite{GuoTHP2020}& Stationary& Statistical CSI & Nonlinear& Maximizing worst case EE& Digital &Non-learning\\
Jacobsson et al.~\cite{Jacobsson1DAC2017}& Stationary &Imperfect CSI & Nonlinear & Minimizing MSE& Digital& Non-learning\\ 
Wang et al.~\cite{WangTHP2012}& Stationary& Imperfect CSI& Nonlinear & Minimizing MSE & Digital & Non-learning\\ 
Mazrouei et al.~\cite{MazroueiTDVP2016}& Stationary & Imperfect CSI& Nonlinear & Minimizing average power& Digital &Non-learning \\
Zhang et al.~\cite{Zhang2019DLP} & Stationary&Perfect CSI & Nonlinear &Maximixing capacity& Digital & Model-driven DNN\\
Huang et al.~\cite{Huang2019DLP}& Stationary& Perfect CSI& Nonlinear& Minimizing MSE & Hybrid& Data-driven DNN\\
Vu et al.~\cite{Vu2021ML} & Stationary & Perfect CSI &Nonlinear & Maximizing sum rate & Digital & Data-driven DNN \\
Lei et al.~\cite{Lei2021deep} & Stationary & Perfect CSI & Nonlinear &Maximizing constructive region threshold &Digital& Model-driven DNN\\
He et al.~\cite{He2020deepFA} & Stationary & Perfect CSI & Nonlinear &Minimizing MSE energy & Digital & Model-driven DNN\\
Gao et al.~\cite{Gao2017LP} & Stationary & Perfect CSI & Nonlinear & Maximizing sum rate & Hybrid & Model-driven ML\\ 
Elbir et al.~\cite{Elbir2020DLP} & Stationary& Imperfect CSI & Nonlinear & Maximizing sum rate& Hybrid& Data-driven CNN\\ 
Sohrabi et al.~\cite{Sohrabi2021DLP} & Stationary& Imperfect CSI& Nonlinear & Maximizing sum rate& Digital& Data-driven DNN\\ 
Ma et al.~\cite{Ma2020deep} & Stationary & Imperfect CSI & Nonlinear & Maximizing beamforming gain & Hybrid & Data-driven CNN\\
He et al.~\cite{He2020deepCE} & Stationary & Imperfect CSI & Nonlinear &Minimizing MUI energy & Digital & Model-driven DNN\\
\hline
This paper & Non-stationary& Statistical CSI& Nonlinear& &Digital& \\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\scriptsize
\caption{Current precoding complexity}
\label{tab:3}
\begin{tabular}{|l|l|}
\hline
Paper & Complexity\\
\hline \hline
Wiesel et al.~\cite{WieselLP2006} & Conic optimization for SINR\\\hline
Stankovic et al.~\cite{Stankovic2008lp} & Regularized block diagonaliztion with three modifications\\\hline
Anderson et al.~\cite{AndersonLP2008} & $O(M^4)$,$O(2M^2)$ and $O(3M^2)$ for different channel modes\\
& (M is antennas per node)\\\hline
Lu et al.~\cite{LuLP2019} & $O(KM_t^3)$, $O(\dfrac{1}{2}M_t^3)$ and $O(KM_kM_t)$ per iteration \\
&(K is the number of UEs)\\ \hline
Zeng et al.~\cite{Zeng2012LP} & Numerical running time significantly \\
&less than maximizing average mutual information\\\hline
Costa~\cite{CostaDPC1983} & %$O(([KN_t]^{3.5}+K^2N_t M)K!log(\epsilon^{-1})))$ 
$O(K!K^3)$(Need to verify)\\\hline
Tomlinson~\cite{TomlinsonTHP1971} & $O(K!K^3)$~\cite{DietrichTHP2007} \\\hline
Ma et al.~\cite{MaD2VP2016} &$O(2S(\dfrac{5}{3}U^3+3BU^2+(6B-\dfrac{2}{3})U)+4TB(2SU+2Nlog_2N-5N+8)) $\\
& (T is iteration times; S is ocuppied subcarriers; U is number of UEs; N is the number of samples per OFDM symbol) \\\hline
Chu et al.~\cite{Chu1DAC2019}& $O(R^2)$ \\
& (R is number of signal components)\\\hline
Castanheira~\cite{CastanheiraPGS2013}& Numerical running time $6$ times higher than linear ZF SOCAP\\ \hline
Dietriche et al.~\cite{DietrichTHP2007}& $O(K^3)$\\\hline
Guo et al.~\cite{GuoTHP2020}& Iterative maximizing EE by CVX tool\\\hline
Jacobsson et al.~\cite{Jacobsson1DAC2017}& $O((2(k_1R^3 + k_2 R^2))$~\cite{Chu1DAC2019}\\
& ($k_1$ and $k_2$ are iteration number of two loops, and R is the number of antennas)\\\hline
Wang et al.~\cite{WangTHP2012}& $O(n_{ite}(n_{ite}^s(N+1)^2+\ceil[\big]{log_2(\overline{N}/e)}))$ \\ 
& ($n_{ite}$is the number of iterations;$e$ is error precision; $\overline{N}$ is the preset search upper bound)\\\hline
Mazrouei et al.~\cite{MazroueiTDVP2016} & Perturbed data vector calculation\\\hline
Zhang et al.~\cite{Zhang2019DLP} & Numerical running time less than AO-WF and GSVD \\\hline
Huang et al.~\cite{Huang2019DLP}& $O(L^2N_sN_t^2)$\\\hline
Vu et al.~\cite{Vu2021ML} & $96\%$ sum rate with $5\%$ complexity compared with exhaustive search\\\hline
Lei et al.~\cite{Lei2021deep} & $2(K+KN)r_1 +2K N r_{L-1} + \sum_{l=2}^{L-1}r_{l-1}r_l)$\\
&  ($r_i$ is the number of nodes at layer $i$)\\\hline
He et al.~\cite{He2020deepFA}& $O(2NK+N)$\\\hline
Gao et al.~\cite{Gao2017LP} & $ O(ISNK)$ \\ 
& (I is iteration times; S is number of channel matrix)\\\hline
Elbir et al.~\cite{Elbir2020DLP} & Numerical running time less than LRHB, TS-HB, SOMP but longer than MLP\\ \hline
Sohrabi et al.~\cite{Sohrabi2021DLP} & Fully connected DNN learning linear precoder matrix\\ \hline
Ma et al.~\cite{Ma2020deep} & $6$ layers to learn analog precoders with input matrix\\\hline
He et al.~\cite{He2020deepCE} & Numerical running time less than RMO-based CG and Sequential GD \\
\hline
This paper & \\ \hline
\end{tabular}
\end{table}
\end{comment}

==> results_icc22.tex <==
\section{Results}

\begin{comment}
\noindent
\textbf{Non-stationary channel precoding:}
We consider a $100$ time instance channel. At each instance, the minimal delay taps are $10$ and maximum delay taps are $20$. The channel gains at delay taps is Gaussian distributed with mean and variance changing over time. Figure~\ref{fig:stat} shows the boxplot of channel gains. 
\begin{figure}[h]
  \centering
  \includegraphics[width=0.6\linewidth]{figures/boxplot.png}
  \caption{Distribution of channel gains at delay taps changing over time.}
  \label{fig:stat}
\label{fig:stat}
\end{figure}


\begin{figure}[h]
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/time_varying_response.png}
  \caption{Time-varying impulse response $h(t,\tau)$.}
  \label{fig:ht}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/kht.png}
  \caption{Kernel $k_H(t,t')$.}
  \label{fig:kht}
\end{subfigure}
\caption{Example of Non-WSSUS channel.}
  \vspace{-10pt}
\label{fig:ns}
\end{figure}

Figure~\ref{fig:ht} and Figure~\ref{fig:kht} gives an example of time-varying impulse response $h(t,\tau)$ and kernel $k_H(t,t')$, respectively. By theorem~\ref{thm:GMT}, $k_H(t,t')$ can be decomposed to infinite eigenfunctions $\{\psi_n(t)\}$ and $\{\phi_n(t')\}$.
\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/tranceiver.png}
  \caption{Example of transmit and receive signal pair.}
  \label{fig:x_and_r}
\label{fig:x_and_r}
\end{figure}

The transmit signal energy is set as $||x(t)||^2 {=} T$. Figure~\ref{fig:x_and_r} gives the example of transmit signal $x(t)$ and the received signal $r(t)$ at non-WSSUS noise free channel. In the first few instances, the received signal $r(t)$ has error, that's because the transmitted signal before $t {=} 0$ is unknown, whose delays will affect the signal at first few instances. As maximal delay taps is $20$, $s(t)$ is error free when $t \geq 20$.

\noindent
\textbf{Spatial precoding:} consider a noise-free BC channel with $100$ users. The spatial channel $k_H(u,u')$ is shown in figure~\ref{fig:hs}, which can be decomposed to eigenfuntions at space domian $\{\psi_n(u)\}$ and $\{\phi_n(u')\}$. The precoded signal $x(u)$ can be obtained by thoerem~\ref{thm:thm2}. Figure~\ref{fig:tranceiver_space} shows an example of transmit signal and receive signal pair. Different from time-varying response where the kernel $k_H(t,t')$ can not describe the delay effects of signals with $t<0$, spatial domain only consider effects among users, which can be fully described by kernel $k_H(u,u')$. Thus the received channel $r(u)$ can perfect fit the data signal $s(u)$. 

\begin{figure}[h]
  \centering
  \includegraphics[width=0.7\linewidth]{figures/hs.png}
  \caption{Example of spatial channel kernel $k_H(u,u')$.}
  \label{fig:hs}
\label{fig:hs}
\end{figure}


\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/tranceiver_space.png}
  \caption{Example of transmit and receive signal pair for different users.}
  \label{fig:tranceiver_space}
\label{fig:tranceiver_space}
\end{figure}

\end{comment}



% \noindent
We analyze the accuracy of the proposed unified channel characterization and joint spatio-temporal precoding using a non-stationary channel simulation framework in Matlab.
% \note{Rewrite in a practical sense: e.g., The CSI corresponding to 10 users for 100 time instances were used to compute a 4-D kernel. Mention known CSI or CSI with Gaussian error.}
% \note{Check this: 
The simulation environment considers $10$ mobile receivers (users) and $100$ time instances of a non-stationary 4-D kernel $k_H(u,t;u',t')$, where the number of delayed symbols (delay taps) causing interference are uniformly distributed between $[10,20]$ symbols for each user at each time instance. 
% \ingreen{
% Then the decomposition of the kernel involves: 


The pre-processing of the 4-D channel kernel and 2-D data symbols involves mapping them to a low-dimensional space using an invertible mapping %$f$, i.e, 
$f{:}u{\times}t{\to}m$.
Although Theorem \ref{thm:hogmt} decomposes the channel kernel into infinite %number of 
eigenfunctions, we show that it is sufficient to decompose the channel kernel into a finite number of eigenfunctions and select only those whose eigenvalues are greater than a threshold value $\epsilon^2$ for precoding, i.e., $\{(\phi_n(\cdot),\psi_n(\cdot)): \sigma_n{>}\epsilon\}$.
These eigenfunctions are used to calculate the coefficients for joint spatio temporal precoding, which subsequently construct the precoded signal after inverse KLT. 
% We study the BER performance of precoding using  for 16QAM modulated symbols, . We also compared the proposed methods for BPSK, QPSK, 16QAM and 64QAM in Appendix E.
% The precoded signal 

% Since the channel kernel is complex (contains twice as many eigenfunctions as a real-valued kernel), it is split into real and imaginary parts before decomposition 
% Then split them to real and imaginary parts and construct new kernel and new data symbols with same linear relation, which are used to get precoded signal by HOGMT-precoding. Then combine the real and imaginary parts and do inverse mapping, the final precoded symbol is obtained. More details are in Appendix E. 


\begin{figure}[t]
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/hs_1.pdf}
  \caption{4-D kernel $k_H(u,t;u',t')$ at $t {=} 1$ and $t' {=} 1$ which shows the spatial interference}
  \label{fig:hs1}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/ht_1.pdf}
  \caption{4-D kernel $k_H(u,t;u',t')$ at $u {=} 1$ and $u' {=} 1$ which shows the temporal interference}
  \label{fig:ht1}
\end{subfigure}
  \caption{Separately spatial and delay effects of 4-D kernel}
\end{figure}

% \ingreen{Theoretically, channel kernel is decomposed to infinite eigenfunctions. However, in implementation we can choose finite eigenfunctions with eigenvalues $\lambda{>}\epsilon$ to approximate kernel. ([] shows KLT can approximate kernel with N eigenfunctions).}
% We use PAM for this demonstration. 
% Add more on the implementation of the channel simulator and the decomposition technique: The channel gains at each delay tap is Gaussian distributed with its mean and variance changing over time (how does it change over time, is the change also Gaussian?).
% 
% }
% 
% 
% 
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.5\linewidth]{figures/boxplot.pdf}
%   \caption{The distribution of the mean channel gains at channel delay taps. 
% %   \note{If possible, show also the variance.}
% }
%   \label{fig:stat}
% \label{fig:stat}
% \end{figure}
% \ingreen{
% The number of basis at complex space is twice at real space. To get sufficient eigenfunctions, first do dimension reduction to 4-D kernel and 2-D data symbols by invertible mapping $f{:}u{\times}t{\to}m$. Then split them to real and imaginary parts and construct new kernel and new data symbols with same linear relation, which are used to get precoded signal by HOGMT-precoding. Then combine the real and imaginary parts and do inverse mapping, the final precoded symbol is obtained. More details are in Appendix E. 
% }
Figure~\ref{fig:stat} shows distribution of the statistics of the channel gain (mean and variance) for each time instance of the non-stationary channel and further corroborates its non-stationarity. 
% \note{What is its significance? \ingreen{Figure 4 is just for showing the channel is NS}}
% 
% 
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.6\linewidth]{figures/Joint_space_time_interference.pdf}
%   \caption{Channel kernel $k_H(u,t;u',t')$ for $u {=} 1$ and $t {=} 50$. \ingreen{interference or response?}
% %   \ingreen{Be careful if it's appropriate to call kernel as interference. At least $K_H(1,50,1,50)$ is not interference but channel attenuation/gain.}
%   }
% %   \note{Include z label and same scale.}}
%   \label{fig:joint_interference_kernel}
% \end{figure}
% 
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.6\linewidth]{figures/Eigenfunctions.pdf}
%   \caption{2-D Eigenfunctions.}
% %   \note{Include z label and same scale.}}
%   \label{fig:Eigenfunctions}
% \label{fig:Eigenfunctions}
% \end{figure}
% 

\begin{figure*}[t]
\centering
\begin{subfigure}{.27\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/Eigenfunctions.pdf}
  \caption{Dual spatio-temporal eigenfunctions decomposed from kernel $k_H(u,t;u',t')$ by HOGMT}
  \label{fig:Eigenfunctions}
\end{subfigure}
\qquad
\begin{subfigure}{.27\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/Ber_space_time.pdf}
  \caption{BER of HOGMT based spatial-temporal precoding for different $\epsilon$ and comparison with the state-of-the-art}
%   $\epsilon {=} 0.02$, $0.01$, $0.005$, and $0.001$, and comparison with the state-of-the-art}
  \label{fig:ber_space_time}
\end{subfigure}
\qquad
\begin{subfigure}{.27\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/Ber_space_time_multimod.pdf}
  \caption{BER of HOGMT based spatio-temporal precoding for BPSK, QPSK ,16-QAM and 64-QAM modulations}
  \label{fig:Ber_space_time_multimod}
\end{subfigure}
  \caption{HOGMT based spatio-temporal precoding}
  \vspace{-20pt}
\end{figure*}
Figure~\ref{fig:joint_interference_kernel} shows the channel response for user $u {=} 1$ at $t{=}50$ which indicates the manifestation of interference. For $u{=}1$, the spatial interference from other users (inter-user interference) occurs on the red plane (at $t'{=50}$), while the temporal interference at $t{=}50$ occurs due to previous delayed symbols (inter-symbol interference) on the grey plane (at $u'{=}1$). However, the received symbols at user $u{=}1$ is also affected by other delayed symbols from other users (i.e., $t'{<50}$ for $u'{\neq}1$), which leads to joint spatio-temporal interference, and necessitates joint precoding over space-time dimensions. 
The varitation of the channel kernels over time and for different users is demonstrated and further explained in Appendix D in \cite{appendix_link} for completion.
% We call it space-time joint interference.  
This is the cause of joint space-time interference which necessitates joint precoding in the 2-dimensional space using eigenfunctions that are jointly orthogonal.
% Figure~\ref{fig:hst_1_10_50_100} shows the channel response for user $u {=} 1$ at $t{=}1$, $t{=}10$, $t{=}50$ and $t{=}100$, where at each instance, the response for user $u {=} 1$ is not only affected by its own delay and other users' spatial interference, but also affected by other users' delayed symbols. 
% % We call it space-time joint interference.  
% This is the cause of joint space-time interference which necessitates joint precoding in the 2-dimensional space using eigenfunctions that are jointly orthogonal.

Figure~\ref{fig:hs1} shows the spatial (inter-user) interference caused by other users for a fixed time instance (time instances $t{=}1$ and $t'{=}1$) in terms of the 4-D channel kernel, i.e., $k_H(u,1,u',1)$. 
% 
Figure~\ref{fig:ht1} shows the temporal (inter-symbol) interference for a user $u{=}1$ caused by its own (i.e., $u'{=}1$) delayed symbols (\eg due to multipath), i.e., $k_H(1,t;1,t')$. We also observe that the temporal interference for each user occurs from it's own 20 immediately delayed symbols. 
% (\rood{Zhibin: What is the largest delay in symbols that cause interference} \ingreen{Maximal delay is 20. We have mentioned the delay taps are uniformly distributed between[10,20]}).

\begin{comment}
\begin{figure}[h]
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/Ber_space.pdf}
  \caption{Spatial Precoding}
  \label{fig:ber_space}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/Ber_space_time_multi_EP.pdf}
  \caption{Spatio-temporal precoding}
  \label{fig:ber_space_time}
\end{subfigure}
  \caption{BER performance for EP with $\epsilon {=} 0.02$, $0.01$, $0.005$, and $0.001$, and comparison with the state-of-the-art}
\end{figure}
\end{comment}

% 
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.6\linewidth]{figures/Ber_space_time_multi_EP.pdf}
%   \caption{BER performance for EP with $\epsilon {=} 0.02$, $0.01$, $0.005$, and $0.001$, and comparison with the state-of-the-art}
% %   \note{Include z label and same scale.}}
%   \label{fig:ber_space_time}
% \end{figure}
% 
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.6\linewidth]{figures/ber_precoding.pdf}
%   \caption{BER performance of space-time precoding.} 
% %   \note{Include a comparison with SoTA.}}
%   \label{fig:Ber}
% \end{figure}
% \note{Figures \ref{fig:Eigenfunctions} shows two pairs of dual spatio-temporal eigenfunctions in $\{\phi_n(u',t')\}$ and $\{\psi_n(u,t)\}$ decomposed from $k_H(u,t;u',t')$. Eigenfunctions of different pairs are jointly orthorgonal across space-time domain. Propagating the eigenfunction of one pair will give another the eigenfunction of this pair at receiver, so the non-stationary fast fading 4-D channel is decomposed to dual flat fading sub-channels.}
% Figures \ref{fig:Eigenfunctions} shows two pairs of dual spatio-temporal eigenfunctions in $\{\phi_n(u',t')\}$ and $\{\psi_n(u,t)\}$ decomposed from $k_H(u,t;u',t')$ as in \eqref{eq:thm2_decomp}, 
Figure \ref{fig:Eigenfunctions} shows two pairs of dual spatio-temporal eigenfunctions $(\phi_n(u',t'),\psi_n(u,t))$ (absolute values) %in $\{\phi_n(u',t')\}$ and $\{\psi_n(u,t)\}$ 
obtained by decomposing $k_H(u,t;u',t')$ in \eqref{eq:thm2_decomp}.
We see that this decomposition is indeed asymmetric as each $\phi_n(u',t')$ and $\psi_n(u',t')$ are not equivalent (but shifted), and that each $\phi_1(u',t')$ and $\psi_1(u,t)$ are jointly orthogonal with $\phi_2(u',t')$ and $\psi_2(u,t)$ as in \eqref{eq:properties}, respectively.
Therefore, when $\phi_1(u',t')$ (or $\phi_2(u',t')$) is transmitted through the channel, the dual eigenfunctions, $\psi_1(u,t)$ (or $\psi_2(u,t)$) is received with $\sigma_1$ and $\sigma_2$, respectively.
Therefore, the non-stationary 4-D channel is decomposed to dual flat-fading sub-channels.
% \ingreen{where $\phi_1(u',t')$ and $\psi_1(u,t)$ are jointly orthogonal with $\phi_2(u',t')$ and $\psi_2(u,t)$, respectivly. Further, we see that transmitting $\phi_1(u',t')$ or $\phi_2(u',t')$ will give us $\psi_1(u,t)$ or $\psi_2(u,t)$ with $\sigma_1$ and $\sigma_2$, respectively.
% Therefore, the non-stationary 4-D channel is decomposed to dual flat-fading sub-channels.} 
% \note{The figure shows the asymmetric channel decomposition as $\phi$ and $\psi$ are not the same.}
%
% Further, we see that transmitting one of the eigenfunction in the pair $\phi_n(u',t')$ will give the other eigenfunction, $\psi_n(u,t))$ of the pair at the receiver. 
% Therefore, the non-stationary 4-D channel is decomposed to dual flat-fading sub-channels.
% 


Figures \ref{fig:ber_space_time} shows the %performance of the 
BER at the receiver, using joint spatio-temporal precoding (HOGMT-precoding) at the transmitter with 16-QAM modulated symbols for non-stationary channels.
% 
Since this precoding is able to cancel all interference that occurs in space, time and across space-time dimensions which are shown in figure \ref{fig:joint_interference_kernel}, 
% \ingreen{
it achieves significantly lower BER over existing precoding methods that employ DPC %precoding 
at the transmitter to cancel spatial interference and Zero Forcing equalization at the receiver to mitigate temporal interference. 
Further, we show that with sufficient eigenfunctions ($\epsilon{=}10^{-4}$ in this case), proposed method can achieve near ideal BER, only 0.5dB more SNR to achieve the same BER as the ideal case, where the ideal case assumes all interference is cancelled and only AWGN noise remains at the receiver.
% The precoding requires only 0.5dB more SNR to achieve the same BER as the ideal case, where the 
This gap exists since practical implementation employs a finite number of eigenfunctions as opposed to an infinite number in \eqref{eq:thm2_decomp}. 
Figure \ref{fig:Ber_space_time_multimod} compares the BER of HOGMT based spatio-temporal precoding for various modulations (BPSK, QPSK, 16-QAM and 64-QAM) for the same non-stationary channel with $\epsilon{=}10^{-3}$.
As expected we observe that the lower the order of the modulation, the lower the BER but at the cost of lower data rate. 
However, we observe that even with high-order modulations (\eg 64-QAM) the proposed precoding achieves low BER (${\approx}10^{-2}$ at SNR${=}20$dB), allowing high data-rates even over challenging non-stationary channels. The choice of the order of the modulation is therefore, based on the desired BER and data rate for different non-stationary scenarios.
% Different modulation schemes are the trade-off between BER and data rate for different senarios.
% \ingreen{The 0.5dB gap is because, in practice the precoding employs a finite number of eigenfunctions as opposed to an infinite number in \eqref{eq:thm2_decomp}.
% }


% it achieves significantly lower BER over existing precoding methods that employ DPC %precoding 
% at the transmitter to cancel spatial interference and Zero Forcing equalization at the receiver to mitigate temporal interference. 
% Further, we show that the BER improves by accommodating more number of eigenfunctions in the precoding step in Theorem \ref{thm:thm2}, i.e., by using a smaller threshold $\epsilon$, %the BER improves with increasing number of eigenfunctions, 
% however there is no significant improvement for $\epsilon{<}10^{-4}$. 
% The ideal scenario is one in which assume %there is 
% perfect precoding of the non-stationary channel where only AWGN noise remains at the receiver, which is shown for comparison. The proposed precoding only requires about 0.5 dB more SNR to achieve the same BER as the ideal case. %as highlighted. 
% This gap is because, in practice the precoding employs a finite number of eigenfunctions as opposed to an infinite number in \eqref{eq:thm2_decomp}.

% Moreover, we observe that the proposed precoding only 
% Corollary 1 -- 7a corresponds -- alternate 6a.
% Corollary 2 -- 
% Theorem 1: In 7b EP cancels all interference in 5 (5c), while DPC+Eq cancels all interference in both slices in 5 or 6a and 6b. 

% \noindent
% \textbf{Space case:} 
Figure \ref{fig:spatial_precoding} shows an example of precoding for an example of a multi-user deterministic channel defined by the 2-D kernel, $K_H(u,u')$ with 30 mobile users as defined in \eqref{eq:h_space}, where only spatial interference from other users exists. 
The spatial interference from other users is portrayed in figure \eqref{fig:Hs} in terms of $K_H(u,u')$. The achieved BER at the receiver by precoding using Corollary \ref{col:EP_space} is shown in figure \ref{fig:ber_space} and is compared with the state-of-the-art DPC for spatial precoding \cite{CostaDPC1983}. 
The performance of HOGMT based spatial precoding for various modulations with $\epsilon{=}10^{-3}$ is compared in figure \ref{fig:Ber_space_multimode}.
\begin{figure*}[t]
\centering
\begin{subfigure}{.27\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/Hs.pdf}
  \caption{2-D kernel $k_H(u,u')$ where only spatial interference exists}
  \label{fig:Hs}
\end{subfigure}
\qquad
\begin{subfigure}{.27\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/Ber_space.pdf}
  \caption{BER of HOGMT based spatial precoding for different $\epsilon$ and comparison with the state-of-the-art}
  \label{fig:ber_space}
\end{subfigure}
\qquad
\begin{subfigure}{.27\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/Ber_space_multimod.pdf}
  \caption{BER of HOGMT based spatial precoding for BPSK, QPSK, 16-QAM and 64-QAM modulations }
  \label{fig:Ber_space_multimode}
\end{subfigure}
  \caption{HOGMT based spatial precoding}
  \label{fig:spatial_precoding}
  \vspace{-10pt}
\end{figure*}
We observe that with low number of eigenfunctions ($\epsilon{=}10^{-1}$), the proposed precoding results in higher BER than DPC because precoding using these limited eigenfunctions is not sufficient to cancel all the spatial interference. 
% Although the proposed precoding results in higher BER than DPC with $\epsilon{=}10^{-1}$, %and similar BER with $\epsilon{=}5{\times}10^{-2}$ for SNR greater than 15dB. 
However, with more eigenfunctions ($\epsilon{=}10^{-2}$), it achieves significantly lower BER compared to DPC for SNR ${>}9$dB and consequently only requires 3dB more SNR to achieve the same BER as the ideal case.
In contrast, while DPC is optimal in the sum rate at the transmitter is not optimal in terms of the BER at the receiver and its BER performance depends on the complementary decoding performed at the receiver.



% \ingreen{We observe proposed method achieve higher BER than DPC with $\epsilon{=}10^{-1}$, and similar BER with $\epsilon{=}5{\times}10^{-2}$ for SNR greater than 15dB. However, with $\epsilon{=}10^{-2}$, it can achieve significant lower BER than DPC for SNR greater than 13 dB and consequently is only around 2dB away from the ideal precoding scenario at 20dB SNR. .
% In contrast, while DPC is optimal in the sum rate at the transmitter is not optimal in terms of the BER at the receiver and its BER performance depends on the complementary decoding performed at the receiver. 
% In both simulations, we use 16QAM modulation. We also compared the proposed methods for BPSK, QPSK, 16QAM and 64QAM in Appendix E.(You can put this at the beginning of this section)}
% We observe a \rood{88.27\%} improvement in BER using the proposed precoding since it uses the constituent eigenfunctions of the spatial channel to precode, and consequently is only \rood{2dB} away from the ideal precoding scenario at \rood{15dB} SNR. 
% In contrast, while DPC is optimal in the sum rate at the transmitter is not optimal in terms of the BER at the receiver and its BER performance depends on the complementary decoding performed at the receiver.
%obtained by decomposing non-stationary channels. 
% \rood{Zhibin: Why do we see an improvement if this is for deterministic channels, where DPC is optimal?}

\begin{comment}
\noindent
\textbf{Complexity:}
In the implementation, we map space-time dimension to one dimension, the mapping is invertible. Then do SVD and mapping back to achieve 2-D eigenfunctions. Complexity of Theorem~\ref{thm:thm2} in our simulation is $O((L_u \times L_t)^3 + N (L_u \times L_t))$, where $L_u$ and $L_t$ are length of user and time domain, respectively. $N$ is the number of eigenfunctions. The complexity of DPC is about $O(L_t \times L_u!)$.
\end{comment}

\begin{comment}
\noindent
\textbf{Future work:} corollary~\ref{col:svdforNSchannel} can extend the theorem~\ref{thm:thm2} to higher dimension, which gives us chance to implement space-time or even space-time-frequency joint precoding which can minimize the joint interference. The joint precoding require decomposing high dimensional eigenfunctions, which would be planes for 2-D and tensors for 3-D. The deep learning method give us chance to implement it. Meanwhile, we will also investigate the system implementation i.e., consider channel estimation and robust precoding with eigenfunctions under CSI error.
\end{comment}

==> results_old.tex <==
\section{Evaluation and Results}
\label{sec:results}


% \subsection{Characteristic curves}
% \note{Performance and penalty plots with $n,d,w,$ and completeness metric. The pareto surface. }
% This is shown in figure \ref{fig:characteristic_curves}.

We analyze the impact of training and the model structure of {\tnn} receiver on the equivalence with {\tmap} using a practical simulation framework.
% and compare its performance against classical receivers. %to corroborate the theoretical results.
% We analyze the various facets of this NN-based receivers using a practical simulation framework and compare its performance against classical receivers to corroborate the theoretical results.
The simulation parameters are detailed in table \ref{tab:notations}.
Experiments are conducted on 100 sets of training samples of size $n$ drawn randomly from different channel distributions including AWGN and Rayleigh channels. 
The model structure of {\tnn} is parameterized by its number of trained parameters, $N{=}|\delta_n^*|$.
% , and is equal to the total number of weights and biases in {\tnn}, where $|.|$ is the cardinality.
In general, $N$ is a measure of the depth and width of {\tnn} and determines its capacity to generalize beyond the training data \cite{ML_Probability_book_Murphy}.
100 different neural networks for each choice of $n$ and $N$ are trained using different training sets and initializations of the {\tnn} parameters. 
% Then, we estimate 
$\mu_n$ and $\sigma_n^2$ are estimated as described in Section \ref{sec:ber_bounds}, where the population expectation $\mathbb{E}_{\mathcal{D}}$ is estimated over the validation set. 
% Furthermore, we compute 99\% confidence intervals for the bias and variance estimates.
{\tnn} is trained using SCGD \cite{SCGD} and its parameters, are initialized by randomly sampling from a distribution whose variance is inversely proportional to $N$, i.e, $\delta_{0}{\sim}\mathcal{N}\left(0,\frac{1}{N}\mathbf{I}\right)$. %the width of the NN-receiver.

\begin{table}%[h]
\centering
%\renewcommand{\arraystretch}{1}
\caption{Simulation Parameters}
\label{tab:notations}
%\vspace{-5pt}
\begin{tabular}{|c|c|}
\hline
Parameters/Hyperparameters & Value/Model\\
\hline
Neural Network Type & Deep Feed-Forward NN\\
Empirical Risk ($\mathcal{R}$)  & Mean-Squared Error (MSE)\\
Training Algorithm & Scaled Conjugate Gradient Descent(SCGD)\\ 
Activation Function ($\phi_l$) & Hidden:Tan-Sig \cite{Vogl2004AcceleratingTC}, Output:Softmax\\
Channel Models & AWGN, Rayleigh\\
Antenna Configuration & SISO, MIMO\\ 
%Node Speed & 0-20 m/s\\
Number of Hidden Layers & [3, 5]\\
Number of Input Neurons & 2 (I,Q streams)\\
Number of Output Neurons & $M=[2,4,16,64]$\\
Number of Samples ($n$) & $10^2$ - $10^5$\\
Number of Parameters ($N$) & $10^0$ - $10^5$\\
Training,Validation,Testing  & [60, 20, 20] \%\\ 
%\cite{SHA}\\
% Maximum Difficulty ($D_{max}$) & 16 \\
% Tuning parameter ($\alpha$) & 0.5 \\
\hline
\end{tabular}
%\vspace{-5pt}
\end{table}
\setlength{\textfloatsep}{10pt}


% \subsection{Simulation Framework}
% {\abbrev} is evaluated on a mobile sensing and Blockchain simulator built on Matlab. 

% We analyze the various facets of this paper using practical simulations.


% \note{
% Take an existing dataset and plot the BER curve based on measures of data.
% }

\subsection{Model Parameters of {\tnn} for Equivalence}
% \subsection{Learnability and Generalizability}
\begin{figure}[h]
        \centering
        \begin{subfigure}{0.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bias_variance_num_samples_empirical.pdf}
                \caption{With amount of training $n$}%Constellation before pre-compensation
                \label{fig:bias_variance_num_samples}
        \end{subfigure}% 
        \
        \begin{subfigure}{0.24\textwidth}
         \includegraphics[width=\textwidth]{figures/bias_variance_num_parameters_new.pdf}
                \caption{With number of parameters $N$}%Constellation after pre-compensation
                \label{fig:bias_variance_num_parameters}
        \end{subfigure}
	\caption{Bias and Variance of the expected risk of {\tnn}.}
	\label{fig:bias_variance}
%	\vspace{-10pt}
\end{figure}

% The expected risk of the {\tnn} receiver is a measure of its ability to learn to classify the signals or its \textit{learnability}.
Designing computationally efficient {\tnn} receivers, require determining the amount of training and its structure %of the NN model 
that guarantee minimum BER.
% number of training samples and the size of the neural network that guarantee minimum BER.
Figure \ref{fig:bias_variance} shows the variation of the bias and variance of {\tnn} with the number of training samples, $n$ and the number of parameters, $N$ for received data drawn from AWGN channels averaged over SNR from 0-20dB. 
% The number of parameters of the {\tnn} is given by $N{=}|\delta^*|$, where $|.|$ is the cardinality. 
% For the {\tnn}, $N{=}|\delta^*|$ is the total number of weights and biases in the {\tnn} and is a measure of its model complexity or its depth and width \cite{ML_Probability_book_Murphy}, where $|.|$ is the cardinality.
Figure \ref{fig:bias_variance_num_samples} shows a decreasing trend in the average values of $\mu_n$ and $\sigma_n^2$ with increasing $n$, over all possible $N$. 
% {\tnn} receiver, i.e., $N$ is fixed. 
This indicates that the expected risk and consequently the BER decreases as more training samples are incorporated,  
% Figure \ref{fig:bias_variance_num_samples} shows a clearly decreasing trend in the bias and variance with increasing $n$ for a fixed structure of the {\tnn} receiver, i.e., $N$ is fixed. This shows that the expected risk and consequently the BER decreases as number of training samples increases. 
However, we also observe that there is negligible improvement in $\mu_n$ and $\sigma_n^2$ %the bias or variance 
for $n{\geqslant}10^3$ samples. %for AWGN channels. 
Therefore, we set $n_{emp}{=}10^3$ for which the structural risk is approximately zero, and consequently the complete training criteria is approximately achieved.
% Moreover, when $n{\geqslant}n_{emp}$, the complete training criteria is approximately achieved.
% 
Figure \ref{fig:bias_variance_num_parameters} shows a convex trend of $\mu_n$ and $\sigma_n^2$ %the bias and variance 
with increasing $N$ for a fixed $n{=}10^3$, with a minimum when $N{=}10^2$. 
% Since, $N$ determines the training and computational complexity of {\tnn}, the choice of $N$ is crucial to ensuring computationally efficient design. %and minimum BER. 
It is clear that under-parameterized ($N{\ll}10^2$) and over-parameterized ($N{\gg}10^2$) {\tnn} receivers result in large $\mu_n$ and $\sigma_n^2$ and 
Therefore, we observe that for a given $n$, there exists a specific structure of {\tnn} with $N{=}10^2$, for which the structural risk and consequently the BER is minimum. 
% Moreover, it is clear that under-parameterized ($N{\ll}10^2$) and over-parameterized ($N{\gg}10^2$) {\tnn} receivers result in large $\mu_n$ and $\sigma_n^2$ and consequently high BER. 
% This result also corroborates the existence of a specific structure (width and depth) of the {\tnn} receiver, for which the expected risk is minimum for a given $n$. 
% In other words, for a given $n$, the width and depth of the {\tnn} receiver can be pre-determined to ensure the minimum BER among all possible {\tnn} receivers. 
% The choice of $N$ also determines the training and computational complexity of the {\tnn} receiver. Therefore, determining the empirically determining the value of $N$ allows for computationally efficient implementation of {\tnn} that achieves minimum BER.

\begin{figure}[h]
        \centering
        \begin{subfigure}{0.15\textwidth}
		\includegraphics[width=\textwidth]{figures/underfittedF.pdf}
                \caption{Under fitted boundaries, $N{\ll}10^2$}%Constellation before pre-compensation
                \label{fig:underfit}
        \end{subfigure}% 
        \enskip
        \begin{subfigure}{0.15\textwidth}
        \includegraphics[width=\textwidth]{figures/overfittedF.pdf}
                %\includegraphics[width=\textwidth]{figures/over_fitted_decision_boundaryF.pdf}
                \caption{Over fitted boundaries, $N{\gg}10^2$}%Constellation after pre-compensation
                \label{fig:overfit}
        \end{subfigure}
        \enskip
        \begin{subfigure}{0.15\textwidth}
		\includegraphics[width=\textwidth]{figures/perfectfittedF.pdf}
                \caption{Perfect fitted boundaries, $N{=}10^2$}%Constellation before pre-compensation
                \label{fig:perfectfit}
        \end{subfigure}% 
	\caption{Decision boundaries of the {\tnn} for AWGN channel %at SNR${=}6$dB 
	for 16-QAM constellation.}
	\label{fig:decision_boundary}
%	\vspace{-10pt}
\end{figure}
% Figure \ref{fig:decision_boundary} shows the impact of the number of parameters $N$ or the structure of the {\tnn} receiver on the learned decision boundaries for an AWGN channel for $SNR{=}6$dB for a 16-QAM constellation when there is only limited samples available, $n=10^3$. 
Figure \ref{fig:decision_boundary} shows the impact of the structure of {\tnn} (i.e., the choice of $N$) on the learned decision boundaries for an AWGN channel 
% for $SNR{=}6$dB 
for 16-QAM constellation when only limited training samples are available, $n{=}10^3$. 
% Hence, we set $$
% It is well-known that 
For AWGN channel, the optimum decision boundaries %(for which the error rate is minimum) 
of {\tmap} %or the nearest-neighbour decoder 
are the perpendicular bisectors of the lines connecting the constellations, which guarantees minimum error rate \cite{Proakis2007Book}.
Therefore the learned decision boundaries by {\tnn}, is a visual metric to explain its behaviour, and gauge its ability to achieve equivalence and generalize beyond the training data. 
% data on which it is trained. 
When {\tnn} is under-parameterized ($N{\ll}10^2$), the decision boundaries are underfitted and are not the optimal boundaries. Therefore, more training samples are required to learn the optimum boundaries. 
% We observe that the when $N{\ll}10^2$, the decision boundaries are underfitted, i.e., the decision boundaries are not the optimal boundaries, and more training samples are required to learn the optimum boundaries. 
When {\tnn} is over-parameterized ($N{\gg}10^2$), the decision boundaries are overfitted to the specific data samples on which it is trained and the noise. 
% It is clear that the %decision boundaries of a complex 
This is because the {\tnn} receiver configures the decision boundaries to also accommodate outliers in the training set, and therefore will not generalize to data not seen during training.
Therefore, we observe that for a given $n$, there exists a specific structure of {\tnn} and choice of $N$ for which the learned decision boundaries are optimum, and consequently result in the minimum BER. 
We also highlight that under complete training, $n{\rightarrow}\infty$), {\tnn} will always learn the optimum decision boundaries, due to its capacity to as universal approximators \cite{Cybenko1989ApproximationBS}, regardless of the choice of $N$.

\subsection{Impact of Training Schemes on Equivalence}
\begin{figure}[h]
        \centering
		\includegraphics[width=0.25\textwidth]{figures/ber_training_schemes.pdf}  %{FullSystemFFF.pdf}
% 		\vspace{-30pt}
        \caption{BER of the {\tnn} for AWGN channel for 16-QAM modulation scheme with different training schemes.
        }   %IMAGE MUST BE MODIFIED
        \label{fig:training_snr}
    %  \vspace{-10pt}   
\end{figure}
% \begin{figure}[h]
%         \centering
%         \begin{subfigure}{0.15\textwidth}
% 		\includegraphics[width=\textwidth]{figures/berNN_M16_eachSNR.pdf}
%                 \caption{Trained at each SNR ($n=10^4$).}%Constellation before pre-compensation
%                 \label{fig:each_snr}
%         \end{subfigure}% 
%         \enskip
%         % \quad \quad \quad
%         \begin{subfigure}{0.15\textwidth}
%                 \includegraphics[width=\textwidth]{figures/berNN_M16_allSNR.pdf}
%                 \caption{Trained over all SNR ($n=10^4$).}%Constellation after pre-compensation
%                 \label{fig:all_snr}
%         \end{subfigure}
%         \enskip
%         \begin{subfigure}{0.15\textwidth}
%                 \includegraphics[width=\textwidth]{figures/berNN_M16_SNR6dB_2.pdf}
%                 \caption{Trained at 6dB SNR ($n=10^5$).}%Constellation after pre-compensation
%                 \label{fig:one_snr}
%         \end{subfigure}
% 	\caption{BER of the {\tnn} receiver for AWGN channel for 16QAM modulation scheme with different training schemes.}
% 	\label{fig:training_snr}
% % 	\vspace{-10pt}
% \end{figure}
The impact on the BER by the SNR at which the {\tnn} receiver is trained is investigated in figure \ref{fig:training_snr}.
It is clear that under complete training that is representative of the entire channel distribution, the {\tnn} receiver will learn the optimum decision boundaries.
% It is clear that provided complete training that is representative of the entire channel distribution the {\tnn} receiver will learn the optimum decision boundaries.
% For a given $n$, it is clear that provided complete training that is representative of the entire channel distribution the {\tnn} receiver will learn the optimum decision boundaries.
Therefore, we observe that training different {\tnn} models for each SNR or training a single {\tnn} model over all SNR eventually learn the optimum decision boundaries and achieve equivalent BER as the {\tmap} receiver under complete training (\eg $n{=}10^4{\gg}10^3$). 
These results corroborate the significance of training the {\tnn} receiver using a dataset that is representative of the entire channel distribution.
Alternatively, figure \ref{fig:training_snr} also shows that for AWGN channels, provided that the {\tnn} receiver is trained at a sufficiently low SNR (\eg SNR${=}6$dB), it is still able to achieve equivalent BER as {\tmap}, because it learns the optimal decision boundaries. 
However, when the training SNR is high (SNR${\geqslant}9$dB), the decision boundaries are configured for lower-noise margins and is not able to handle the noise at lower SNRs, and consequently results in high BER.

\subsection{Error Performance of the {\tnn} Receiver}
\begin{figure}[h]
        \centering
        \begin{subfigure}{0.25\textwidth}
		\includegraphics[width=\textwidth]{figures/ber_num_samples.pdf}
                \caption{BER for AWGN channel for 16-QAM modulation scheme.}%Constellation before pre-compensation
                \label{fig:ber_awgn}
        \end{subfigure}% 
        % \quad \quad \quad
        \begin{subfigure}{0.25\textwidth}
        \includegraphics[width=\textwidth]{figures/ber_rayleigh_MIMO_MRC.pdf}
                \caption{BER for MIMO Fading channel for BPSK modulation scheme.}%Constellation after pre-compensation
                \label{fig:ber_rayleigh}
        \end{subfigure}
	\caption{BER comparison of {\tnn} and {\tmap}: a) for SISO AWGN channel, and b) for MIMO Rayleigh fading channel with MRC employed at the {\tnn}.}
	\label{fig:ber_curves}
%	\vspace{-10pt}
\end{figure}
Figure \ref{fig:ber_curves} shows the BER of the {\tnn} receiver for SISO and MIMO systems using AWGN and Rayleigh fading channels as representative examples of stationary channels with known distribution. 
Figure \ref{fig:ber_awgn} confirms that with more training samples ($n{\geqslant}10^3$), the BER of {\tnn} approaches that of {\tmap}.
Figure \ref{fig:ber_rayleigh} shows the performance of the {\tnn} receiver for multiple-antenna systems when MRC is employed at the receiver to combine the streams from each antenna. 
It is also clear that the proposed feed-forward neural network based receiver is able to achieve equivalent BER as the {\tmap} receiver under sufficient training over a variety of channels. This corroborates the theoretical equivalence of {\tnn} and {\tmap} receivers, under sufficient training and choice of structure of {\tnn}. 
% We further observe that under finite training, the BER of the {\tnn} receiver is upper-bounded by $P_{UB}$ as derived in Theorem \ref{thm:ber_bounds}.










% \subsection{Comparison with Black-box approaches}

% % \note{
% \noindent
% 1. Use an existing black-box model with source code.\\ 
% 2. Implement the {\tnn} for a given $n$.\\
% 3. Show the gains of your model in terms 
% }
% \subsection{Known Channel Distributions}

% \subsection{Unknown Channel Distributions}


% \begin{table}
% \centering
% \renewcommand{\arraystretch}{1.3}

% \caption{Simulation Parameters}
% \label{tab:notations}
% %\vspace{-5pt}
% \begin{tabular}{|c||c|}
% \hline
% Parameters & Value/Model\\
% \hline
% Area & 300m $\times$ 300m\\
% Node Distribution & Uniform Distribution\\ 
% Mobility Model & Random Waypoint\\ 
% Propagation Model & Log-distance propagation model \cite{maqsood2018spatio}\\
% Path-loss exponent ($\gamma$) & 3 (urban area) \\
% % shadowing dB-spread & 2-20 dB
% Carrier Frequency (f) & 600 MHz\\
% Number of Validators & 5\\
% Number of Sensors & 20\\
% Antenna Type & Omnidirectional\\
% Broadcast Range & 100\\
% %Node Speed & 0-20 m/s\\
% Maximum Difficulty ($D_{max}$) & 16 \\
% Block-wait Time ($\tau_{\mathcal{B}}$) & 7 s \\
% Target location error ($d_{err}$) & Uniformly distributed in [20,30] m \\
% \hline
% \end{tabular}
% \vspace{-5pt}
% \end{table}
% \setlength{\textfloatsep}{15pt}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/ber_match_Rayleigh.pdf}
%     \caption{BER for {\tnn} and {\tmap} receiver for 16QAM modulation scheme.}
%     \label{fig:my_label}
% \end{figure}





==> system.tex <==
\section{System Design}
\label{sec:system}

\begin{comment}
\begin{corollary}
\label{col:svdfortensors}
The tensor form of theorem~\ref{thm:svdforfunctions}: Let $\mathbf{K}$ be $P$ order tensor with rank $N$, obtained by Kronecker product of $P$ vectors $\mathbf{K} = \mathbf{x}_1 \otimes \mathbf{x}_2 \otimes,...,\otimes \mathbf{x}_P$. Then $\mathbf{K}$ can be expressed by
\begin{equation}
\mathbf{K} = \sum_n^N \sigma_n \mathbf{u}_n^{(1)}\otimes \mathbf{u}_n^{(2)} \otimes,...,\otimes \mathbf{u}_n^{(P)}
\end{equation}
where $\sigma_n$ is singular value. $\{\mathbf{u}_n^{(p)}\}_n$ are eigenvectors.
Specially, when $P$ = 2, it's the same with SVD.
\end{corollary}
\end{comment}


\subsection{CSI Processing \& Eigendecomposition}
\label{sec:AE}


\begin{definition}
Given a $k^2$ order tensor $\mathcal{A}(A_{j_1,j_2,\cdots,j_k})$, where $A_{j_1,j_2,\cdots,j_k}$ is the $k$ order cell. If
\begin{equation}
    \mathcal{A}(\langle A_{j_1,j_2,\cdots,j_k}, T_i\rangle_{\mathrm{F}}) = \lambda_i T_i
\end{equation}
where $\langle\mathbf{\cdot}, \mathbf{\cdot}\rangle_{\mathrm{F}}$ is \textit{Frobenius inner product}. Then $T_i$ is a $k$ order eigentensor, where eigentensor $T_i$ is orthonormal. 
\begin{align}
    &\langle T_i, T_i\rangle_{\mathrm{F}} = 1 \nonumber \\ 
    &\langle T_i, T_j\rangle_{\mathrm{F}} = 0 \quad \text{for }\quad i \neq j \nonumber \\ 
\end{align}

\begin{comment}
    \begin{equation}
    \langle\mathbf{A}, \mathbf{B}\rangle_{\mathrm{F}}=\sum_{i, j} \overline{A_{i j}} B_{i j}=\operatorname{Tr}\left(\overline{\mathbf{A}^{T}} \mathbf{B}\right) \equiv \operatorname{Tr}\left(\mathbf{A}^{\dagger} \mathbf{B}\right)
    \end{equation}
\end{comment}

\end{definition}

\begin{corollary}
\label{col:svdfortensors}
The tensor form of corollary~\ref{col:svdforNSchannel}: 
Denote non-stationary jointly Gaussian channel as six order tensor $\textbf{H}$. The entry $H(u,k,p; m,l,q)$ denotes the space-time-frequency response of user $u$ at time $k$ (period of k is OFDM symbol duration time) and carrier $q$.
$\textbf{H}$ can be expressed as 
\begin{equation}
    \textbf{H} = \sum_n^N \sigma_n \textbf{A}_n \otimes \textbf{B}_n
\end{equation}
where \textbf{A} and \textbf{B} are both three order tensors and have entry $A(u,k,p)$ and $B(m,l,q)$, respectively.
\end{corollary}


\begin{theorem}
% The proposed autoencoder provides a computationally efficient and correct decomposition of the channel into KLT eigenfunctions.
\inred{Need modify} Training a deep autoencoder by sequentially feeding  each column of hankel matrix represented as $\textbf{x}$ (or each lateral slice of hankel tensor) with the following regularized loss, 
% $\mathcal{L}{=}\mathcal{J}{+}\Omega$, where $\mathcal{J}{=}\|\textbf{x}-\hat{\textbf{x}}\|^2$ ($\textbf{x}$ represents each column of the hankel matrix $\textbf{U}$ which is used to train the AE) and $\Omega$ as defined below,
\begin{align*}
% \small
\mathcal{L}&{=}\mathcal{J}{+}\Omega, \quad \text{where}, \quad \mathcal{J}{=}\|\textbf{x}-\hat{\textbf{x}}\|^2\\
% \operatorname{L}_{KLT}(\Phi)=-\sum_{i=1}^{m} \phi_{i}^{\mathrm{T}} Q \phi_{i}+ \gamma \sum_{i=1}^{m}\left(\phi_{i}^{T} \phi_{i}-1\right)+ \beta \sum_{i=1}^{m} \sum_{j=1}^{i-1} \phi_{i}^{T} \phi_{j}+ \eta \sum_{i=1}^{m} \sum_{j=1}^{i-1}  \phi_{i}^{T} Q \phi_{j}
% \Omega(\boldsymbol{W}_{dec})= \lambda \left(\sum_{i{=}1}^{M}\left(w_{i}^{H} \phi_{i}-1\right)+ \sum_{i=1}^{M} \sum_{j=1}^{i-1} \phi_{i}^{H} \phi_{j}+ \sum_{i=1}^{M} \sum_{j=1}^{i-1}  \phi_{i}^{H} \mathbf{R_{\mathbf{xx}}} \phi_{j} \right)
\Omega(\boldsymbol{W}_{dec})&{=} \lambda \left([\boldsymbol{W}_{dec}^H\boldsymbol{W}_{dec}-\boldsymbol{I}] + \boldsymbol{W}_{dec}^H\mathbf{R_{\mathbf{xx}}}\boldsymbol{W}_{dec}\right)
\end{align*}
ensures that the weights of the trained AE, $W_{enc}^T=W_1^TW_2^T{\ldots}W_d^t=W_{dec}\rightarrow \mathbf{\Phi}$.
\end{theorem}

The proof is presented in Appendix.

\begin{comment}
Transmitting the unprecoded data $S$, we receive $y(u,k,p)$ at the receiver\footnote[1]{$\circledast_d$ denotes d-dimensional convolution.},
\begin{align}
   &y(u,k,p) {=} h(u,k,q;u,k,q)\circledast_3 s(u,k,q) \nonumber\\
   &{=} \sum_{m}\sum_{l}\sum_{q} h(u,k,p;m,l,q) s^*(u-m,k-l,p-q) \nonumber\\
   &{=}  h(u,k,p;0,0,0) s(u,k,p) \\
   &{+} \sum_{m' \neq 0} \sum_{l'\neq 0} \sum_{q' \neq 0} h(u,k,p;m',l',q') s^*(u-m',k-l',p-q')\nonumber
\end{align}
The second item is space-time-frequency interference.
\note{\noindent
Space-time-frequency interference not only includes IUI, ISI and ICI, but also includes IUI-ISI-ICI joint interference. 
Therefore, joint precoding is benefitial compared to separate precoding.
}
%
The \textit{channel correlation function} (CCF) is 
\begin{align}
    & R_h(\Delta u, \Delta k, \Delta p;\Delta m, \Delta l, \Delta q) {=} \sum_{u} \sum_{k} \sum_{p} E \{h(u,k,p;m,l,q) \\
    & {\cdot} h(u + \Delta u, k + \Delta k, p + \Delta p; m +\Delta m, l + \Delta l, q + \Delta q)\}\\
    & {=} \sum_{n}^ N \lambda_n R_{\psi_n}(\Delta u,\Delta k,\Delta p) R_{\phi_n}(\Delta m,\Delta l, \Delta q)
\end{align}

The \textit{local scattering function} (LSF) is
\begin{align}
    & C_h(u, k, p; m, l, q) {=} \sum_{u} \sum_{k} \sum_{p}R_h(\Delta u, \Delta k, \Delta p;\Delta m, \Delta l, \Delta q) \\
    & {\cdot} h(u + \Delta u, k + \Delta k, p + \Delta p; m +\Delta m, l + \Delta l, q + \Delta q)\}\\
    & {=} \sum_{n}^ N \lambda_n R_{\psi_n}(\Delta u,\Delta k,\Delta p) R_{\phi_n}(\Delta m,\Delta l, \Delta q)
\end{align}

%
Before precoding, we need to extract space-time-frequency joint orthogonal functions.
% 
The \textbf{Mix} module is to combine space-time-frequency response of all users over all moments and carriers. 
% 
\begin{equation}
z(m,l,q) = \sum_{u} \sum_{k} \sum_{p} h(u,k,p;m,l,q)
\end{equation}
% 
Through \textbf{AE-KLT}, we have eigenfunctions that are jointly orthonormal in space-time-frequency.
\begin{align}
&z(m,l,q) = \sum_{n=1}^N \sigma_n \phi_n(m,l,q), \quad \text{where,} \quad \\
&\sum_m \sum_l \sum_q \phi_n(m,l,q)\phi^*_n(m,l,q) {=} 1\\
&\sum_m \sum_l \sum_q \phi_n(m,l,q)\phi^*_{n'}(m,l,q) {=} 0 ~\text{for}~n \neq n'
\end{align}
% 
As $z(m,l,q)$ combine all $h(u,k,p;m,l,q)$, the eigenfunctions decomposed from $z(m,l,q)$ are also basis of $h(u,k,p;m,l,q)$.
\begin{equation}
h(u,k,p;m,l,q) = \sum_{n=1}^N \sigma_n(u,k,p) \phi_n(m,l,q)
\end{equation}

where, $\sigma_n(u,k,p)$ can be obtained by \textbf{Projection}
\begin{equation}
\sigma_n(u,k,p) = \sum_{m} \sum_{l} \sum_{q} h(u,k,p;m,l,q) \phi_n^*(m,l,q)
\end{equation}
\end{comment}
\subsection{Space-time-frequency Eigen-Precoding}
\begin{comment}

\textbf{Precoding} $X = W(\Sigma, \Phi; S)$ has two parts:

\noindent
\textbf{Step A:} \textbf{Minimize IUI-ISI-ICI} module is to design $\{x_n\}$ that can achieve least sum distance in space-time-frequency domain  (minimal total interference).
\begin{equation}
\label{eq:argmin}
\argmin_{\{x_n\}} \sum_{u} \sum_{k} \sum_{p}||s(u,k,p) - \sum_{n=1}^N x_n \sigma_n(u,k,p)||^2
\end{equation}
\note{\noindent
Given tensor S and the tensor set {$\Sigma_n(u,k,p)$}, how to combine {$\Sigma_n(u,k,p)$} with the coefficients $x_n$ to get the minimal distance from S (interference). If it is one dimension (vector), it's easy to cancel the interference (depends on the rank of basis). Higher order, harder to cancel all interference.

The combination problem is suitable to NN.

Minimizing BER criteria: Let $r(u,k,p) = \sum_{n=1}^N x_n \sigma_n(u,k,p)$, and given noise variance $\sigma_0^2$. If a QAM symbol $s(u,k,p)$ has decision region $D(u,k,p)$, and let $C\{r(u,k,p), \sigma_0\}$ denotes a circle area with center $r(u,k,p)$ and radius $\sigma_0$,  the minimizing BER criteria would be

\begin{align}
& \argmax_{\{x_n\}} \sum_u \sum_k \sum_p D(u,k,p) \cap C\{r(u,k,p), \sigma_0\} \quad \text{where,} \quad\\
& r(u,k,p) {=} \sum_{n=1}^N x_n \sigma_n(u,k,p)
\end{align}
}

\noindent
\textbf{Step B:}
The \textbf{construction} module constructs $X$ by linear combining the eigenfunctions with the designed coefficients $\{x_n\}$.
% 
\begin{equation}
x(u,k,p) = \sum_{n=1}^N x_n \phi_n(m-u,l-k,q-p)
\end{equation}
Transmitting the precoded data $X$, we receive $y'(u,k,p)$ at the receiver given by, 
% 
\begin{align}
    &y'(u,k,p) {=} h(u,k,p;u,k,p) \circledast_3 x(u,k,p) + w(u,k,p)\nonumber\\
    &{=} \sum_{m} \sum_{l} \sum_{q} h(u,k,p;m,l,q) x^*(u-m,k-l,p-q) \nonumber\\
    & {+} w(u,k,p)\nonumber \nonumber\\
    & {=} \sum_{m} \sum_{l} \sum_{q} \sum_{n=1}^N \sigma_n(u,k,p) \phi_n(m,l,q) \nonumber \\  
    &{\cdot} \sum_{n'=1}^N x_{n'} \phi_{n'}^*(m,l,q) {+} w(u,k,p) \nonumber\\
    & {=} \sum_{n=1}^N x_{n} \sigma_n(u,k,p) \sum_{m} \sum_{l} \sum_{q}  \phi_n(m,l,q) \phi_{n}^*(m,l,q) \nonumber\\
    & {+} {\sum_{n'\neq n}^N x_{n'} \sigma_n(u,k,p) \sum_{m} \sum_{l} \sum_{q}} \phi_n(m,l,q) \phi_{n'}^*(m,l,q)\nonumber \\
    &{+} w (u,k,p) \nonumber\\
    & {=} {\sum_{n=1}^N} x_n \sigma_n(u,k,p){+} w (u,k,p) \nonumber
\end{align}

\end{comment}
\begin{comment}

\subsection{Performance analysis}
For non-precoding data $S$, we can get the KLT expasion:
\begin{equation}
    s(u,k,p) = \sum_n s_n \phi_n(m-u,l-k,q-p)
\end{equation}

The total interference is 
\begin{align}
&\epsilon {=} \sum_{u} \sum_{k} \sum_{p}||s(u,k,p) - \sum_{n=1}^N s_n \sigma_n(u,k,p)||^2 \\
& {\leq} \sum_{u} \sum_{k} \sum_{p}||s(u,k,p) - \sum_{n=1}^N x_n \sigma_n(u,k,p)||^2
\end{align}

\end{comment}


\begin{comment}
\begin{equation}
\begin{aligned}
\mathcal{H}(X(t)) &=\int_{0}^{T_{m}} H(t;\tau) X(t-\tau) d \tau \\
&=\int_{0}^{T_{m}} \int_{-B_{d} / 2}^{B_{d} / 2} H(\tau, \nu) X(t-\tau) e^{j 2 \pi \nu t} d \nu d \tau 
\end{aligned}
\end{equation}

Where $H(t;\tau) = [H_1^H(1, t;\tau),\cdots,H_M^H(t;\tau)]^H$. 


The eigenfunction $\phi_n(\tau,\nu)$ and eigenvalue $\lambda_n$ of $H_u(\tau,\nu)$ are defined by the eigenequation
\begin{equation}
H_u\phi_n(\tau, \nu) = \lambda_n \phi_n(\tau,\nu)
\end{equation}


By KLT, we can also get 
\begin{equation}
Z(\tau, \nu) = \sum_{n=1}^N \sigma_n \phi_n(\tau,\nu)
\end{equation}
\end{comment}

\begin{comment}
\note{Why eigenfunctions: If we have a flat fading channel H, we can transmit data through the orthogonal space of the channel to cancel ISI. We know any channel can be represented by orthogonal sine waves. So we can transmit data trough frequency space, which is OFDM. but when it comes to delay-Doppler time-varying channels. There will be interferences at frequency space. So we can find eigenfunctions jointly orthogonal at time-frequency space to cancel ISI-ICI joint interference. Expand it to space, eigenfunctions can jointly orthogonal at space-time-frequency domain and cancel IUI-ISI-ICI.}
\end{comment}


